The Direct and Spillover Effects of Large-scale Affirmative Action at an Elite Brazilian University

We examine the effects of an affirmative action policy at an elite Brazilian university that reserved 45 percent of admission slots for Black and low-income students. We find that marginally-admitted students who enrolled through the affirmative action tracks experienced a 14 percent increase in early-career earnings. But the adoption of affirmative action also caused a large decrease in earnings for the university's most highly-ranked students. We present evidence that the negative spillover effects on highly-ranked students' earnings were driven by both a reduction in human capital accumulation and a decline in the value of networking.

==> results/apply_summ_dd.tex <==
Total applicants &47,633 & &50,553 &4,374 &2,118 &58 \\
Applicants in RD sample &0 & &0 &0 &0 &0 \\
Enrollees in DD sample &13,765 & &14,105 &2,469 &1,326 &38 \\
Top enrollees in DD sample &8,534 & &9,179 &495 &253 &9 \\\midrule
Female &0.56 & &0.53 &0.62 &0.63 &0.57 \\
Age at applicantion &22.34 & &21.62 &22.54 &24.09 &26.24 \\
White (UERJ data) & & &0.59 &0.49 &0.03 &0.32 \\
White (RAIS data) &0.75 & &0.65 &0.60 &0.20 &0.47 \\
Mother has a high school degree & & &0.78 &0.45 &0.52 &0.43 \\
HH income $>$ 1.5$\times$ min. wage & & &0.74 &0.28 &0.30 &0.25 \\
%Standardized admission score &0.00 & &0.05 &-0.39 &-0.40 &-0.43 \\


==> results/apply_summ_rddd.tex <==
Total applicants &95,659 & &159,408 &10,996 &7,263 &318 \\
Applicants in RD sample &93,930 & &159,383 &9,624 &5,600 &0 \\
Enrollees in DD sample &15,512 & &11,588 &4,465 &3,241 &211 \\
Top enrollees in DD sample &7,932 & &8,922 &362 &178 &2 \\\midrule
Female &0.50 & &0.55 &0.60 &0.60 &0.48 \\
Age at applicantion &20.75 & &20.28 &21.88 &23.04 &24.30 \\
White (UERJ data) & & &0.64 &0.49 &0.03 &0.35 \\
White (RAIS data) &0.78 & &0.67 &0.57 &0.15 &0.48 \\
Mother has a high school degree & & &0.85 &0.49 &0.56 &0.54 \\
HH income $>$ 1.5$\times$ min. wage & & &0.82 &0.35 &0.35 &0.45 \\
%Standardized admission score &-0.00 & &0.06 &-0.48 &-0.52 &-0.64 \\


==> results/bal_f.tex <==
Joint balance test ($ p$ value)&&&&1.729&&&&1.034&&&&0.523&\\


==> results/bal_n.tex <==
\(N\) (applicants within BW = 0.5)&&3,234&&30,213&&4,012&&39,914&&543&&6,461&\\


==> results/bal_no_rais_f.tex <==
\quad Excluding RAIS variables&&&&2.492&&&&0.522&&&&0.573&\\


==> results/bal_no_rais_p.tex <==
\quad Excluding RAIS variables&&&&0.058&&&&0.819&&&&0.778&\\


==> results/dd_aa_age.tex <==
Age at application&&0.281&&0.113&&0.526&\sym{**}&0.146&\\
&&(0.210&)&(0.324&)&(0.237&)&(0.319&)\\


==> results/dd_aa_black.tex <==
Black&&0.016&&$-$0.029&\sym{**}&0.051&\sym{***}&$-$0.020&\\
&&(0.011&)&(0.014&)&(0.013&)&(0.014&)\\


==> results/dd_aa_black_brown.tex <==
Black or Brown&&0.017&&$-$0.041&\sym{*}&0.073&\sym{***}&$-$0.020&\\
&&(0.017&)&(0.022&)&(0.020&)&(0.022&)\\


==> results/dd_aa_brown.tex <==
Brown&&0.001&&$-$0.012&&0.022&\sym{*}&0.001&\\
&&(0.009&)&(0.013&)&(0.012&)&(0.014&)\\


==> results/dd_aa_enrol.tex <==
Enrolled in UERJ&&$-$0.020&&0.022&&&&&\\
&&(0.040&)&(0.027&)&&&&\\


==> results/dd_aa_grad.tex <==
Graduated from UERJ&&0.022&&0.050&\sym{**}&0.056&\sym{**}&0.055&\sym{**}\\
&&(0.029&)&(0.024&)&(0.025&)&(0.026&)\\


==> results/dd_aa_male.tex <==
trt_post&&$-$0.044&\sym{**}&$-$0.021&&$-$0.045&\sym{**}&$-$0.031&\\
&&(0.019&)&(0.022&)&(0.018&)&(0.022&)\\


==> results/dd_aa_n.tex <==
\(N\)&&105,560&&28,603&&52,330&&28,602&\\


==> results/dd_aa_pct_aa_py.tex <==
Prop.\ of classmates from AA tracks&&0.106&\sym{***}&0.108&\sym{***}&0.244&\sym{***}&0.244&\sym{***}\\
&&(0.021&)&(0.035&)&(0.025&)&(0.025&)\\


==> results/dd_aa_pct_avg.tex <==
Average percentile subject tests&&0.016&&$-$0.002&&$-$0.025&&0.003&\\
&&(0.018&)&(0.023&)&(0.022&)&(0.023&)\\


==> results/dd_aa_pct_writing.tex <==
Writing score percentile&&0.011&&0.029&&$-$0.023&&0.017&\\
&&(0.017&)&(0.021&)&(0.018&)&(0.023&)\\


==> results/dd_aa_score_pct.tex <==
Enrollees' admission score percentile&&$-$0.027&&0.011&&$-$0.001&&0.001&\\
&&(0.018&)&(0.007&)&(0.001&)&(0.001&)\\


==> results/dd_aa_white.tex <==
White&&$-$0.020&&0.036&&$-$0.077&\sym{***}&0.016&\\
&&(0.017&)&(0.023&)&(0.020&)&(0.023&)\\


==> results/dd_admit_age.tex <==
Age at application&&21.068&&$-$0.090&&0.296&&0.202&&0.287&\\
&&&&(0.089&)&(0.180&)&(0.271&)&(0.183&)\\


==> results/dd_admit_black.tex <==
Black&&0.026&&0.067&\sym{***}&0.012&&$-$0.023&\sym{**}&0.021&\sym{*}\\
&&&&(0.005&)&(0.009&)&(0.011&)&(0.011&)\\


==> results/dd_admit_brown.tex <==
Brown&&0.157&&0.084&\sym{***}&0.010&&$-$0.004&&0.012&\\
&&&&(0.004&)&(0.009&)&(0.012&)&(0.010&)\\


==> results/dd_admit_enrol.tex <==
Enrolled in UERJ&&0.490&&0.008&&$-$0.018&&0.023&&$-$0.049&\\
&&&&(0.017&)&(0.036&)&(0.024&)&(0.050&)\\


==> results/dd_admit_female.tex <==
Female&&0.000&&0.518&\sym{***}&$-$0.032&&$-$0.046&&$-$0.029&\\
&&&&(0.048&)&(0.093&)&(0.092&)&(0.094&)\\


==> results/dd_admit_grad.tex <==
Graduated from UERJ&&0.281&&$-$0.024&\sym{**}&0.010&&0.047&\sym{**}&$-$0.016&\\
&&&&(0.011&)&(0.023&)&(0.021&)&(0.034&)\\


==> results/dd_admit_mean_subj.tex <==
Average score across subject tests&&$-$0.004&&$-$0.025&&0.201&\sym{**}&0.189&\sym{**}&0.285&\sym{**}\\
&&&&(0.047&)&(0.085&)&(0.094&)&(0.109&)\\


==> results/dd_admit_n.tex <==
\(N\) (admits)&&59,630&&136,982&&136,982&&35,881&&101,114&\\


==> results/dd_admit_pct_aa_py.tex <==
Prop.\ of classmates from AA tracks&&0.000&&0.188&\sym{***}&0.074&\sym{***}&0.082&\sym{**}&0.073&\sym{***}\\
&&&&(0.013&)&(0.024&)&(0.036&)&(0.019&)\\


==> results/dd_admit_score_std.tex <==
Admission score (among admits)&&0.000&&$-$0.000&\sym{*}&$-$0.000&&$-$0.142&\sym{**}&0.024&\\
&&&&(0.000&)&(0.000&)&(0.057&)&(0.027&)\\


==> results/dd_admit_std_essay.tex <==
Essay score&&0.000&&$-$0.017&&0.042&&0.099&&0.026&\\
&&&&(0.029&)&(0.057&)&(0.076&)&(0.069&)\\


==> results/dd_admit_wage_index.tex <==
Predicted log wage&&3.242&&$-$0.123&\sym{***}&$-$0.053&\sym{***}&$-$0.036&\sym{***}&$-$0.061&\sym{***}\\
&&&&(0.010&)&(0.012&)&(0.012&)&(0.013&)\\


==> results/dd_admit_wage_index_rais.tex <==
Predicted log wage (if in RAIS)&&3.155&&$-$0.084&\sym{***}&$-$0.069&\sym{***}&$-$0.054&\sym{***}&$-$0.077&\sym{***}\\
&&&&(0.013&)&(0.017&)&(0.016&)&(0.018&)\\


==> results/dd_admit_white.tex <==
White&&0.813&&$-$0.153&\sym{***}&$-$0.024&&0.022&&$-$0.034&\sym{*}\\
&&&&(0.007&)&(0.016&)&(0.020&)&(0.018&)\\


==> results/dd_age.tex <==
Age at application&&21.921&&0.191&&0.794&&0.666&\sym{***}\\
&&&&(0.312&)&(0.899&)&(0.229&)\\


==> results/dd_bio.tex <==
Field biology&&$-$0.000&&$-$0.000&&0.322&&$-$0.111&&0.069&\\
&&&&(0.170&)&(0.236&)&(0.192&)&(0.218&)\\


==> results/dd_black_rais.tex <==
Black&&0.025&&$-$0.005&&$-$0.009&&0.077&\sym{***}\\
&&&&(0.010&)&(0.037&)&(0.012&)\\


==> results/dd_brown_rais.tex <==
Brown&&0.156&&0.000&&&&0.043&\sym{**}\\
&&&&(0.012&)&&&(0.017&)\\


==> results/dd_chem.tex <==
Field chemistry&&$-$0.000&&$-$0.325&\sym{**}&0.000&&0.000&&0.000&\\
&&&&(0.126&)&&&&&&\\


==> results/dd_earn_mean6.tex <==
Monthly earnings (2019 USD)&&1,380.558&&$-$169.838&\sym{***}&$-$28.036&&$-$272.989&\sym{***}\\
&&&&(53.057&)&(100.006&)&(89.500&)\\


==> results/dd_earn_mean6_rob.tex <==
Monthly earnings (2019 USD)&&$-$169.838&\sym{***}&$-$127.202&\sym{**}&$-$164.806&\sym{*}&$-$138.020&\sym{**}&$-$59.327&&$-$167.080&\sym{*}&$-$166.958&\sym{***}\\
&&(53.057&)&(53.273&)&(84.616&)&(56.696&)&(59.432&)&(85.169&)&(59.631&)\\


==> results/dd_enade_age.tex <==
Age&&26.520&&0.661&\sym{**}&0.042&&0.700&\sym{*}\\
&&&&(0.261&)&(0.209&)&(0.361&)\\


==> results/dd_enade_ce.tex <==
Field-specific component&&0.519&&$-$0.037&\sym{***}&$-$0.021&\sym{**}&$-$0.048&\sym{***}\\
&&&&(0.005&)&(0.009&)&(0.006&)\\


==> results/dd_enade_comp_ce.tex <==
Field-specific component&&0.522&&$-$0.020&\sym{***}&$-$0.015&\sym{***}&$-$0.026&\sym{***}\\
&&&&(0.006&)&(0.005&)&(0.006&)\\


==> results/dd_enade_comp_ct.tex <==
\# exam takers&&56.850&&29.212&\sym{***}&36.228&\sym{***}&16.914&\sym{***}\\
&&&&(8.272&)&(4.357&)&(3.398&)\\


==> results/dd_enade_comp_enade.tex <==
Overall score&&0.550&&$-$0.018&\sym{***}&$-$0.014&\sym{***}&$-$0.025&\sym{***}\\
&&&&(0.006&)&(0.005&)&(0.005&)\\


==> results/dd_enade_comp_fg.tex <==
General component&&0.633&&$-$0.014&\sym{**}&$-$0.010&&$-$0.020&\sym{***}\\
&&&&(0.006&)&(0.006&)&(0.005&)\\


==> results/dd_enade_comp_high_inc.tex <==
HH income > 3x min.\ wage&&0.899&&0.059&\sym{***}&0.065&\sym{***}&0.051&\sym{***}\\
&&&&(0.010&)&(0.010&)&(0.010&)\\


==> results/dd_enade_comp_lct.tex <==
Log \# exam takers&&3.859&&0.308&\sym{***}&0.338&\sym{***}&0.243&\sym{***}\\
&&&&(0.068&)&(0.057&)&(0.079&)\\


==> results/dd_enade_ct.tex <==
\# exam takers&&36.086&&4.322&&$-$7.926&\sym{***}&9.142&\sym{***}\\
&&&&(2.664&)&(1.398&)&(1.777&)\\


==> results/dd_enade_dad_hs.tex <==
Father has a HS degree&&0.711&&$-$0.090&\sym{***}&&&$-$0.089&\sym{***}\\
&&&&(0.011&)&(0.010&)&(0.012&)\\


==> results/dd_enade_enade.tex <==
Overall score&&0.553&&$-$0.038&\sym{***}&$-$0.022&\sym{**}&$-$0.051&\sym{***}\\
&&&&(0.005&)&(0.008&)&(0.006&)\\


==> results/dd_enade_fam_inc.tex <==
HH income / minimum wage&&7.724&&$-$1.577&\sym{***}&0.292&&$-$1.873&\sym{***}\\
&&&&(0.098&)&(0.210&)&(0.117&)\\


==> results/dd_enade_female.tex <==
Female&&0.526&&$-$0.005&&$-$0.009&&$-$0.016&\\
&&&&(0.011&)&(0.012&)&(0.011&)\\


==> results/dd_enade_fg.tex <==
General component&&0.657&&$-$0.041&\sym{***}&$-$0.026&\sym{***}&$-$0.059&\sym{***}\\
&&&&(0.005&)&(0.007&)&(0.007&)\\


==> results/dd_enade_fg_hat.tex <==
Predicted general score &&0.563&&$-$0.008&\sym{***}&0.001&\sym{**}&$-$0.007&\sym{***}\\
&&&&(0.001&)&(0.001&)&(0.001&)\\


==> results/dd_enade_high_inc.tex <==
HH income > 3x min.\ wage&&0.899&&$-$0.031&\sym{***}&0.038&\sym{***}&$-$0.058&\sym{***}\\
&&&&(0.010&)&(0.007&)&(0.011&)\\


==> results/dd_enade_hs_priv.tex <==
Private HS student&&0.570&&$-$0.131&\sym{***}&&&$-$0.040&\sym{***}\\
&&&&(0.015&)&&&(0.009&)\\


==> results/dd_enade_lct.tex <==
Log \# exam takers&&3.508&&0.057&&$-$0.430&\sym{***}&0.319&\sym{***}\\
&&&&(0.060&)&(0.077&)&(0.054&)\\


==> results/dd_enade_ltot.tex <==
Log \# graduates&&2.925&&$-$0.454&\sym{***}&0.351&\sym{***}&0.120&\sym{**}\\
&&&&(0.129&)&(0.071&)&(0.051&)\\


==> results/dd_enade_mom_hs.tex <==
Mother has a HS degree&&0.692&&$-$0.086&\sym{***}&0.016&&$-$0.081&\sym{***}\\
&&&&(0.012&)&(0.012&)&(0.012&)\\


==> results/dd_enade_n.tex <==
\(N\) (exam takers)&&1,059&&61,112&&16,851&&37,992&\\


==> results/dd_enade_nprog.tex <==
\(N\) (programs $\times$ years)&&36&&1,664&&1,664&&1,664&\\


==> results/dd_enade_pct_took.tex <==
Prop.\ of graduates taking exam&&0.692&&0.055&\sym{*}&0.008&&$-$0.002&\\
&&&&(0.029&)&(0.025&)&(0.024&)\\


==> results/dd_enade_tot.tex <==
\# graduates&&21.709&&$-$10.757&\sym{**}&17.700&\sym{***}&16.185&\sym{**}\\
&&&&(3.927&)&(5.398&)&(5.719&)\\


==> results/dd_enade_white.tex <==
White&&0.716&&$-$0.132&\sym{***}&&&$-$0.066&\sym{***}\\
&&&&(0.009&)&&&(0.009&)\\


==> results/dd_enade_white_priv.tex <==
White private HS student&&0.440&&$-$0.150&\sym{***}&&&&\\
&&&&(0.014&)&&&&\\


==> results/dd_enrol_age.tex <==
Age at application&&21.871&&$-$0.438&\sym{***}&0.251&&0.946&\sym{***}&0.596&\sym{***}\\
&&&&(0.138&)&(0.277&)&(0.270&)&(0.194&)\\


==> results/dd_enrol_black.tex <==
Black&&0.025&&0.048&\sym{***}&$-$0.017&&0.083&\sym{***}&0.038&\sym{***}\\
&&&&(0.006&)&(0.011&)&(0.017&)&(0.010&)\\


==> results/dd_enrol_brown.tex <==
Brown&&0.156&&0.071&\sym{***}&0.011&&0.053&\sym{***}&0.034&\sym{***}\\
&&&&(0.007&)&(0.013&)&(0.014&)&(0.012&)\\


==> results/dd_enrol_female.tex <==
Female&&0.000&&0.514&\sym{***}&$-$0.042&&$-$0.007&&$-$0.027&\\
&&&&(0.047&)&(0.091&)&(0.077&)&(0.084&)\\


==> results/dd_enrol_grad.tex <==
Graduated from UERJ&&0.570&&$-$0.084&\sym{***}&0.041&\sym{*}&0.036&&0.038&\sym{*}\\
&&&&(0.012&)&(0.021&)&(0.028&)&(0.020&)\\


==> results/dd_enrol_mean_subj.tex <==
Average score across subject tests&&$-$0.004&&0.021&&0.204&\sym{**}&0.064&&0.044&\\
&&&&(0.055&)&(0.095&)&(0.102&)&(0.077&)\\


==> results/dd_enrol_n.tex <==
\(N\) (students)&&16,472&&35,880&&35,880&&30,844&&66,724&\\


==> results/dd_enrol_pct_aa_py.tex <==
Prop.\ of classmates from AA tracks&&0.000&&0.305&\sym{***}&0.196&\sym{***}&0.199&\sym{***}&0.196&\sym{***}\\
&&&&(0.021&)&(0.024&)&(0.024&)&(0.024&)\\


==> results/dd_enrol_score_std.tex <==
Admission score (among admits)&&0.573&&0.082&\sym{***}&$-$0.031&&$-$0.268&\sym{***}&$-$0.110&\sym{**}\\
&&&&(0.030&)&(0.057&)&(0.063&)&(0.047&)\\


==> results/dd_enrol_std_essay.tex <==
Essay score&&$-$0.000&&0.000&&0.073&&$-$0.201&\sym{***}&$-$0.067&\\
&&&&(0.045&)&(0.086&)&(0.073&)&(0.063&)\\


==> results/dd_enrol_wage_index.tex <==
Predicted log wage&&3.196&&$-$0.122&\sym{***}&0.096&\sym{***}&$-$0.000&&0.056&\sym{***}\\
&&&&(0.016&)&(0.024&)&(0.015&)&(0.018&)\\


==> results/dd_enrol_wage_index_rais.tex <==
Predicted log wage (if in RAIS)&&3.123&&$-$0.101&\sym{***}&0.067&\sym{***}&$-$0.013&&0.033&\sym{**}\\
&&&&(0.012&)&(0.020&)&(0.013&)&(0.014&)\\


==> results/dd_enrol_white.tex <==
White&&0.816&&$-$0.121&\sym{***}&0.004&&$-$0.140&\sym{***}&$-$0.076&\sym{***}\\
&&&&(0.010&)&(0.020&)&(0.027&)&(0.018&)\\


==> results/dd_female_any.tex <==
Female&&0.501&&0.032&&0.102&&0.038&\sym{*}\\
&&&&(0.022&)&(0.078&)&(0.021&)\\


==> results/dd_female_rais.tex <==
Female&&0.501&&0.038&&0.101&&0.041&\sym{**}\\
&&&&(0.023&)&(0.079&)&(0.020&)\\


==> results/dd_field_bio.tex <==
Field biology&&0.183&&0.380&\sym{**}&0.000&&0.000&&0.000&\\
&&&&(0.146&)&&&&&&\\


==> results/dd_field_chem.tex <==
Field chemistry&&0.118&&0.074&&0.000&&0.000&&0.000&\\
&&&&(0.130&)&&&&&&\\


==> results/dd_field_forl.tex <==
Field foreign language&&0.196&&0.085&&0.027&&$-$0.144&&$-$0.033&\\
&&&&(0.094&)&(0.148&)&(0.090&)&(0.117&)\\


==> results/dd_field_geo.tex <==
Field geography&&0.048&&0.680&\sym{***}&0.079&&0.057&&$-$0.003&\\
&&&&(0.119&)&(0.121&)&(0.241&)&(0.151&)\\


==> results/dd_field_hist.tex <==
Field history&&0.065&&0.288&\sym{**}&0.180&&$-$0.033&&0.053&\\
&&&&(0.118&)&(0.139&)&(0.119&)&(0.129&)\\


==> results/dd_field_math.tex <==
Field math&&0.158&&0.307&\sym{***}&0.054&&$-$0.133&&$-$0.111&\\
&&&&(0.070&)&(0.099&)&(0.097&)&(0.077&)\\


==> results/dd_field_mean.tex <==
Mean field exam subject score&&0.151&&$-$0.029&&0.039&&$-$0.182&\sym{**}\\
&&&&(0.064&)&(0.121&)&(0.084&)\\


==> results/dd_field_mean2.tex <==
Field mean 2&&0.119&&0.318&\sym{***}&0.064&&$-$0.127&&$-$0.063&\\
&&&&(0.051&)&(0.064&)&(0.076&)&(0.069&)\\


==> results/dd_field_phys.tex <==
Field physics&&0.194&&0.389&\sym{***}&$-$0.200&\sym{*}&$-$0.372&\sym{**}&$-$0.300&\sym{***}\\
&&&&(0.063&)&(0.100&)&(0.149&)&(0.105&)\\


==> results/dd_field_port.tex <==
Field Portuguese&&0.130&&0.087&&$-$0.095&&$-$0.240&\sym{***}&$-$0.151&\\
&&&&(0.087&)&(0.100&)&(0.079&)&(0.099&)\\


==> results/dd_field_writing.tex <==
Field exam writing score&&0.178&&$-$0.045&&0.031&&$-$0.246&\sym{***}\\
&&&&(0.043&)&(0.129&)&(0.046&)\\


==> results/dd_firm_any_alum_aa_coh6.tex <==
Only AA alumni from same cohort&&0.000&&0.036&\sym{***}&0.035&\sym{**}&0.051&\sym{***}\\
&&&&(0.009&)&(0.014&)&(0.007&)\\


==> results/dd_firm_any_alum_aa_diff6.tex <==
Only AA alumni from diff.\ cohort&&0.012&&0.010&\sym{**}&$-$0.017&&0.014&\sym{***}\\
&&&&(0.005&)&(0.022&)&(0.004&)\\


==> results/dd_firm_any_alum_aa_yr10.tex <==
AA track alum in same year&&0.314&&0.045&\sym{**}&0.080&\sym{***}&0.057&\sym{***}\\
&&&&(0.020&)&(0.024&)&(0.019&)\\


==> results/dd_firm_any_alum_aa_yr6.tex <==
AA track alum in same year&&0.215&&0.060&\sym{*}&0.088&\sym{***}&0.071&\sym{**}\\
&&&&(0.034&)&(0.028&)&(0.029&)\\


==> results/dd_firm_any_alum_aa_yr6_field.tex <==
AA track alum in same year&&0.018&&0.024&&0.139&\sym{***}&$-$0.042&\\
&&(0.044&)&(0.078&)&(0.017&)&(0.070&)\\


==> results/dd_firm_any_alum_aa_yr6_rob.tex <==
AA track alum in same year&&0.060&\sym{*}&0.035&&0.096&\sym{***}&0.060&\sym{*}&$-$0.011&&0.100&\sym{***}&0.075&\sym{**}\\
&&(0.034&)&(0.029&)&(0.035&)&(0.032&)&(0.029&)&(0.034&)&(0.028&)\\


==> results/dd_firm_any_alum_coh10.tex <==
Any alum from same cohort&&0.463&&$-$0.063&\sym{**}&$-$0.010&&$-$0.042&\sym{*}\\
&&&&(0.024&)&(0.027&)&(0.022&)\\


==> results/dd_firm_any_alum_coh6.tex <==
Any alum from same cohort&&0.451&&$-$0.062&\sym{***}&$-$0.021&&$-$0.044&\sym{**}\\
&&&&(0.019&)&(0.026&)&(0.019&)\\


==> results/dd_firm_any_alum_coh6_field.tex <==
Any alum from same cohort&&$-$0.015&\sym{*}&$-$0.072&\sym{*}&$-$0.057&\sym{*}&$-$0.106&\sym{**}\\
&&(0.004&)&(0.038&)&(0.030&)&(0.029&)\\


==> results/dd_firm_any_alum_coh6_rob.tex <==
Any alum from same cohort&&$-$0.062&\sym{***}&$-$0.066&\sym{***}&$-$0.052&\sym{**}&$-$0.060&\sym{***}&$-$0.061&\sym{***}&$-$0.046&\sym{*}&$-$0.056&\sym{***}\\
&&(0.019&)&(0.015&)&(0.025&)&(0.020&)&(0.020&)&(0.025&)&(0.021&)\\


==> results/dd_firm_any_alum_gen_coh6.tex <==
General track alumni from same cohort&&0.451&&$-$0.098&\sym{***}&$-$0.118&\sym{*}&$-$0.072&\sym{**}\\
&&&&(0.021&)&(0.068&)&(0.028&)\\


==> results/dd_firm_any_alum_gen_diff6.tex <==
General track alumni from diff.\ cohort&&0.233&&0.042&\sym{**}&0.138&&0.004&\\
&&&&(0.016&)&(0.086&)&(0.017&)\\


==> results/dd_firm_any_alum_gen_yr10.tex <==
General track alum in same year&&0.624&&$-$0.031&&0.004&&$-$0.022&\\
&&&&(0.022&)&(0.024&)&(0.019&)\\


==> results/dd_firm_any_alum_gen_yr6.tex <==
General track alum in same year&&0.577&&$-$0.036&\sym{*}&$-$0.006&&$-$0.029&\\
&&&&(0.019&)&(0.029&)&(0.020&)\\


==> results/dd_firm_any_alum_gen_yr6_field.tex <==
General track alum in same year&&$-$0.095&\sym{***}&$-$0.018&&$-$0.030&&$-$0.072&\sym{*}\\
&&(0.001&)&(0.036&)&(0.031&)&(0.032&)\\


==> results/dd_firm_any_alum_gen_yr6_rob.tex <==
General track alum in same year&&$-$0.036&\sym{*}&$-$0.043&\sym{**}&$-$0.023&&$-$0.031&&$-$0.043&\sym{*}&$-$0.011&&$-$0.040&\sym{*}\\
&&(0.019&)&(0.017&)&(0.020&)&(0.020&)&(0.024&)&(0.021&)&(0.020&)\\


==> results/dd_firm_any_alum_post6.tex <==
Only post-AA alumni&&0.067&&0.049&\sym{**}&0.019&&0.036&\\
&&&&(0.023&)&(0.056&)&(0.023&)\\


==> results/dd_firm_any_alum_pre6.tex <==
Pre-AA alumni&&0.602&&$-$0.055&\sym{**}&$-$0.009&&$-$0.044&\\
&&&&(0.023&)&(0.081&)&(0.033&)\\


==> results/dd_firm_any_alum_pre_priv10.tex <==
Any pre-AA alum (private firms)&&0.232&&$-$0.025&&$-$0.042&&$-$0.035&\\
&&&&(0.026&)&(0.029&)&(0.026&)\\


==> results/dd_firm_any_alum_pre_priv6.tex <==
Any pre-AA alum (private firms)&&0.285&&$-$0.044&\sym{*}&$-$0.071&\sym{**}&$-$0.061&\sym{**}\\
&&&&(0.026&)&(0.031&)&(0.027&)\\


==> results/dd_firm_any_alum_pre_priv6_field.tex <==
Any pre-AA alum (private firms)&&$-$0.045&\sym{*}&$-$0.026&&$-$0.068&&$-$0.054&\\
&&(0.013&)&(0.040&)&(0.044&)&(0.035&)\\


==> results/dd_firm_any_alum_pre_priv6_rob.tex <==
Any pre-AA alum (private firms)&&$-$0.044&\sym{*}&$-$0.050&\sym{**}&$-$0.050&\sym{*}&$-$0.048&\sym{**}&$-$0.013&&$-$0.055&\sym{**}&$-$0.038&\\
&&(0.026&)&(0.021&)&(0.027&)&(0.023&)&(0.020&)&(0.027&)&(0.026&)\\


==> results/dd_firm_any_alum_pre_pub10.tex <==
Any pre-AA alum (public firms)&&0.379&&$-$0.016&&0.021&&$-$0.001&\\
&&&&(0.019&)&(0.024&)&(0.018&)\\


==> results/dd_firm_any_alum_pre_pub6.tex <==
Any pre-AA alum (public firms)&&0.345&&$-$0.014&&0.025&&0.004&\\
&&&&(0.020&)&(0.019&)&(0.016&)\\


==> results/dd_firm_any_alum_pre_pub6_field.tex <==
Any pre-AA alum (public firms)&&$-$0.031&&$-$0.001&&0.010&&$-$0.133&\sym{**}\\
&&(0.013&)&(0.032&)&(0.027&)&(0.039&)\\


==> results/dd_firm_any_alum_pre_pub6_rob.tex <==
Any pre-AA alum (public firms)&&$-$0.014&&$-$0.015&&$-$0.018&&$-$0.006&&$-$0.030&&$-$0.018&&$-$0.027&\\
&&(0.020&)&(0.019&)&(0.029&)&(0.017&)&(0.019&)&(0.028&)&(0.021&)\\


==> results/dd_firm_any_alum_yr10.tex <==
Any alum in same year&&0.634&&$-$0.014&&0.023&&$-$0.004&\\
&&&&(0.021&)&(0.024&)&(0.019&)\\


==> results/dd_firm_any_alum_yr6.tex <==
Any alum in same year&&0.585&&$-$0.017&&0.020&&$-$0.006&\\
&&&&(0.020&)&(0.029&)&(0.021&)\\


==> results/dd_firm_any_alum_yr6_field.tex <==
Any alum in same year&&$-$0.072&\sym{**}&0.007&&$-$0.004&&$-$0.087&\sym{*}\\
&&(0.009&)&(0.036&)&(0.033&)&(0.032&)\\


==> results/dd_firm_any_alum_yr6_rob.tex <==
Any alum in same year&&$-$0.017&&$-$0.031&\sym{*}&$-$0.005&&$-$0.012&&$-$0.034&&0.006&&$-$0.018&\\
&&(0.020&)&(0.016&)&(0.020&)&(0.021&)&(0.023&)&(0.021&)&(0.022&)\\


==> results/dd_firm_p000_aa10.tex <==
Any AA alum&&0.428&&$-$0.022&\sym{**}&0.020&&0.012&&0.037&\\
&&&&(0.009&)&(0.018&)&(0.019&)&(0.025&)\\


==> results/dd_firm_p000_aa6.tex <==
Any AA alum&&0.395&&0.026&\sym{*}&0.033&&0.016&&0.057&\sym{**}\\
&&&&(0.014&)&(0.021&)&(0.022&)&(0.025&)\\


==> results/dd_firm_p000_gen10.tex <==
Any Post-AA general track alum&&0.502&&$-$0.019&\sym{*}&$-$0.002&&$-$0.010&&0.022&\\
&&&&(0.010&)&(0.017&)&(0.017&)&(0.026&)\\


==> results/dd_firm_p000_gen6.tex <==
Any Post-AA general track alum&&0.456&&0.040&\sym{***}&$-$0.009&&$-$0.010&&0.004&\\
&&&&(0.014&)&(0.021&)&(0.020&)&(0.026&)\\


==> results/dd_firm_p000_post10.tex <==
Any Post-AA alum&&0.550&&$-$0.017&\sym{*}&0.008&&0.002&&0.028&\\
&&&&(0.009&)&(0.017&)&(0.018&)&(0.024&)\\


==> results/dd_firm_p000_post6.tex <==
Any Post-AA alum&&0.504&&0.049&\sym{***}&0.007&&0.003&&0.020&\\
&&&&(0.012&)&(0.020&)&(0.019&)&(0.024&)\\


==> results/dd_firm_p000_pre10.tex <==
Firm w/ any pre-AA alum&&0.595&&$-$0.043&&$-$0.023&&$-$0.038&\\
&&&&(0.027&)&(0.034&)&(0.028&)\\


==> results/dd_firm_p000_pre6.tex <==
Firm w/ any pre-AA alum&&0.602&&$-$0.055&\sym{**}&$-$0.044&&$-$0.054&\sym{**}\\
&&&&(0.023&)&(0.033&)&(0.026&)\\


==> results/dd_firm_p000_pre6_rob.tex <==
Firm w/ any pre-AA alum&&$-$0.055&\sym{**}&$-$0.061&\sym{***}&$-$0.072&\sym{***}&$-$0.050&\sym{*}&$-$0.035&\sym{*}&$-$0.064&\sym{**}&$-$0.064&\sym{***}\\
&&(0.023&)&(0.020&)&(0.026&)&(0.025&)&(0.021&)&(0.024&)&(0.021&)\\


==> results/dd_firm_p001_pre10.tex <==
Firm w/ 1 pre-AA alum per 1000 employees&&0.388&&$-$0.043&&$-$0.044&&$-$0.048&\\
&&&&(0.034&)&(0.037&)&(0.033&)\\


==> results/dd_firm_p001_pre6.tex <==
Firm w/ 1 pre-AA alum per 1000 employees&&0.419&&$-$0.050&&$-$0.067&\sym{*}&$-$0.061&\sym{*}\\
&&&&(0.030&)&(0.036&)&(0.031&)\\


==> results/dd_firm_p001_pre6_rob.tex <==
Firm w/ 1 pre-AA alum per 1000 workers&&$-$0.050&&$-$0.054&\sym{**}&$-$0.069&\sym{**}&$-$0.050&\sym{*}&$-$0.029&&$-$0.071&\sym{**}&$-$0.045&\\
&&(0.030&)&(0.026&)&(0.030&)&(0.030&)&(0.034&)&(0.030&)&(0.030&)\\


==> results/dd_firm_p005_pre10.tex <==
Firm w/ 5 pre-AA alumni per 1000 employees&&0.180&&$-$0.041&&$-$0.051&&$-$0.047&\\
&&&&(0.033&)&(0.031&)&(0.030&)\\


==> results/dd_firm_p005_pre6.tex <==
Firm w/ 5 pre-AA alumni per 1000 employees&&0.226&&$-$0.066&\sym{**}&$-$0.057&&$-$0.063&\sym{**}\\
&&&&(0.032&)&(0.035&)&(0.031&)\\


==> results/dd_firm_p005_pre6_rob.tex <==
Firm w/ 5 pre-AA alumni per 1000 workers&&$-$0.066&\sym{**}&$-$0.072&\sym{**}&$-$0.061&\sym{**}&$-$0.067&\sym{**}&$-$0.034&&$-$0.065&\sym{**}&$-$0.048&\\
&&(0.032&)&(0.028&)&(0.029&)&(0.030&)&(0.030&)&(0.028&)&(0.029&)\\


==> results/dd_firm_p010_pre10.tex <==
Firm w/ 10 pre-AA alumni per 1000 employees&&0.113&&$-$0.032&&$-$0.027&&$-$0.031&\\
&&&&(0.030&)&(0.026&)&(0.026&)\\


==> results/dd_firm_p010_pre6.tex <==
Firm w/ 10 pre-AA alumni per 1000 employees&&0.160&&$-$0.051&&$-$0.035&&$-$0.044&\\
&&&&(0.033&)&(0.029&)&(0.029&)\\


==> results/dd_firm_p010_pre6_rob.tex <==
Firm w/ 10 pre-AA alumni per 1000 workers&&$-$0.051&&$-$0.053&\sym{*}&$-$0.040&&$-$0.052&&$-$0.028&&$-$0.048&\sym{*}&$-$0.030&\\
&&(0.033&)&(0.029&)&(0.028&)&(0.031&)&(0.025&)&(0.028&)&(0.028&)\\


==> results/dd_firm_p025_pre10.tex <==
Firm w/ 25 pre-AA alumni per 1000 employees&&0.050&&$-$0.002&&0.007&&0.002&\\
&&&&(0.011&)&(0.012&)&(0.011&)\\


==> results/dd_firm_p025_pre6.tex <==
Firm w/ 25 pre-AA alumni per 1000 employees&&0.078&&$-$0.009&&0.003&&$-$0.004&\\
&&&&(0.016&)&(0.017&)&(0.016&)\\


==> results/dd_firm_p025_pre6_rob.tex <==
Firm w/ 25 pre-AA alumni per 1000 workers&&$-$0.009&&$-$0.019&&0.001&&$-$0.011&&$-$0.009&&$-$0.002&&$-$0.002&\\
&&(0.016&)&(0.013&)&(0.017&)&(0.015&)&(0.013&)&(0.016&)&(0.016&)\\


==> results/dd_firm_p050_pre10.tex <==
Firm w/ 50 pre-AA alumni per 1000 employees&&0.019&&0.003&&0.006&&0.004&\\
&&&&(0.007&)&(0.006&)&(0.006&)\\


==> results/dd_firm_p050_pre6.tex <==
Firm w/ 50 pre-AA alumni per 1000 employees&&0.040&&0.009&&0.013&&0.011&\\
&&&&(0.018&)&(0.014&)&(0.016&)\\


==> results/dd_firm_p050_pre6_rob.tex <==
Firm w/ 50 pre-AA alumni per 1000 workers&&0.009&&0.008&&0.004&&0.008&&0.003&&0.014&&0.014&\\
&&(0.018&)&(0.018&)&(0.013&)&(0.018&)&(0.015&)&(0.016&)&(0.017&)\\


==> results/dd_forl.tex <==
Field foreign language&&0.000&&$-$0.202&&0.061&&$-$0.174&&$-$0.055&\\
&&&&(0.129&)&(0.179&)&(0.111&)&(0.142&)\\


==> results/dd_geo.tex <==
Field geography&&$-$0.000&&0.339&\sym{**}&0.089&&0.109&&$-$0.003&\\
&&&&(0.122&)&(0.125&)&(0.269&)&(0.152&)\\


==> results/dd_grad_by6.tex <==
Graduated from UERJ program&&0.556&&0.013&&0.013&&0.006&\\
&&&&(0.021&)&(0.063&)&(0.028&)\\


==> results/dd_hist.tex <==
Field history&&$-$0.000&&$-$0.067&&0.372&\sym{**}&0.099&&0.163&\\
&&&&(0.114&)&(0.175&)&(0.144&)&(0.122&)\\


==> results/dd_in_rais6.tex <==
Formal employment&&0.734&&$-$0.027&\sym{*}&0.076&&$-$0.012&\\
&&&&(0.015&)&(0.054&)&(0.015&)\\


==> results/dd_large_firm.tex <==
Large firms&&$-$0.028&\sym{***}&$-$0.002&&0.001&&$-$0.024&\sym{***}&$-$0.013&&$-$0.008&\\
&&(0.009&)&(0.016&)&(0.008&)&(0.009&)&(0.016&)&(0.008&)\\


==> results/dd_lest_mean_wage6.tex <==
Firm mean hourly wage (log)&&3.316&&$-$0.095&\sym{**}&$-$0.334&\sym{***}&$-$0.183&\sym{***}\\
&&&&(0.035&)&(0.113&)&(0.051&)\\


==> results/dd_lest_size.tex <==
Log establishment size&&6.704&&$-$0.105&\sym{*}&$-$0.024&&$-$0.118&&$-$0.023&&$-$0.095&\sym{*}\\
&&&&(0.055&)&(0.095&)&(0.093&)&(0.044&)&(0.048&)\\


==> results/dd_lwage6.tex <==
Log hourly wage&&3.245&&$-$0.132&\sym{***}&$-$0.220&\sym{**}&$-$0.212&\sym{***}\\
&&&&(0.045&)&(0.107&)&(0.062&)\\


==> results/dd_male_rais.tex <==
post&&0.499&&$-$0.002&&$-$0.038&&$-$0.041&\sym{**}&$-$0.040&\sym{**}\\
&&&&(0.012&)&(0.023&)&(0.020&)&(0.019&)\\


==> results/dd_math.tex <==
Field math&&0.000&&$-$0.026&&0.175&&$-$0.042&&$-$0.052&\\
&&&&(0.078&)&(0.130&)&(0.127&)&(0.088&)\\


==> results/dd_mean.tex <==
Field mean&&$-$0.000&&$-$0.016&&0.194&\sym{*}&0.032&&0.013&\\
&&&&(0.055&)&(0.100&)&(0.107&)&(0.086&)\\


==> results/dd_n6.tex <==
\(N\) (enrollees)&&16,466&&35,866&&1,631&&30,854&\\


==> results/dd_n_cs.tex <==
\(N\) (students)&&21,378&&45,921&&45,921&&24,553&&45,921&&24,553&\\


==> results/dd_n_panel.tex <==
\(N\) (student/years)&&29,277&&66,720&&66,720&&35,866&&66,720&&35,866&\\


==> results/dd_n_rais.tex <==
\(N\) (wage observations)&&13,388&&17,930&&17,930&&9,669&&17,930&&9,669&\\


==> results/dd_n_wage6.tex <==
\(N\) (wage observations)&&12,062&&26,445&&1,323&&22,975&\\


==> results/dd_other_firm.tex <==
All other small firms&&0.019&\sym{**}&0.005&&0.002&&0.009&&0.009&&0.003&\\
&&(0.007&)&(0.016&)&(0.007&)&(0.007&)&(0.015&)&(0.008&)\\


==> results/dd_pct_aa_py.tex <==
Prop.\ of classmates from AA tracks&&0.000&&0.189&\sym{***}&0.208&\sym{***}&0.192&\sym{***}\\
&&&&(0.017&)&(0.021&)&(0.018&)\\


==> results/dd_peer_any_enrol_aa.tex <==
AA track cohort peer&&0.000&&0.229&\sym{***}&0.002&&$-$0.019&&0.003&&$-$0.010&\\
&&&&(0.021&)&(0.033&)&(0.036&)&(0.016&)&(0.017&)\\


==> results/dd_peer_any_enrol_reg.tex <==
Regular track cohort peer&&0.428&&$-$0.122&\sym{***}&$-$0.075&\sym{***}&$-$0.071&\sym{***}&$-$0.036&\sym{***}&$-$0.035&\sym{***}\\
&&&&(0.013&)&(0.019&)&(0.022&)&(0.009&)&(0.011&)\\


==> results/dd_peer_any_enrol_same.tex <==
Any cohort peer&&0.428&&$-$0.067&\sym{***}&$-$0.031&&$-$0.042&\sym{*}&$-$0.014&&$-$0.020&\sym{*}\\
&&&&(0.010&)&(0.019&)&(0.021&)&(0.010&)&(0.010&)\\


==> results/dd_peer_any_grad_aa10.tex <==
Alum from AA track&&0.314&&0.045&\sym{**}&0.080&\sym{***}&0.057&\sym{***}\\
&&&&(0.020&)&(0.024&)&(0.019&)\\


==> results/dd_peer_any_grad_aa6.tex <==
Alum from AA track&&0.215&&0.060&\sym{*}&0.088&\sym{***}&0.071&\sym{**}\\
&&&&(0.035&)&(0.028&)&(0.029&)\\


==> results/dd_peer_any_grad_aa6_rob.tex <==
Alum from AA track&&0.060&\sym{*}&0.035&&0.096&\sym{***}&0.061&\sym{*}&$-$0.011&&0.100&\sym{***}&0.075&\sym{**}\\
&&(0.035&)&(0.029&)&(0.035&)&(0.033&)&(0.029&)&(0.034&)&(0.028&)\\


==> results/dd_peer_any_grad_any10.tex <==
Any alum&&0.634&&$-$0.014&&0.023&&$-$0.004&\\
&&&&(0.021&)&(0.024&)&(0.019&)\\


==> results/dd_peer_any_grad_any6.tex <==
Any alum&&0.585&&$-$0.017&&0.019&&$-$0.006&\\
&&&&(0.020&)&(0.029&)&(0.021&)\\


==> results/dd_peer_any_grad_any6_rob.tex <==
Any alum&&$-$0.017&&$-$0.031&\sym{*}&$-$0.005&&$-$0.012&&$-$0.035&&0.005&&$-$0.018&\\
&&(0.020&)&(0.016&)&(0.020&)&(0.021&)&(0.023&)&(0.021&)&(0.022&)\\


==> results/dd_peer_any_grad_both10.tex <==
Alum from general track&&0.624&&$-$0.031&&0.004&&$-$0.022&\\
&&&&(0.022&)&(0.024&)&(0.019&)\\


==> results/dd_peer_any_grad_both6.tex <==
Alum from general track&&0.577&&$-$0.036&\sym{*}&$-$0.006&&$-$0.029&\\
&&&&(0.019&)&(0.029&)&(0.020&)\\


==> results/dd_peer_any_grad_both6_rob.tex <==
Alum from general track&&$-$0.036&\sym{*}&$-$0.043&\sym{**}&$-$0.023&&$-$0.031&&$-$0.044&\sym{*}&$-$0.011&&$-$0.040&\sym{*}\\
&&(0.019&)&(0.017&)&(0.020&)&(0.020&)&(0.024&)&(0.021&)&(0.020&)\\


==> results/dd_peer_any_grad_diff10.tex <==
Alum from different cohort&&0.603&&$-$0.071&\sym{***}&$-$0.005&&$-$0.013&&0.019&\\
&&&&(0.008&)&(0.020&)&(0.022&)&(0.025&)\\


==> results/dd_peer_any_grad_diff6.tex <==
Alum from different cohort&&0.546&&$-$0.015&&$-$0.001&&$-$0.018&&0.034&\\
&&&&(0.010&)&(0.022&)&(0.021&)&(0.029&)\\


==> results/dd_peer_any_grad_same10.tex <==
Alum from same cohort&&0.398&&$-$0.059&\sym{**}&$-$0.004&&$-$0.036&\\
&&&&(0.022&)&(0.029&)&(0.022&)\\


==> results/dd_peer_any_grad_same6.tex <==
Alum from same cohort&&0.384&&$-$0.055&\sym{***}&$-$0.020&&$-$0.039&\sym{*}\\
&&&&(0.019&)&(0.026&)&(0.020&)\\


==> results/dd_peer_any_grad_same6_rob.tex <==
Alum from same cohort&&$-$0.055&\sym{***}&$-$0.059&\sym{***}&$-$0.044&\sym{*}&$-$0.053&\sym{**}&$-$0.056&\sym{***}&$-$0.038&&$-$0.048&\sym{**}\\
&&(0.019&)&(0.016&)&(0.024&)&(0.021&)&(0.021&)&(0.024&)&(0.021&)\\


==> results/dd_peer_any_other.tex <==
Admit to program/cohort who didn't enroll&&$-$0.046&\sym{***}&$-$0.034&&$-$0.010&&$-$0.041&\sym{**}&$-$0.058&\sym{*}&$-$0.025&\sym{*}\\
&&(0.014&)&(0.027&)&(0.012&)&(0.016&)&(0.030&)&(0.013&)\\


==> results/dd_peer_any_uerj.tex <==
UERJ enrollee&&$-$0.055&\sym{***}&$-$0.027&&$-$0.010&&$-$0.054&\sym{***}&$-$0.051&\sym{*}&$-$0.022&\sym{*}\\
&&(0.012&)&(0.022&)&(0.010&)&(0.015&)&(0.027&)&(0.013&)\\


==> results/dd_peer_any_uerj_aa.tex <==
UERJ enrollee from AA track&&0.177&\sym{***}&$-$0.013&&$-$0.003&&0.172&\sym{***}&$-$0.032&&$-$0.015&\\
&&(0.021&)&(0.031&)&(0.015&)&(0.023&)&(0.033&)&(0.016&)\\


==> results/dd_peer_any_uerj_next.tex <==
Enrollee in \emph{next} cohort of same program&&$-$0.004&&$-$0.005&&$-$0.004&&$-$0.004&&$-$0.038&\sym{**}&$-$0.022&\sym{***}\\
&&(0.010&)&(0.017&)&(0.008&)&(0.010&)&(0.016&)&(0.007&)\\


==> results/dd_peer_any_uerj_reg.tex <==
UERJ enrollee from regular track&&$-$0.102&\sym{***}&$-$0.061&\sym{**}&$-$0.028&\sym{**}&$-$0.092&\sym{***}&$-$0.071&\sym{**}&$-$0.033&\sym{**}\\
&&(0.014&)&(0.023&)&(0.011&)&(0.016&)&(0.028&)&(0.013&)\\


==> results/dd_phys.tex <==
Field physics&&0.000&&0.196&\sym{***}&$-$0.189&\sym{*}&$-$0.345&\sym{**}&$-$0.293&\sym{***}\\
&&&&(0.063&)&(0.101&)&(0.144&)&(0.097&)\\


==> results/dd_port.tex <==
Field Portuguese&&0.000&&$-$0.299&\sym{**}&$-$0.084&&$-$0.230&\sym{***}&$-$0.179&\sym{*}\\
&&&&(0.134&)&(0.114&)&(0.082&)&(0.102&)\\


==> results/dd_prog_enade_dad_hs.tex <==
Father has a HS degree&&0.754&&$-$0.060&\sym{***}&$-$0.053&&$-$0.045&\sym{***}\\
&&&&(0.018&)&(0.031&)&(0.015&)\\


==> results/dd_prog_enade_high_inc.tex <==
HH income > 3x min.\ wage&&0.916&&$-$0.061&\sym{***}&0.055&\sym{*}&$-$0.106&\sym{***}\\
&&&&(0.018&)&(0.028&)&(0.017&)\\


==> results/dd_prog_enade_lct.tex <==
Log \# exam takers&&3.557&&$-$0.046&&$-$0.356&\sym{***}&$-$0.025&\\
&&&&(0.063&)&(0.096&)&(0.115&)\\


==> results/dd_prog_enade_white_priv.tex <==
White private HS student&&0.464&&$-$0.135&\sym{***}&&&&\\
&&&&(0.019&)&&&&\\


==> results/dd_score.tex <==
Admission score&&0.270&&$-$0.080&&0.034&&$-$0.498&\sym{***}\\
&&&&(0.112&)&(0.160&)&(0.143&)\\


==> results/dd_score_std.tex <==
Admission score (relative to admits)&&0.577&&0.080&\sym{**}&$-$0.054&&$-$0.221&\sym{***}&$-$0.140&\sym{***}\\
&&&&(0.030&)&(0.049&)&(0.073&)&(0.041&)\\


==> results/dd_small_other.tex <==
Small firms w/ other alumni&&0.007&\sym{***}&0.006&&0.003&&0.011&\sym{***}&0.012&&0.007&\sym{*}\\
&&(0.002&)&(0.005&)&(0.002&)&(0.003&)&(0.007&)&(0.004&)\\


==> results/dd_small_uerj.tex <==
Small firms w/ UERJ alumni&&0.001&&$-$0.008&&$-$0.006&&0.004&&$-$0.008&&$-$0.002&\\
&&(0.005&)&(0.008&)&(0.005&)&(0.005&)&(0.009&)&(0.004&)\\


==> results/dd_small_uerj_both.tex <==
Both pre- and post-AA grads&&0.001&&$-$0.005&&$-$0.006&\sym{**}&0.001&&$-$0.005&&$-$0.005&\sym{**}\\
&&(0.003&)&(0.006&)&(0.002&)&(0.003&)&(0.005&)&(0.002&)\\


==> results/dd_small_uerj_post.tex <==
Small firms w/ post-AA UERJ alumni&&0.055&\sym{***}&0.005&&0.002&&0.056&\sym{***}&0.006&&0.006&\\
&&(0.007&)&(0.013&)&(0.006&)&(0.008&)&(0.013&)&(0.007&)\\


==> results/dd_small_uerj_post_only.tex <==
Post-AA grads only&&0.056&\sym{***}&0.023&\sym{*}&0.009&&0.057&\sym{***}&0.024&\sym{*}&0.009&\\
&&(0.006&)&(0.012&)&(0.006&)&(0.007&)&(0.013&)&(0.007&)\\


==> results/dd_small_uerj_pre.tex <==
Small firms w/ pre-AA UERJ alumni&&$-$0.054&\sym{***}&$-$0.017&&$-$0.011&\sym{*}&$-$0.052&\sym{***}&$-$0.018&&$-$0.009&\\
&&(0.007&)&(0.011&)&(0.005&)&(0.008&)&(0.013&)&(0.006&)\\


==> results/dd_small_uerj_pre_only.tex <==
Pre-AA grads only&&$-$0.052&\sym{***}&$-$0.026&\sym{**}&$-$0.007&&$-$0.050&\sym{***}&$-$0.025&\sym{*}&$-$0.007&\\
&&(0.007&)&(0.012&)&(0.005&)&(0.007&)&(0.013&)&(0.005&)\\


==> results/dd_subjs.tex <==
Field subject mean&&0.000&&$-$0.007&&0.268&\sym{*}&0.021&&0.109&\\
&&&&(0.077&)&(0.148&)&(0.138&)&(0.136&)\\


==> results/dd_wage_index.tex <==
Predicted log wage&&3.298&&$-$0.023&&$-$0.011&&$-$0.161&\sym{***}\\
&&&&(0.029&)&(0.049&)&(0.043&)\\


==> results/dd_wage_index_rais.tex <==
Predicted log wage (if in RAIS)&&3.251&&$-$0.033&&$-$0.009&&$-$0.154&\sym{***}\\
&&&&(0.028&)&(0.053&)&(0.043&)\\


==> results/dd_white_rais.tex <==
White&&0.810&&0.013&&&&$-$0.121&\sym{***}\\
&&&&(0.018&)&&&(0.025&)\\


==> results/dd_writing.tex <==
Field writing&&0.000&&0.000&&0.086&&$-$0.188&\sym{**}&$-$0.066&\\
&&&&(0.045&)&(0.072&)&(0.070&)&(0.061&)\\


==> results/enrol_censo_1153.tex <==
censo1153&&&&&&1.090&&$-$0.002&&1.112&&$-$0.182&\sym{**}\\
&&&&&&&&(0.031&)&&&(0.083&)\\


==> results/enrol_censo_16.tex <==
censo16&&&&&&0.769&&$-$0.018&&0.809&&$-$0.120&\\
&&&&&&&&(0.023&)&&&(0.074&)\\


==> results/enrol_censo_165.tex <==
censo165&&&&&&1.041&&$-$0.054&\sym{*}&0.870&&$-$0.050&\\
&&&&&&&&(0.031&)&&&(0.070&)\\


==> results/enrol_censo_176.tex <==
censo176&&&&&&0.750&&$-$0.026&&0.767&&0.036&\\
&&&&&&&&(0.023&)&&&(0.069&)\\


==> results/enrol_censo_663.tex <==
censo663&&&&&&1.460&&0.046&&1.623&&$-$0.089&\\
&&&&&&&&(0.033&)&&&(0.114&)\\


==> results/enrol_censo_any.tex <==
censoany&&&&&&29.623&&$-$0.466&\sym{*}&24.963&&1.149&\sym{*}\\
&&&&&&&&(0.253&)&&&(0.603&)\\


==> results/enrol_censo_centro.tex <==
censocentro&&&&&&3.820&&$-$0.069&&3.679&&0.017&\\
&&&&&&&&(0.059&)&&&(0.159&)\\


==> results/enrol_censo_comp.tex <==
Enrolled in a Top 5 UERJ competitor&&$-$0.489&\sym{***}&0.248&&0.030&&0.117&\\
&&(0.151&)&(0.411&)&(0.453&)&(0.300&)\\


==> results/enrol_censo_comp9.tex <==
Enrolled in a Top 9 UERJ competitor&&$-$0.507&\sym{***}&$-$0.032&&0.118&&$-$0.009&\\
&&(0.194&)&(0.513&)&(0.580&)&(0.380&)\\


==> results/enrol_censo_comp9_grad.tex <==
Graduated from a Top 9 UERJ competitor&&$-$0.190&\sym{*}&$-$0.171&&0.497&&0.101&\\
&&(0.105&)&(0.297&)&(0.328&)&(0.218&)\\


==> results/enrol_censo_comp_grad.tex <==
Graduated from a Top 5 UERJ competitor&&$-$0.135&&$-$0.154&&0.289&&0.023&\\
&&(0.084&)&(0.235&)&(0.260&)&(0.172&)\\


==> results/enrol_censo_comp_priv.tex <==
Enrolled in UERJ private competitor&&$-$0.153&\sym{*}&0.231&&0.168&&0.174&\\
&&(0.083&)&(0.246&)&(0.283&)&(0.183&)\\


==> results/enrol_censo_comp_priv_grad.tex <==
Graduated from UERJ private competitor&&$-$0.009&&0.111&&0.112&&0.105&\\
&&(0.047&)&(0.138&)&(0.152&)&(0.101&)\\


==> results/enrol_censo_comp_pub.tex <==
Enrolled in UERJ public competitor&&$-$0.339&\sym{***}&$-$0.000&&0.053&&0.012&\\
&&(0.119&)&(0.324&)&(0.339&)&(0.232&)\\


==> results/enrol_censo_comp_pub_grad.tex <==
Graduated from UERJ public competitor&&$-$0.131&\sym{*}&$-$0.212&&0.322&&0.011&\\
&&(0.070&)&(0.197&)&(0.215&)&(0.143&)\\


==> results/enrol_censo_fac.tex <==
censofac&&&&&&3.979&&$-$0.049&&3.321&&0.156&\\
&&&&&&&&(0.062&)&&&(0.135&)\\


==> results/enrol_censo_fed.tex <==
Enrolled in a Federal Univ.\ in RJ&&$-$0.338&\sym{***}&$-$0.012&&0.055&&0.008&\\
&&(0.119&)&(0.327&)&(0.343&)&(0.233&)\\


==> results/enrol_censo_fed_grad.tex <==
Graduated from a Federal Univ.\ in RJ&&$-$0.215&\sym{***}&$-$0.026&&0.280&&0.096&\\
&&(0.079&)&(0.226&)&(0.248&)&(0.164&)\\


==> results/enrol_censo_oth_fed.tex <==
\# enrolled in other federal universities&&&&&&4.407&&$-$0.165&\sym{**}&3.181&&0.041&\\
&&&&&&&&(0.083&)&&&(0.168&)\\


==> results/enrol_censo_oth_fed_grad.tex <==
Graduated from another federal university&&$-$0.086&&0.115&\\
&&(0.055&)&(0.118&)\\


==> results/enrol_censo_oth_priv.tex <==
\# enrolled in other private universities&&&&&&5.110&&$-$0.041&&5.181&&$-$0.457&\sym{**}\\
&&&&&&&&(0.062&)&&&(0.229&)\\


==> results/enrol_censo_oth_priv_grad.tex <==
Graduated from a lower-ranked private university&&0.010&&$-$0.125&\\
&&(0.045&)&(0.115&)\\


==> results/enrol_censo_priv_oth.tex <==
Enrolled in any other private univ.\ in RJ&&$-$0.003&&$-$0.482&\sym{*}&$-$0.518&\sym{*}&$-$0.476&\sym{**}\\
&&(0.084&)&(0.286&)&(0.313&)&(0.208&)\\


==> results/enrol_censo_priv_oth_grad.tex <==
Graduated from any other private univ.\ in RJ&&$-$0.010&&$-$0.101&&$-$0.204&&$-$0.137&\\
&&(0.044&)&(0.152&)&(0.167&)&(0.111&)\\


==> results/enrol_censo_priv_top.tex <==
Enrolled in a top private univ.\ in RJ&&$-$0.153&\sym{*}&0.233&&0.168&&0.169&\\
&&(0.083&)&(0.247&)&(0.286&)&(0.184&)\\


==> results/enrol_censo_priv_top_grad.tex <==
Graduated from a top private univ.\ in RJ&&$-$0.034&&$-$0.030&&0.091&&0.019&\\
&&(0.052&)&(0.157&)&(0.171&)&(0.114&)\\


==> results/enrol_censo_pucrio.tex <==
Enrolled in PUC Rio&&$-$0.003&&$-$0.017&&0.193&\sym{**}&0.071&\\
&&(0.038&)&(0.105&)&(0.099&)&(0.072&)\\


==> results/enrol_censo_pucrio_grad.tex <==
Graduated from PUC Rio&&$-$0.012&&$-$0.030&&0.115&&0.035&\\
&&(0.029&)&(0.082&)&(0.076&)&(0.056&)\\


==> results/enrol_censo_rj.tex <==
Enrolled in any univ.\ in RJ&&$-$0.231&&0.325&&1.081&&0.650&\\
&&(0.222&)&(0.615&)&(0.691&)&(0.453&)\\


==> results/enrol_censo_rj_grad.tex <==
Graduated from any univ.\ in RJ&&$-$0.106&&0.223&&0.905&\sym{**}&0.517&\sym{*}\\
&&(0.132&)&(0.389&)&(0.427&)&(0.284&)\\


==> results/enrol_censo_top_priv.tex <==
\# enrolled in a top-100 private university&&&&&&5.154&&$-$0.176&\sym{**}&4.312&&0.147&\\
&&&&&&&&(0.077&)&&&(0.164&)\\


==> results/enrol_censo_top_priv_grad.tex <==
Graduated from a top-100 private univerity&&$-$0.049&&$-$0.001&\\
&&(0.053&)&(0.118&)\\


==> results/enrol_censo_uerj.tex <==
\# enrolled in UERJ&&&&&&1.465&&0.271&\sym{***}&1.051&&0.880&\sym{***}\\
&&&&&&&&(0.037&)&&&(0.088&)\\


==> results/enrol_censo_uerj_grad.tex <==
Graduated from UERJ (higher ed.\ census)&&0.153&\sym{***}&0.434&\sym{***}\\
&&(0.029&)&(0.067&)\\


==> results/enrol_censo_uff.tex <==
censouff&&&&&&2.620&&$-$0.084&&1.833&&0.019&\\
&&&&&&&&(0.054&)&&&(0.121&)\\


==> results/enrol_censo_uff_grad.tex <==
Graduated from UFF&&$-$0.061&&0.049&&0.091&&0.062&\\
&&(0.044&)&(0.132&)&(0.134&)&(0.093&)\\


==> results/enrol_censo_ufrj.tex <==
\# enrolled in UFRJ&&&&&&3.369&&$-$0.147&\sym{***}&2.381&&$-$0.111&\\
&&&&&&&&(0.057&)&&&(0.137&)\\


==> results/enrol_censo_ufrj_grad.tex <==
Graduated from UFRJ&&$-$0.124&\sym{**}&$-$0.090&\\
&&(0.049&)&(0.102&)\\


==> results/enrol_censo_ufrrj.tex <==
censoufrrj&&&&&&1.021&&$-$0.058&\sym{*}&0.726&&0.098&\\
&&&&&&&&(0.035&)&&&(0.069&)\\


==> results/enrol_censo_unesa.tex <==
censounesa&&&&&&4.050&&$-$0.157&\sym{**}&3.740&&0.059&\\
&&&&&&&&(0.065&)&&&(0.147&)\\


==> results/enrol_censo_unesa_grad.tex <==
Graduated from UNESA&&$-$0.022&&0.001&&$-$0.024&&$-$0.017&\\
&&(0.042&)&(0.135&)&(0.148&)&(0.098&)\\


==> results/enrol_censo_unigranrio.tex <==
Enrolled in Unigranrio&&0.000&&0.000&&0.000&&0.000&\\
&&&&&&&&&\\


==> results/enrol_censo_unigranrio_grad.tex <==
Graduated from Unigranrio&&0.000&&0.000&&0.000&&0.000&\\
&&&&&&&&&\\


==> results/enrol_censo_unirio.tex <==
censounirio&&&&&&0.766&&$-$0.029&&0.623&&$-$0.027&\\
&&&&&&&&(0.024&)&&&(0.053&)\\


==> results/enrol_censo_univ.tex <==
censouniv&&&&&&21.824&&$-$0.410&\sym{**}&17.963&&0.736&\\
&&&&&&&&(0.203&)&&&(0.476&)\\


==> results/enrol_censo_universo.tex <==
Enrolled in Universo&&0.050&&$-$0.031&&$-$0.281&\sym{*}&$-$0.136&\\
&&(0.041&)&(0.143&)&(0.146&)&(0.102&)\\


==> results/enrol_censo_universo_grad.tex <==
Graduated from Universo&&0.043&\sym{*}&$-$0.007&&$-$0.119&&$-$0.050&\\
&&(0.026&)&(0.086&)&(0.102&)&(0.065&)\\


==> results/enrol_college_any.tex <==
Enrolled in any college (RAIS data)&&0.010&&$-$0.068&\\
&&(0.021&)&(0.055&)\\


==> results/enrol_college_degree.tex <==
Graduated from any college(RAIS data)&&0.005&&$-$0.063&\\
&&(0.020&)&(0.050&)\\


==> results/enrol_enrol.tex <==
Enrolled in UERJ program (UERJ data)&&0.277&\sym{***}&0.724&\sym{***}\\
&&(0.010&)&(0.022&)\\


==> results/enrol_grad.tex <==
Graduated from UERJ program (UERJ data)&&0.189&\sym{***}&0.474&\sym{***}\\
&&(0.009&)&(0.025&)\\


==> results/enrol_n.tex <==
\(N\) (\# enrolled in UERJ)&&&&&&1,553&&19,895&&215&&2,757&\\


==> results/enrol_same_prog_area.tex <==
\# enrolled in same progam area (1-dig)&&&&&&6.378&&0.149&\sym{*}&5.958&&0.455&\sym{**}\\
&&&&&&&&(0.089&)&&&(0.219&)\\


==> results/enrol_same_prog_area2.tex <==
\# enrolled in same progam area (2-dig)&&&&&&3.448&&0.120&\sym{**}&2.647&&0.351&\sym{**}\\
&&&&&&&&(0.059&)&&&(0.138&)\\


==> results/enrol_same_prog_area3.tex <==
\# enrolled in same progam area (3-dig)&&&&&&1.661&&0.192&\sym{***}&1.367&&0.459&\sym{***}\\
&&&&&&&&(0.040&)&&&(0.082&)\\


==> results/enrol_topsame_prog_area.tex <==
\# enrolled in same progam area (1-dig)&&&&&&7.525&&0.440&\sym{**}&6.616&&0.593&\\
&&&&&&&&(0.213&)&&&(0.406&)\\


==> results/enrol_topsame_prog_area2.tex <==
\# enrolled in same progam area (2-dig)&&&&&&4.663&&0.370&\sym{**}&2.907&&0.647&\sym{**}\\
&&&&&&&&(0.154&)&&&(0.276&)\\


==> results/enrol_topsame_prog_area3.tex <==
\# enrolled in same progam area (3-dig)&&&&&&2.433&&0.320&\sym{***}&1.837&&0.459&\sym{**}\\
&&&&&&&&(0.105&)&&&(0.179&)\\


==> results/firm_n.tex <==
\(N\)&&7,959&&81,928&&5,507&&77,857&&848&&13,835&\\


==> results/firm_p000_aa.tex <==
Any AA track alum (2004--2011 cohorts)&&0.319&&0.060&\sym{*}&0.338&&0.106&\sym{***}&0.323&&0.097&\sym{**}\\
&&&&(0.031&)&&&(0.035&)&&&(0.041&)\\


==> results/firm_p000_both.tex <==
Both pre- and post-AA alumni&&0.324&&0.011&&0.223&&$-$0.021&&0.226&&0.038&\\
&&&&(0.030&)&&&(0.034&)&&&(0.044&)\\


==> results/firm_p000_other.tex <==
Firm w/ only UERJ decliners&&0.103&&$-$0.007&&0.124&&$-$0.004&&0.071&&$-$0.006&\\
&&&&(0.022&)&&&(0.027&)&&&(0.024&)\\


==> results/firm_p000_post.tex <==
Post-AA alumni only&&0.093&&0.027&&0.220&&0.074&\sym{**}&0.172&&0.019&\\
&&&&(0.020&)&&&(0.035&)&&&(0.039&)\\


==> results/firm_p000_postB.tex <==
Any post-AA alum (bottom half)&&0.331&&0.074&\sym{**}&0.362&&0.089&\sym{**}&0.334&&0.112&\sym{***}\\
&&&&(0.031&)&&&(0.036&)&&&(0.041&)\\


==> results/firm_p000_postT.tex <==
Any post-AA alum (top half)&&0.331&&0.067&\sym{**}&0.362&&0.122&\sym{***}&0.289&&0.059&\\
&&&&(0.032&)&&&(0.035&)&&&(0.040&)\\


==> results/firm_p000_pre.tex <==
Pre-AA alumni only&&0.122&&0.020&&0.060&&$-$0.008&&0.040&&$-$0.007&\\
&&&&(0.024&)&&&(0.018&)&&&(0.024&)\\


==> results/firm_p000_preB.tex <==
Any pre-AA alum (bottom half)&&0.423&&0.088&\sym{***}&0.259&&0.077&\sym{**}&0.254&&0.054&\\
&&&&(0.033&)&&&(0.033&)&&&(0.038&)\\


==> results/firm_p000_preT.tex <==
Any pre-AA alum (top half)&&0.434&&0.060&\sym{*}&0.263&&0.021&&0.263&&0.028&\\
&&&&(0.033&)&&&(0.033&)&&&(0.038&)\\


==> results/firm_p000_uerj.tex <==
Firm w/ any alum&&0.506&&0.057&&0.458&&0.059&&0.397&&0.089&\sym{**}\\
&&&&(0.036&)&&&(0.037&)&&&(0.042&)\\


==> results/firm_p000_uerj_after.tex <==
Any alum (hired after)&&0.278&&0.030&&0.108&&0.014&&0.097&&0.043&\sym{*}\\
&&&&(0.028&)&&&(0.020&)&&&(0.025&)\\


==> results/firm_p000_uerj_before.tex <==
Any alum (hired before)&&0.168&&0.057&\sym{**}&0.303&&0.077&\sym{**}&0.245&&0.062&\sym{*}\\
&&&&(0.025&)&&&(0.030&)&&&(0.034&)\\


==> results/firm_p001_aa.tex <==
1 AA track alum (2004--2011 cohorts)&&0.119&&0.047&\sym{**}&0.198&&0.124&\sym{***}&0.100&&0.124&\sym{***}\\
&&&&(0.022&)&&&(0.029&)&&&(0.030&)\\


==> results/firm_p001_both.tex <==
1 alum (both)&&0.149&&0.097&\sym{***}&0.115&&0.040&&0.063&&0.037&\sym{*}\\
&&&&(0.028&)&&&(0.028&)&&&(0.019&)\\


==> results/firm_p001_other.tex <==
1 alum per 1000 employees&&0.102&&$-$0.012&&0.144&&0.008&&0.089&&0.014&\\
&&&&(0.021&)&&&(0.028&)&&&(0.025&)\\


==> results/firm_p001_post.tex <==
1 post-AA alum (only)&&0.061&&$-$0.002&&0.203&&0.094&\sym{***}&0.111&&0.050&\\
&&&&(0.021&)&&&(0.030&)&&&(0.032&)\\


==> results/firm_p001_postB.tex <==
1 post-AA alum (bottom half)&&0.139&&0.050&\sym{**}&0.224&&0.114&\sym{***}&0.117&&0.123&\sym{***}\\
&&&&(0.023&)&&&(0.030&)&&&(0.031&)\\


==> results/firm_p001_postT.tex <==
1 post-AA alum (top half)&&0.146&&0.076&\sym{***}&0.235&&0.101&\sym{***}&0.117&&0.072&\sym{**}\\
&&&&(0.024&)&&&(0.030&)&&&(0.029&)\\


==> results/firm_p001_pre.tex <==
1 pre-AA alum (only)&&0.191&&0.045&\sym{*}&0.073&&$-$0.000&&0.057&&0.016&\\
&&&&(0.026&)&&&(0.019&)&&&(0.021&)\\


==> results/firm_p001_preB.tex <==
1 pre-AA alum (bottom half)&&0.226&&0.095&\sym{***}&0.125&&0.065&\sym{***}&0.057&&0.061&\sym{***}\\
&&&&(0.027&)&&&(0.024&)&&&(0.023&)\\


==> results/firm_p001_preT.tex <==
1 pre-AA alum (top half)&&0.239&&0.075&\sym{***}&0.136&&0.030&&0.074&&0.027&\\
&&&&(0.027&)&&&(0.025&)&&&(0.024&)\\


==> results/firm_p001_uerj.tex <==
Firm w/ 1 alum per 1000 employees&&0.319&&0.056&\sym{**}&0.301&&0.075&\sym{**}&0.213&&0.053&\\
&&&&(0.028&)&&&(0.034&)&&&(0.041&)\\


==> results/firm_p005_aa.tex <==
5 AA track alumni (2004--2011 cohorts)&&0.038&&0.009&&0.078&&0.076&\sym{***}&0.043&&0.066&\sym{***}\\
&&&&(0.013&)&&&(0.021&)&&&(0.022&)\\


==> results/firm_p005_both.tex <==
5 alumni (both)&&0.057&&0.055&\sym{***}&0.044&&0.036&\sym{**}&0.023&&0.026&\sym{**}\\
&&&&(0.018&)&&&(0.018&)&&&(0.013&)\\


==> results/firm_p005_other.tex <==
5 alumni per 1000 employees&&0.067&&0.001&&0.104&&$-$0.014&&0.031&&0.036&\sym{*}\\
&&&&(0.018&)&&&(0.024&)&&&(0.019&)\\


==> results/firm_p005_post.tex <==
5 post-AA alumni (only)&&0.034&&0.011&&0.124&&0.089&\sym{***}&0.057&&0.047&\sym{*}\\
&&&&(0.011&)&&&(0.024&)&&&(0.026&)\\


==> results/firm_p005_postB.tex <==
5 post-AA alumni (bottom half)&&0.044&&0.013&&0.090&&0.085&\sym{***}&0.051&&0.057&\sym{**}\\
&&&&(0.014&)&&&(0.023&)&&&(0.023&)\\


==> results/firm_p005_postT.tex <==
5 post-AA alumni (top half)&&0.057&&0.046&\sym{***}&0.096&&0.102&\sym{***}&0.040&&0.032&\\
&&&&(0.016&)&&&(0.023&)&&&(0.020&)\\


==> results/firm_p005_pre.tex <==
5 pre-AA alumni (only)&&0.143&&0.027&&0.057&&0.014&&0.029&&0.025&\sym{*}\\
&&&&(0.025&)&&&(0.018&)&&&(0.014&)\\


==> results/firm_p005_preB.tex <==
5 pre-AA alumni (bottom half)&&0.106&&0.085&\sym{***}&0.047&&0.054&\sym{***}&0.026&&0.005&\\
&&&&(0.021&)&&&(0.017&)&&&(0.016&)\\


==> results/firm_p005_preT.tex <==
5 pre-AA alumni (top half)&&0.124&&0.059&\sym{***}&0.060&&0.023&&0.031&&0.028&\\
&&&&(0.021&)&&&(0.018&)&&&(0.017&)\\


==> results/firm_p005_uerj.tex <==
Firm w/ 5 alumni per 1000 employees&&0.149&&0.052&\sym{**}&0.128&&0.074&\sym{**}&0.083&&0.009&\\
&&&&(0.023&)&&&(0.029&)&&&(0.027&)\\


==> results/firm_p010_aa.tex <==
10 AA track alumni (2004--2011 cohorts)&&0.017&&0.008&&0.039&&0.046&\sym{***}&0.023&&0.031&\sym{*}\\
&&&&(0.009&)&&&(0.016&)&&&(0.017&)\\


==> results/firm_p010_both.tex <==
10 alumni (both)&&0.030&&0.034&\sym{***}&0.028&&0.037&\sym{***}&0.011&&0.022&\sym{**}\\
&&&&(0.010&)&&&(0.013&)&&&(0.011&)\\


==> results/firm_p010_other.tex <==
10 alumni per 1000 employees&&0.060&&$-$0.020&&0.069&&0.020&&0.026&&0.016&\\
&&&&(0.016&)&&&(0.021&)&&&(0.015&)\\


==> results/firm_p010_post.tex <==
10 post-AA alumni (only)&&0.024&&0.011&&0.076&&0.071&\sym{***}&0.043&&0.014&\\
&&&&(0.009&)&&&(0.020&)&&&(0.022&)\\


==> results/firm_p010_postB.tex <==
10 post-AA alumni (bottom half)&&0.021&&0.009&&0.048&&0.060&\sym{***}&0.034&&0.031&\sym{*}\\
&&&&(0.011&)&&&(0.018&)&&&(0.018&)\\


==> results/firm_p010_postT.tex <==
10 post-AA alumni (top half)&&0.030&&0.012&&0.043&&0.071&\sym{***}&0.029&&0.022&\\
&&&&(0.012&)&&&(0.018&)&&&(0.016&)\\


==> results/firm_p010_pre.tex <==
10 pre-AA alumni (only)&&0.103&&0.026&&0.033&&$-$0.005&&0.011&&0.015&\\
&&&&(0.018&)&&&(0.015&)&&&(0.010&)\\


==> results/firm_p010_preB.tex <==
10 pre-AA alumni (bottom half)&&0.049&&0.061&\sym{***}&0.022&&0.036&\sym{***}&0.009&&0.005&\\
&&&&(0.015&)&&&(0.012&)&&&(0.010&)\\


==> results/firm_p010_preT.tex <==
10 pre-AA alumni (top half)&&0.059&&0.035&\sym{**}&0.035&&0.002&&0.006&&0.023&\sym{**}\\
&&&&(0.016&)&&&(0.014&)&&&(0.011&)\\


==> results/firm_p010_uerj.tex <==
Firm w/ 10 alumni per 1000 employees&&0.094&&0.026&&0.072&&0.033&&0.051&&$-$0.005&\\
&&&&(0.018&)&&&(0.024&)&&&(0.018&)\\


==> results/firm_p025_aa.tex <==
25 AA track alumni (2004--2011 cohorts)&&0.008&&0.007&&0.013&&0.023&\sym{**}&0.003&&0.012&\\
&&&&(0.007&)&&&(0.010&)&&&(0.010&)\\


==> results/firm_p025_both.tex <==
25 alumni (both)&&0.008&&0.012&\sym{*}&0.009&&0.001&&0.006&&0.012&\sym{*}\\
&&&&(0.006&)&&&(0.006&)&&&(0.007&)\\


==> results/firm_p025_other.tex <==
25 alumni per 1000 employees&&0.041&&$-$0.004&&0.031&&0.024&&0.014&&0.008&\\
&&&&(0.013&)&&&(0.016&)&&&(0.011&)\\


==> results/firm_p025_post.tex <==
25 post-AA alumni (only)&&0.013&&0.003&&0.030&&0.060&\sym{***}&0.020&&0.008&\\
&&&&(0.007&)&&&(0.015&)&&&(0.014&)\\


==> results/firm_p025_postB.tex <==
25 post-AA alumni (bottom half)&&0.008&&0.010&&0.015&&0.036&\sym{***}&0.009&&0.010&\\
&&&&(0.007&)&&&(0.011&)&&&(0.011&)\\


==> results/firm_p025_postT.tex <==
25 post-AA alumni (top half)&&0.012&&0.003&&0.016&&0.018&&0.017&&$-$0.005&\\
&&&&(0.007&)&&&(0.011&)&&&(0.010&)\\


==> results/firm_p025_pre.tex <==
25 pre-AA alumni (only)&&0.036&&0.024&\sym{*}&0.015&&$-$0.002&&0.003&&$-$0.002&\\
&&&&(0.013&)&&&(0.009&)&&&(0.006&)\\


==> results/firm_p025_preB.tex <==
25 pre-AA alumni (bottom half)&&0.013&&0.025&\sym{***}&0.006&&0.002&&0.003&&0.005&\\
&&&&(0.009&)&&&(0.006&)&&&(0.007&)\\


==> results/firm_p025_preT.tex <==
25 pre-AA alumni (top half)&&0.017&&0.025&\sym{**}&0.012&&$-$0.003&&0.000&&0.011&\\
&&&&(0.010&)&&&(0.008&)&&&(0.007&)\\


==> results/firm_p025_uerj.tex <==
Firm w/ 25 alumni per 1000 employees&&0.031&&0.011&&0.023&&0.040&\sym{***}&0.013&&$-$0.002&\\
&&&&(0.011&)&&&(0.012&)&&&(0.011&)\\


==> results/firm_p050_aa.tex <==
50 AA track alumni (2004--2011 cohorts)&&0.003&&$-$0.002&&0.004&&0.013&\sym{**}&0.000&&0.007&\\
&&&&(0.004&)&&&(0.006&)&&&(0.007&)\\


==> results/firm_p050_both.tex <==
50 alumni (both)&&0.002&&0.005&&0.003&&0.005&&0.000&&0.008&\sym{*}\\
&&&&(0.003&)&&&(0.004&)&&&(0.004&)\\


==> results/firm_p050_other.tex <==
50 alumni per 1000 employees&&0.022&&$-$0.007&&0.017&&0.013&&0.014&&$-$0.003&\\
&&&&(0.009&)&&&(0.012&)&&&(0.009&)\\


==> results/firm_p050_post.tex <==
50 post-AA alumni (only)&&0.007&&$-$0.004&&0.013&&0.023&\sym{***}&0.009&&$-$0.001&\\
&&&&(0.006&)&&&(0.009&)&&&(0.009&)\\


==> results/firm_p050_postB.tex <==
50 post-AA alumni (bottom half)&&0.004&&$-$0.002&&0.005&&0.021&\sym{***}&0.000&&0.010&\\
&&&&(0.005&)&&&(0.007&)&&&(0.008&)\\


==> results/firm_p050_postT.tex <==
50 post-AA alumni (top half)&&0.004&&0.002&&0.007&&0.012&&0.003&&0.006&\\
&&&&(0.005&)&&&(0.008&)&&&(0.006&)\\


==> results/firm_p050_pre.tex <==
50 pre-AA alumni (only)&&0.010&&0.022&\sym{**}&0.005&&$-$0.004&&0.000&&0.001&\\
&&&&(0.009&)&&&(0.004&)&&&(0.004&)\\


==> results/firm_p050_preB.tex <==
50 pre-AA alumni (bottom half)&&0.006&&0.010&\sym{*}&0.003&&0.004&&0.000&&0.010&\sym{*}\\
&&&&(0.006&)&&&(0.004&)&&&(0.005&)\\


==> results/firm_p050_preT.tex <==
50 pre-AA alumni (top half)&&0.007&&0.015&\sym{**}&0.005&&$-$0.003&&0.000&&0.005&\\
&&&&(0.006&)&&&(0.005&)&&&(0.005&)\\


==> results/firm_p050_uerj.tex <==
Firm w/ 50 alumni per 1000 employees&&0.004&&0.007&&0.003&&0.005&&0.004&&$-$0.014&\\
&&&&(0.005&)&&&(0.006&)&&&(0.009&)\\


==> results/firm_summ.tex <==
Any UERJ alum &2,635 &395 &2,152 &0.78 &0.43 &0.53 &12.97 \\
\quad 00--01 alumni per 1000 employees &1,087 &72 &12,029 &0.66 &0.75 &0.46 &11.11 \\
\quad 01--05 alumni per 1000 employees &835 &98 &1,468 &0.77 &0.33 &0.52 &13.04 \\
\quad 05--10 alumni per 1000 employees &430 &47 &960 &0.87 &0.28 &0.60 &15.89 \\
\quad 10--25 alumni per 1000 employees &419 &65 &463 &0.91 &0.11 &0.61 &14.52 \\
\quad 25--50 alumni per 1000 employees &192 &46 &212 &0.93 &0.24 &0.64 &17.02 \\
\quad 50+ alumni per 1000 employees &152 &67 &25 &0.86 &0.05 &0.57 &9.13 \\\midrule
No UERJ alumni &4,185 &4,238 &126 &0.65 &0.15 &0.39 &8.90 \\
\quad UERJ admits who declined &1,110 &555 &475 &0.68 &0.24 &0.50 &12.00 \\
\quad All other firms &3,344 &3,683 &84 &0.64 &0.13 &0.35 &7.96 \\\midrule
All firms &6,101 &4,633 &450 &0.70 &0.26 &0.44 &10.51 \\


==> results/firm_top10_all.tex <==
1& Rio de Janeiro City Hall &4,639 &24 &88,982 &Yes &Yes &0.50 &9.22 \\
2& State Secretary of Education &3,866 &24 &90,557 &Yes &Yes &0.43 &4.75 \\
3& Brazilian Petroleum (Petrobras - HQ) &592 &12 &5,976 &Yes &No &0.80 &33.86 \\
4& State Courthouse &1,435 &24 &15,524 &Yes &Yes &0.76 &19.45 \\
5& Military &2,539 &24 &170,464 &No &Yes &0.17 &7.38 \\
6& UERJ Foundation &686 &24 &7,226 &Yes &Yes &0.65 &15.61 \\
7& National Bank of Econ. \& Social Dev. &237 &10 &2,234 &Yes &No &0.89 &45.89 \\
8& Health Secretary &1,274 &24 &24,440 &Yes &Yes &0.37 &3.72 \\
9& Brazilian Petroleum Research Center &196 &7 &2,115 &Yes &No &0.74 &31.04 \\
10& Accenture Corp. &337 &9 &1,782 &Yes &No &0.80 &15.68 \\


==> results/firm_top10_p1000.tex <==
1& National Bank of Econ. \& Social Dev. &175 &5 &2,234 &Yes &No &0.89 &45.89 \\
2& Accenture Corp. &224 &7 &1,782 &Yes &No &0.80 &15.68 \\
3& Brazilian Petroleum Research Center &134 &10 &2,115 &Yes &No &0.74 &31.04 \\
4& Brazilian Petroleum Distributor &109 &8 &1,236 &Yes &No &0.79 &24.96 \\
5& Electrobras (Electric Utilities) &76 &8 &1,055 &Yes &No &0.77 &20.83 \\
6& General Public Defender of the State &294 &18 &1,805 &Yes &Yes &0.59 &29.60 \\
7& Brazilian Petroleum (Satellite location) &414 &22 &1,542 &Yes &No &0.85 &30.87 \\
8& Brazilian Petroleum (Petrobras - HQ) &396 &12 &5,976 &Yes &No &0.80 &33.86 \\
9& Rio de Janeiro Federal Courthouse &404 &20 &2,889 &Yes &Yes &0.74 &24.64 \\
10& Duque de Caxias Refinery (Reduc) &364 &22 &1,771 &No &No &0.53 &33.59 \\


==> results/firm_top10_p500.tex <==
1& pH Schooling Platform &399 &24 &515 &Yes &No &0.39 &9.11 \\
2& National Bank of Econ. \& Social Dev. &159 &5 &2,234 &Yes &No &0.89 &45.89 \\
3& State Attorney General Office &131 &18 &808 &Yes &Yes &0.40 &24.66 \\
4& Accenture Corp. &242 &8 &1,782 &Yes &No &0.80 &15.68 \\
5& Brazilian Petroleum Research Center &146 &4 &2,115 &Yes &No &0.74 &31.04 \\
6& National Health Agency &137 &20 &630 &Yes &Yes &0.92 &19.49 \\
7& Brazilian Petroleum Distributor &112 &12 &1,236 &Yes &No &0.79 &24.96 \\
8& Ipiranga Brazilian Petroleum Company &107 &16 &600 &Yes &No &0.76 &17.59 \\
9& Funding Authority for Studies and Projects &94 &16 &622 &Yes &No &0.82 &26.00 \\
10& Electrobras (Electric Utilities) &105 &12 &1,055 &Yes &No &0.77 &20.83 \\


==> results/napply_1.tex <==
1 Accounting & Accounting & \textbf{351} & \textbf{463} & \textbf{450} & \textbf{471} & \textbf{476} & \textbf{469} & \textbf{1,160} & \textbf{350} & \textbf{442} & \textbf{502} & \textbf{374} & \textbf{484} & \textbf{492} & \textbf{551} & \textbf{492} \\\midrule
2 Art & Art &0 &0 &0 &0 &0 &0 &0 &384 &413 &402 &0 &0 &0 &0 &0 \\
  & Art history &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &114 &0 &85 &160 &127 \\
  & Artistic education &198 &233 &210 &230 &235 &234 &547 &0 &0 &0 &0 &0 &0 &0 &0 \\
  & Visual arts &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &326 &334 &292 &328 \\
  & Visual arts (bachelor) &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &127 &0 &0 &0 &0 \\
  & Visual arts (license) &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &125 &0 &0 &0 &0 \\\midrule
3 Biological sciences & Biological sciences & \textbf{194} & \textbf{295} & \textbf{225} & \textbf{292} & \textbf{297} & \textbf{351} & \textbf{1,899} & \textbf{659} & \textbf{1,059} & \textbf{1,156} & \textbf{973} & \textbf{873} & \textbf{1,160} & \textbf{1,028} & \textbf{1,148} \\\midrule
4 Biological sciences (SGO) & Biological sciences (SGO) &94 &229 &151 &236 &222 &235 &643 &271 &246 &380 &274 &325 &252 &209 &227 \\\midrule
5 Business & Business & \textbf{466} & \textbf{583} & \textbf{459} & \textbf{590} & \textbf{590} & \textbf{593} & \textbf{2,200} & \textbf{537} & \textbf{964} & \textbf{983} & \textbf{824} & \textbf{864} & \textbf{1,071} & \textbf{943} & \textbf{1,108} \\\midrule
6 Cartographic eng. & Cartographic engineering &43 &112 &86 &119 &117 &117 &185 &69 &79 &129 &104 &115 &156 &218 &148 \\\midrule
7 Chemical eng. & Chemical engineering &0 &0 &0 &0 &0 & \textbf{317} & \textbf{897} & \textbf{420} & \textbf{662} & \textbf{811} & \textbf{838} & \textbf{817} & \textbf{1,149} & \textbf{1,128} & \textbf{1,290} \\\midrule
8 Chemistry & Chemistry & \textbf{352} & \textbf{474} &340 & \textbf{352} & \textbf{353} & \textbf{160} & \textbf{408} & \textbf{212} & \textbf{206} & \textbf{336} & \textbf{319} & \textbf{317} & \textbf{363} & \textbf{349} & \textbf{321} \\\midrule
9 Computer science & Computer science &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 & \textbf{742} \\
  & Information science & \textbf{633} & \textbf{705} & \textbf{567} & \textbf{587} & \textbf{590} & \textbf{593} & \textbf{2,029} & \textbf{592} & \textbf{699} & \textbf{775} & \textbf{637} & \textbf{603} & \textbf{665} & \textbf{548} &0 \\\midrule
10 Dentistry & Dentistry & \textbf{357} & \textbf{357} & \textbf{350} & \textbf{356} & \textbf{356} & \textbf{359} & \textbf{1,235} & \textbf{450} & \textbf{447} & \textbf{632} & \textbf{446} & \textbf{458} & \textbf{441} & \textbf{503} & \textbf{605} \\\midrule
11 Economics & Economics &442 &541 &408 &539 &548 &547 &1,355 &529 &640 &664 &538 &532 &752 &709 &754 \\\midrule
12 General eng. & Civil engineering &0 &0 &0 &0 &0 &0 & \textbf{736} & \textbf{291} & \textbf{512} & \textbf{574} & \textbf{511} & \textbf{691} & \textbf{908} & \textbf{905} & \textbf{1,310} \\
  & Electrical engineering &0 &0 &0 &0 &0 &0 & \textbf{2,409} & \textbf{614} & \textbf{922} & \textbf{1,070} & \textbf{695} & \textbf{765} & \textbf{1,048} & \textbf{1,066} & \textbf{1,109} \\
  & Engineering &1,065 & \textbf{1,252} & \textbf{1,182} & \textbf{1,407} & \textbf{1,410} & \textbf{1,417} &0 &0 &0 &0 &0 &0 &0 &0 &0 \\
  & Textile engineering &18 & \textbf{153} &42 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\\midrule
13 General language (SGO) & General language (SGO) &298 &351 &326 &469 &470 &475 &910 &332 &334 &395 &208 &246 &251 &180 &233 \\\midrule
14 Geography & Geography & \textbf{113} & \textbf{119} & \textbf{115} & \textbf{157} & \textbf{198} & \textbf{196} & \textbf{943} & \textbf{337} & \textbf{578} & \textbf{524} & \textbf{523} & \textbf{587} & \textbf{532} & \textbf{544} & \textbf{523} \\\midrule
15 Geography (SGO) & Geography (SGO) &137 &214 &131 &232 &237 &237 &591 &291 &366 &369 &259 &259 &334 &225 &202 \\\midrule
16 Geology & Geology &28 & \textbf{84} & \textbf{65} & \textbf{88} & \textbf{89} & \textbf{86} & \textbf{203} & \textbf{94} & \textbf{144} & \textbf{216} & \textbf{185} & \textbf{264} & \textbf{409} & \textbf{317} & \textbf{329} \\\midrule
17 History & History & \textbf{383} & \textbf{298} & \textbf{288} & \textbf{392} & \textbf{395} & \textbf{393} & \textbf{1,991} & \textbf{723} & \textbf{981} & \textbf{1,007} & \textbf{863} & \textbf{719} & \textbf{828} & \textbf{830} & \textbf{772} \\\midrule
18 History (SGO) & History (SGO) & \textbf{202} & \textbf{234} & \textbf{185} & \textbf{238} & \textbf{236} & \textbf{236} & \textbf{592} & \textbf{306} & \textbf{311} & \textbf{412} & \textbf{318} & \textbf{264} & \textbf{292} & \textbf{203} & \textbf{226} \\\midrule
19 Industrial design & Industrial design & \textbf{157} & \textbf{174} & \textbf{171} & \textbf{208} & \textbf{175} & \textbf{207} & \textbf{836} & \textbf{357} & \textbf{480} & \textbf{655} & \textbf{517} & \textbf{539} & \textbf{627} & \textbf{627} & \textbf{699} \\\midrule
20 Journalism & Journalism &0 &0 &0 &0 & \textbf{237} & \textbf{239} & \textbf{1,679} & \textbf{528} & \textbf{717} & \textbf{803} & \textbf{737} & \textbf{672} & \textbf{940} & \textbf{777} & \textbf{1,130} \\
  & Public relations &0 &0 &0 &0 & \textbf{159} & \textbf{239} & \textbf{948} & \textbf{311} & \textbf{469} & \textbf{552} & \textbf{500} & \textbf{479} & \textbf{645} & \textbf{619} & \textbf{717} \\
  & Social communication & \textbf{350} & \textbf{355} & \textbf{350} & \textbf{358} &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\\midrule
21 Language I & English/Literature &0 &0 &0 &0 &0 &0 &0 &403 &328 &403 &325 &285 &318 &281 &295 \\
  & Language I &282 &267 &263 &296 &292 &294 &978 &0 &0 &0 &0 &0 &0 &0 &0 \\
  & Portuguese/German &0 &0 &0 &0 &0 &0 &0 &48 &81 &60 &49 &36 &52 &46 &42 \\
  & Portuguese/Japanese &0 &0 &0 &0 &0 &0 &0 &48 &65 &66 &58 &62 &65 &36 &35 \\\midrule
22 Language II & Language II &317 &350 &363 &388 &388 &513 &1,117 &0 &0 &0 &0 &0 &0 &0 &0 \\
  & Portuguese/France &0 &0 &0 &0 &0 &0 &0 &77 &166 &74 &137 &78 &99 &104 &78 \\
  & Portuguese/Italian &0 &0 &0 &0 &0 &0 &0 &93 &165 &87 &95 &80 &77 &86 &74 \\
  & Portuguese/Spanish &0 &0 &0 &0 &0 &0 &0 &245 &200 &312 &220 &206 &232 &184 &216 \\\midrule
23 Language III & Language III & \textbf{255} & \textbf{322} & \textbf{305} & \textbf{295} & \textbf{296} & \textbf{294} & \textbf{1,212} &0 &0 &0 &0 &0 &0 &0 &0 \\
  & Portuguese/Greek &0 &0 &0 &0 &0 &0 &0 & \textbf{30} & \textbf{21} & \textbf{63} & \textbf{21} & \textbf{29} &10 & \textbf{28} &15 \\
  & Portuguese/Latin &0 &0 &0 &0 &0 &0 &0 & \textbf{57} & \textbf{71} & \textbf{50} & \textbf{65} & \textbf{36} & \textbf{47} & \textbf{31} & \textbf{44} \\
  & Portuguese/Literature &0 &0 &0 &0 &0 &0 &0 & \textbf{454} & \textbf{348} & \textbf{460} & \textbf{338} & \textbf{295} & \textbf{330} & \textbf{294} & \textbf{305} \\\midrule
24 Law & Law & \textbf{1,455} & \textbf{1,477} & \textbf{1,479} & \textbf{1,483} & \textbf{1,496} & \textbf{1,486} & \textbf{5,940} & \textbf{2,079} & \textbf{2,271} & \textbf{3,182} & \textbf{2,487} & \textbf{2,468} & \textbf{2,909} & \textbf{2,884} & \textbf{3,734} \\\midrule
25 Math & Math &243 &354 &537 &586 &592 &589 &1,181 &490 &506 &515 &337 &367 &367 &322 &302 \\\midrule
26 Math (SGO) & Math (SGO) &88 &198 &160 &235 &232 &235 &283 &148 &138 &142 &111 &121 &118 &86 &98 \\\midrule
27 Mechanical eng. & Mechanical engineering &0 &0 &0 &0 &0 &0 & \textbf{516} & \textbf{206} & \textbf{371} & \textbf{508} & \textbf{585} & \textbf{505} & \textbf{728} & \textbf{680} & \textbf{822} \\\midrule
28 Mechanical eng. (NF) & Mechanical engineering (NF) &0 &0 &0 &0 &170 &228 &143 &74 &144 &238 &196 &285 &334 &315 &380 \\\midrule
29 Medicine & Medicine & \textbf{541} & \textbf{546} & \textbf{546} & \textbf{550} & \textbf{552} & \textbf{551} & \textbf{4,122} & \textbf{1,473} & \textbf{1,749} & \textbf{2,754} & \textbf{2,838} & \textbf{2,025} & \textbf{2,639} & \textbf{2,669} & \textbf{3,971} \\\midrule
30 Nursing & Nursing & \textbf{187} & \textbf{312} & \textbf{274} & \textbf{313} & \textbf{311} & \textbf{389} & \textbf{1,478} & \textbf{563} & \textbf{565} & \textbf{762} & \textbf{475} & \textbf{585} & \textbf{536} & \textbf{507} & \textbf{499} \\\midrule
31 Nutrition & Nutrition &236 & \textbf{316} & \textbf{368} & \textbf{311} & \textbf{390} & \textbf{444} & \textbf{2,203} & \textbf{566} & \textbf{706} & \textbf{818} & \textbf{561} & \textbf{599} & \textbf{689} & \textbf{516} & \textbf{661} \\\midrule
32 Oceanography & Oceanography &70 &90 &78 &110 &112 &116 &279 &121 &483 &367 &262 &268 &271 &270 &228 \\\midrule
33 Pedagogy & Pedagogy &557 &614 &577 &623 &616 &621 &1,852 &724 &880 &809 &511 &464 &555 &451 &509 \\\midrule
34 Pedagogy (DDC) & Pedagogy (DDC) &267 &251 &267 &354 &347 &343 &637 &0 &0 &0 &143 &155 &151 &138 &183 \\
  & Pedagogy I (DDC) &0 &0 &0 &0 &0 &0 &0 &201 &160 &225 &0 &0 &0 &0 &0 \\
  & Pedagogy II (DDC) &0 &0 &0 &0 &0 &0 &0 &75 &51 &121 &0 &0 &0 &0 &0 \\\midrule
35 Philosophy & Philosophy &246 &292 &264 &288 &288 &287 &593 &362 &272 &381 &276 &228 &251 &199 &186 \\\midrule
36 Physical education & Physical education &177 &236 &238 &290 &295 &352 &1,611 &447 &506 &600 &413 &405 &470 &384 &413 \\\midrule
37 Physics & Physics &196 &321 &299 &402 &432 &434 &664 &295 &410 &472 &397 &289 &378 &325 &320 \\\midrule
38 Production eng. & Production engineering &0 &0 &0 &0 &0 &0 & \textbf{694} & \textbf{294} & \textbf{466} & \textbf{539} & \textbf{572} & \textbf{526} & \textbf{696} & \textbf{578} & \textbf{792} \\\midrule
39 Production eng. (RES) & Production engineering (RES) &144 &284 &264 &288 &290 &293 &338 &185 &284 &375 &301 &356 &400 &372 &394 \\\midrule
40 Psychology & Psychology & \textbf{268} & \textbf{390} & \textbf{355} & \textbf{394} & \textbf{391} & \textbf{383} & \textbf{1,527} & \textbf{719} & \textbf{887} & \textbf{984} & \textbf{789} & \textbf{800} & \textbf{920} & \textbf{854} & \textbf{1,138} \\\midrule
41 Social science & Social sciences & \textbf{283} & \textbf{297} & \textbf{285} & \textbf{294} & \textbf{294} & \textbf{293} & \textbf{1,311} & \textbf{472} & \textbf{594} & \textbf{631} & \textbf{628} & \textbf{448} & \textbf{547} & \textbf{468} & \textbf{440} \\\midrule
42 Social work & Social work & \textbf{261} & \textbf{276} & \textbf{266} & \textbf{276} & \textbf{275} & \textbf{274} & \textbf{1,240} & \textbf{315} & \textbf{374} & \textbf{511} & \textbf{325} & \textbf{324} & \textbf{348} & \textbf{348} & \textbf{427} \\\midrule
43 Statistics & Statistics &148 &286 &343 &465 &468 &465 &475 &203 &107 &303 &134 &179 &139 &190 &149 \\\midrule


==> results/napply_1_p1.tex <==
1 & Accounting & \textbf{0.364} & Accounting & \textbf{351} & \textbf{463} & \textbf{450} & \textbf{471} & \textbf{476} & \textbf{469} & \textbf{1160} & \textbf{350} & \textbf{442} & \textbf{502} & \textbf{374} & \textbf{484} & \textbf{492} & \textbf{551} & \textbf{492} \\\midrule
2 & Art &0.287 & Artistic education &198 &233 &210 &230 &235 &234 &547 & & & & & & & & \\
 & & & Art & & & & & & & &384 &413 &402 & & & & & \\
 & & & Art history & & & & & & & & & & &114 & &85 &160 &127 \\
 & & & Visual arts (bach.) & & & & & & & & & & &127 & & & & \\
 & & & Visual arts (license) & & & & & & & & & & &125 & & & & \\
 & & & Visual arts & & & & & & & & & & & &326 &334 &292 &328 \\\midrule
3 & Biology & \textbf{0.494} & Biology & \textbf{194} & \textbf{295} & \textbf{225} & \textbf{292} & \textbf{297} & \textbf{351} & \textbf{1899} & \textbf{659} & \textbf{1059} & \textbf{1156} & \textbf{973} & \textbf{873} & \textbf{1160} & \textbf{1028} & \textbf{1148} \\\midrule
4 & Biology (SGO) &0.260 & Biology  &94 &229 &151 &236 &222 &235 &643 &271 &246 &380 &274 &325 &252 &209 &227 \\\midrule
5 & Business & \textbf{0.428} & Business & \textbf{466} & \textbf{583} & \textbf{459} & \textbf{590} & \textbf{590} & \textbf{593} & \textbf{2200} & \textbf{537} & \textbf{964} & \textbf{983} & \textbf{824} & \textbf{864} & \textbf{1071} & \textbf{943} & \textbf{1108} \\\midrule
6 & Cartographic eng. &0.126 & Cartographic eng. &43 &112 &86 &119 &117 &117 &185 &69 &79 &129 &104 &115 &156 &218 &148 \\\midrule
7 & Chemical eng. & \textbf{0.465} & Chemical eng. & & & & & & \textbf{317} & \textbf{897} & \textbf{420} & \textbf{662} & \textbf{811} & \textbf{838} & \textbf{817} & \textbf{1149} & \textbf{1128} & \textbf{1290} \\\midrule
8 & Chemistry & \textbf{0.352} & Chemistry & \textbf{352} & \textbf{474} &340 & \textbf{352} & \textbf{353} & \textbf{160} & \textbf{408} & \textbf{212} & \textbf{206} & \textbf{336} & \textbf{319} & \textbf{317} & \textbf{363} & \textbf{349} & \textbf{321} \\\midrule
9 & Computer science & \textbf{0.325} & Information science & \textbf{633} & \textbf{705} & \textbf{567} & \textbf{587} & \textbf{590} & \textbf{593} & \textbf{2029} & \textbf{592} & \textbf{699} & \textbf{775} & \textbf{637} & \textbf{603} & \textbf{665} & \textbf{548} & \\
 & & & Computer science & & & & & & & & & & & & & & & \textbf{742} \\\midrule
10 & Dentistry & \textbf{0.404} & Dentistry & \textbf{357} & \textbf{357} & \textbf{350} & \textbf{356} & \textbf{356} & \textbf{359} & \textbf{1235} & \textbf{450} & \textbf{447} & \textbf{632} & \textbf{446} & \textbf{458} & \textbf{441} & \textbf{503} & \textbf{605} \\\midrule
11 & Economics &0.286 & Economics &442 &541 &408 &539 &548 &547 &1355 &529 &640 &664 &538 &532 &752 &709 &754 \\\midrule
12 & General eng. & \textbf{0.307} & Engineering &1065 & \textbf{1252} & \textbf{1182} & \textbf{1407} & \textbf{1410} & \textbf{1417} & & & & & & & & & \\
 & & & Civil eng. & & & & & & & \textbf{736} & \textbf{291} & \textbf{512} & \textbf{574} & \textbf{511} & \textbf{691} & \textbf{908} & \textbf{905} & \textbf{1310} \\
 & & & Electrical eng. & & & & & & & \textbf{2409} & \textbf{614} & \textbf{922} & \textbf{1070} & \textbf{695} & \textbf{765} & \textbf{1048} & \textbf{1066} & \textbf{1109} \\
 & & & Textile eng. &18 & \textbf{153} &42 & & & & & & & & & & & & \\\midrule
13 & Geography & \textbf{0.468} & Geography & \textbf{113} & \textbf{119} & \textbf{115} & \textbf{157} & \textbf{198} & \textbf{196} & \textbf{943} & \textbf{337} & \textbf{578} & \textbf{524} & \textbf{523} & \textbf{587} & \textbf{532} & \textbf{544} & \textbf{523} \\\midrule
14 & Geog.\ Ed.\ (SGO) &0.275 & Geography  &137 &214 &131 &232 &237 &237 &591 &291 &366 &369 &259 &259 &334 &225 &202 \\\midrule
15 & Geology & \textbf{0.321} & Geology &28 & \textbf{84} & \textbf{65} & \textbf{88} & \textbf{89} & \textbf{86} & \textbf{203} & \textbf{94} & \textbf{144} & \textbf{216} & \textbf{185} & \textbf{264} & \textbf{409} & \textbf{317} & \textbf{329} \\\midrule
16 & History & \textbf{0.457} & History & \textbf{383} & \textbf{298} & \textbf{288} & \textbf{392} & \textbf{395} & \textbf{393} & \textbf{1991} & \textbf{723} & \textbf{981} & \textbf{1007} & \textbf{863} & \textbf{719} & \textbf{828} & \textbf{830} & \textbf{772} \\\midrule
17 & Hist.\ Ed.\ (SGO) & \textbf{0.333} & History  & \textbf{202} & \textbf{234} & \textbf{185} & \textbf{238} & \textbf{236} & \textbf{236} & \textbf{592} & \textbf{306} & \textbf{311} & \textbf{412} & \textbf{318} & \textbf{264} & \textbf{292} & \textbf{203} & \textbf{226} \\\midrule
18 & Industrial design & \textbf{0.456} & Industrial design & \textbf{157} & \textbf{174} & \textbf{171} & \textbf{208} & \textbf{175} & \textbf{207} & \textbf{836} & \textbf{357} & \textbf{480} & \textbf{655} & \textbf{517} & \textbf{539} & \textbf{627} & \textbf{627} & \textbf{699} \\\midrule
19 & Journalism & \textbf{0.481} & Social communication & \textbf{350} & \textbf{355} & \textbf{350} & \textbf{358} & & & & & & & & & & & \\
 & & & Journalism & & & & & \textbf{237} & \textbf{239} & \textbf{1679} & \textbf{528} & \textbf{717} & \textbf{803} & \textbf{737} & \textbf{672} & \textbf{940} & \textbf{777} & \textbf{1130} \\
 & & & Public relations & & & & & \textbf{159} & \textbf{239} & \textbf{948} & \textbf{311} & \textbf{469} & \textbf{552} & \textbf{500} & \textbf{479} & \textbf{645} & \textbf{619} & \textbf{717} \\\midrule
20 & Language (SGO) &0.205 & Language  &298 &351 &326 &469 &470 &475 &910 &332 &334 &395 &208 &246 &251 &180 &233 \\\midrule
21 & Language I &0.259 & Language I &282 &267 &263 &296 &292 &294 &978 & & & & & & & & \\
 & & & Literature/English & & & & & & & &403 &328 &403 &325 &285 &318 &281 &295 \\
 & & & Port./German & & & & & & & &48 &81 &60 &49 &36 &52 &46 &42 \\
 & & & Port./Japanese & & & & & & & &48 &65 &66 &58 &62 &65 &36 &35 \\\midrule


==> results/napply_1_p2.tex <==
22 & Language II &0.293 & Language II &317 &350 &363 &388 &388 &513 &1117 & & & & & & & & \\
 & & & Port./France & & & & & & & &77 &166 &74 &137 &78 &99 &104 &78 \\
 & & & Port./Italian & & & & & & & &93 &165 &87 &95 &80 &77 &86 &74 \\
 & & & Port./Spanish & & & & & & & &245 &200 &312 &220 &206 &232 &184 &216 \\\midrule
23 & Language III & \textbf{0.379} & Language III & \textbf{255} & \textbf{322} & \textbf{305} & \textbf{295} & \textbf{296} & \textbf{294} & \textbf{1212} & & & & & & & & \\
 & & & Port./Greek & & & & & & & & \textbf{30} & \textbf{21} & \textbf{63} & \textbf{21} & \textbf{29} &10 & \textbf{28} &15 \\
 & & & Port./Latin & & & & & & & & \textbf{57} & \textbf{71} & \textbf{50} & \textbf{65} & \textbf{36} & \textbf{47} & \textbf{31} & \textbf{44} \\
 & & & Port./Literature & & & & & & & & \textbf{454} & \textbf{348} & \textbf{460} & \textbf{338} & \textbf{295} & \textbf{330} & \textbf{294} & \textbf{305} \\\midrule
24 & Law & \textbf{0.460} & Law & \textbf{1455} & \textbf{1477} & \textbf{1479} & \textbf{1483} & \textbf{1496} & \textbf{1486} & \textbf{5940} & \textbf{2079} & \textbf{2271} & \textbf{3182} & \textbf{2487} & \textbf{2468} & \textbf{2909} & \textbf{2884} & \textbf{3734} \\\midrule
25 & Math &0.158 & Math &243 &354 &537 &586 &592 &589 &1181 &490 &506 &515 &337 &367 &367 &322 &302 \\\midrule
26 & Math Ed.\ (SGO) &0.143 & Math  &88 &198 &160 &235 &232 &235 &283 &148 &138 &142 &111 &121 &118 &86 &98 \\\midrule
27 & Mech. eng. & \textbf{0.353} & Mech. eng. & & & & & & & \textbf{516} & \textbf{206} & \textbf{371} & \textbf{508} & \textbf{585} & \textbf{505} & \textbf{728} & \textbf{680} & \textbf{822} \\\midrule
28 & Mech. eng. (NF) &0.186 & Mech. eng.  & & & & &170 &228 &143 &74 &144 &238 &196 &285 &334 &315 &380 \\\midrule
29 & Medicine & \textbf{0.454} & Medicine & \textbf{541} & \textbf{546} & \textbf{546} & \textbf{550} & \textbf{552} & \textbf{551} & \textbf{4122} & \textbf{1473} & \textbf{1749} & \textbf{2754} & \textbf{2838} & \textbf{2025} & \textbf{2639} & \textbf{2669} & \textbf{3971} \\\midrule
30 & Nursing & \textbf{0.431} & Nursing & \textbf{187} & \textbf{312} & \textbf{274} & \textbf{313} & \textbf{311} & \textbf{389} & \textbf{1478} & \textbf{563} & \textbf{565} & \textbf{762} & \textbf{475} & \textbf{585} & \textbf{536} & \textbf{507} & \textbf{499} \\\midrule
31 & Nutrition & \textbf{0.411} & Nutrition &236 & \textbf{316} & \textbf{368} & \textbf{311} & \textbf{390} & \textbf{444} & \textbf{2203} & \textbf{566} & \textbf{706} & \textbf{818} & \textbf{561} & \textbf{599} & \textbf{689} & \textbf{516} & \textbf{661} \\\midrule
32 & Oceanography &0.229 & Oceanography &70 &90 &78 &110 &112 &116 &279 &121 &483 &367 &262 &268 &271 &270 &228 \\\midrule
33 & Teaching &0.234 & Teaching &557 &614 &577 &623 &616 &621 &1852 &724 &880 &809 &511 &464 &555 &451 &509 \\\midrule
34 & Teaching (DDC) &0.208 & Teaching  &267 &251 &267 &354 &347 &343 &637 & & & &143 &155 &151 &138 &183 \\
 & & & Teaching I  & & & & & & & &201 &160 &225 & & & & & \\
 & & & Teaching II  & & & & & & & &75 &51 &121 & & & & & \\\midrule
35 & Philosophy &0.222 & Philosophy &246 &292 &264 &288 &288 &287 &593 &362 &272 &381 &276 &228 &251 &199 &186 \\\midrule
36 & Physical ed. &0.206 & Physical education &177 &236 &238 &290 &295 &352 &1611 &447 &506 &600 &413 &405 &470 &384 &413 \\\midrule
37 & Physics &0.135 & Physics &196 &321 &299 &402 &432 &434 &664 &295 &410 &472 &397 &289 &378 &325 &320 \\\midrule
38 & Prod. eng. & \textbf{0.384} & Prod. eng. & & & & & & & \textbf{694} & \textbf{294} & \textbf{466} & \textbf{539} & \textbf{572} & \textbf{526} & \textbf{696} & \textbf{578} & \textbf{792} \\\midrule
39 & Prod. eng. (RES) &0.152 & Prod. eng.  &144 &284 &264 &288 &290 &293 &338 &185 &284 &375 &301 &356 &400 &372 &394 \\\midrule
40 & Psychology & \textbf{0.480} & Psychology & \textbf{268} & \textbf{390} & \textbf{355} & \textbf{394} & \textbf{391} & \textbf{383} & \textbf{1527} & \textbf{719} & \textbf{887} & \textbf{984} & \textbf{789} & \textbf{800} & \textbf{920} & \textbf{854} & \textbf{1138} \\\midrule
41 & Social science & \textbf{0.408} & Social sciences & \textbf{283} & \textbf{297} & \textbf{285} & \textbf{294} & \textbf{294} & \textbf{293} & \textbf{1311} & \textbf{472} & \textbf{594} & \textbf{631} & \textbf{628} & \textbf{448} & \textbf{547} & \textbf{468} & \textbf{440} \\\midrule
42 & Social work & \textbf{0.432} & Social work & \textbf{261} & \textbf{276} & \textbf{266} & \textbf{276} & \textbf{275} & \textbf{274} & \textbf{1240} & \textbf{315} & \textbf{374} & \textbf{511} & \textbf{325} & \textbf{324} & \textbf{348} & \textbf{348} & \textbf{427} \\\midrule
43 & Statistics &0.087 & Statistics &148 &286 &343 &465 &468 &465 &475 &203 &107 &303 &134 &179 &139 &190 &149 \\\midrule


==> results/napply_2.tex <==
1 Accounting & Accounting &. &. &. &. &. &. &. &74 &50 & \textbf{71} & \textbf{41} & \textbf{31} & \textbf{37} & \textbf{50} & \textbf{50} \\\midrule
2 Art & Art &. &. &. &. &. &. &. &84 &26 &19 &0 &0 &0 &0 &0 \\
  & Art history &. &. &. &. &. &. &. &0 &0 &0 &9 &0 &5 &2 &4 \\
  & Visual arts &. &. &. &. &. &. &. &0 &0 &0 &0 &17 &16 &13 &13 \\
  & Visual arts (bachelor) &. &. &. &. &. &. &. &0 &0 &0 &7 &0 &0 &0 &0 \\
  & Visual arts (license) &. &. &. &. &. &. &. &0 &0 &0 &10 &0 &0 &0 &0 \\\midrule
3 Biological sciences & Biological sciences &. &. &. &. &. &. &. & \textbf{126} & \textbf{70} & \textbf{88} & \textbf{64} & \textbf{38} & \textbf{64} & \textbf{51} & \textbf{48} \\\midrule
4 Biological sciences (SGO) & Biological sciences (SGO) &. &. &. &. &. &. &. &66 &19 &37 &21 &19 &13 &19 &25 \\\midrule
5 Business & Business &. &. &. &. &. &. &. & \textbf{111} & \textbf{53} & \textbf{85} & \textbf{59} & \textbf{54} & \textbf{54} & \textbf{67} & \textbf{75} \\\midrule
6 Cartographic eng. & Cartographic engineering &. &. &. &. &. &. &. &12 &2 &4 &3 &2 &8 &5 &14 \\\midrule
7 Chemical eng. & Chemical engineering &. &. &. &. &. &. &. & \textbf{43} &45 & \textbf{42} & \textbf{34} &27 & \textbf{56} & \textbf{42} & \textbf{55} \\\midrule
8 Chemistry & Chemistry &. &. &. &. &. &. &. &29 &11 & \textbf{24} & \textbf{16} & \textbf{24} & \textbf{13} &17 &9 \\\midrule
9 Computer science & Computer science &. &. &. &. &. &. &. &0 &0 &0 &0 &0 &0 &0 & \textbf{35} \\
  & Information science &. &. &. &. &. &. &. & \textbf{111} &40 & \textbf{57} & \textbf{34} & \textbf{43} & \textbf{36} &38 &0 \\\midrule
10 Dentistry & Dentistry &. &. &. &. &. &. &. & \textbf{57} &15 & \textbf{25} &17 &17 & \textbf{23} & \textbf{28} & \textbf{30} \\\midrule
11 Economics & Economics &. &. &. &. &. &. &. &77 &34 &40 &24 &32 &30 &26 &31 \\\midrule
12 General eng. & Civil engineering &. &. &. &. &. &. &. &58 &26 & \textbf{35} & \textbf{30} &23 & \textbf{58} & \textbf{47} & \textbf{74} \\
  & Electrical engineering &. &. &. &. &. &. &. &113 &54 & \textbf{87} & \textbf{56} &38 & \textbf{64} & \textbf{72} & \textbf{72} \\\midrule
13 General language (SGO) & General language (SGO) &. &. &. &. &. &. &. &108 &26 &57 &24 &21 &15 &14 &16 \\\midrule
14 Geography & Geography &. &. &. &. &. &. &. & \textbf{80} & \textbf{56} & \textbf{49} & \textbf{49} & \textbf{25} & \textbf{40} & \textbf{32} &20 \\\midrule
15 Geography (SGO) & Geography (SGO) &. &. &. &. &. &. &. &73 &55 &35 &23 &17 &20 &21 &26 \\\midrule
16 Geology & Geology &. &. &. &. &. &. &. & \textbf{14} &4 &12 &4 &7 & \textbf{20} &10 & \textbf{16} \\\midrule
17 History & History &. &. &. &. &. &. &. & \textbf{174} & \textbf{81} & \textbf{114} & \textbf{84} & \textbf{54} & \textbf{55} & \textbf{53} & \textbf{55} \\\midrule
18 History (SGO) & History (SGO) &. &. &. &. &. &. &. & \textbf{71} &29 & \textbf{50} & \textbf{27} &24 &20 &9 &24 \\\midrule
19 Industrial design & Industrial design &. &. &. &. &. &. &. & \textbf{33} &11 & \textbf{33} &17 & \textbf{18} & \textbf{33} & \textbf{33} & \textbf{36} \\\midrule
20 Journalism & Journalism &. &. &. &. &. &. &. & \textbf{94} & \textbf{30} & \textbf{54} & \textbf{33} & \textbf{33} & \textbf{36} & \textbf{38} & \textbf{44} \\
  & Public relations &. &. &. &. &. &. &. & \textbf{37} & \textbf{13} & \textbf{28} &21 & \textbf{23} & \textbf{25} & \textbf{34} & \textbf{35} \\\midrule
21 Language I & English/Literature &. &. &. &. &. &. &. &53 &17 &27 &9 &8 &15 &19 &10 \\
  & Portuguese/German &. &. &. &. &. &. &. &0 &2 &1 &1 &0 &5 &1 &2 \\
  & Portuguese/Japanese &. &. &. &. &. &. &. &8 &3 &6 &2 &1 &4 &1 &5 \\\midrule
22 Language II & Portuguese/France &. &. &. &. &. &. &. &15 &18 &7 &9 &1 &5 &8 &3 \\
  & Portuguese/Italian &. &. &. &. &. &. &. &22 &13 &13 &9 &6 &4 &6 &7 \\
  & Portuguese/Spanish &. &. &. &. &. &. &. &79 &19 &30 &24 &11 &11 &20 &15 \\\midrule
23 Language III & Portuguese/Greek &. &. &. &. &. &. &. & \textbf{7} &2 &4 &3 &0 &1 &1 &1 \\
  & Portuguese/Latin &. &. &. &. &. &. &. & \textbf{11} &4 &8 &4 &1 &3 &4 &2 \\
  & Portuguese/Literature &. &. &. &. &. &. &. & \textbf{123} & \textbf{37} & \textbf{67} &33 &27 &16 &20 & \textbf{25} \\\midrule
24 Law & Law &. &. &. &. &. &. &. & \textbf{284} & \textbf{113} & \textbf{217} & \textbf{132} & \textbf{147} & \textbf{173} & \textbf{198} & \textbf{203} \\\midrule
25 Math & Math &. &. &. &. &. &. &. &133 &41 &47 &28 &23 &18 &16 &9 \\\midrule
26 Math (SGO) & Math (SGO) &. &. &. &. &. &. &. &35 &13 &18 &11 &10 &3 &8 &7 \\\midrule
27 Mechanical eng. & Mechanical engineering &. &. &. &. &. &. &. & \textbf{31} &9 &16 & \textbf{17} & \textbf{24} & \textbf{27} & \textbf{38} & \textbf{31} \\\midrule
28 Mechanical eng. (NF) & Mechanical engineering (NF) &. &. &. &. &. &. &. &16 &6 &16 &9 &11 &21 &18 &43 \\\midrule
29 Medicine & Medicine &. &. &. &. &. &. &. & \textbf{135} & \textbf{61} & \textbf{73} & \textbf{83} & \textbf{65} & \textbf{106} & \textbf{145} & \textbf{189} \\\midrule
30 Nursing & Nursing &. &. &. &. &. &. &. & \textbf{119} & \textbf{44} & \textbf{74} & \textbf{25} & \textbf{46} & \textbf{52} & \textbf{37} & \textbf{37} \\\midrule
31 Nutrition & Nutrition &. &. &. &. &. &. &. & \textbf{93} &33 & \textbf{80} & \textbf{50} & \textbf{35} & \textbf{41} & \textbf{29} & \textbf{44} \\\midrule
32 Oceanography & Oceanography &. &. &. &. &. &. &. &13 &19 &17 &8 &6 &8 &9 &10 \\\midrule
33 Pedagogy & Pedagogy &. &. &. &. &. &. &. &284 &91 &137 &74 &32 &37 &40 &41 \\\midrule
34 Pedagogy (DDC) & Pedagogy (DDC) &. &. &. &. &. &. &. &0 &0 &0 &16 &9 &7 &12 &9 \\
  & Pedagogy I (DDC) &. &. &. &. &. &. &. &59 &19 &32 &0 &0 &0 &0 &0 \\
  & Pedagogy II (DDC) &. &. &. &. &. &. &. &27 &5 &11 &0 &0 &0 &0 &0 \\\midrule
35 Philosophy & Philosophy &. &. &. &. &. &. &. &70 &14 &30 &18 &13 &11 &15 &11 \\\midrule
36 Physical education & Physical education &. &. &. &. &. &. &. &105 &27 &51 &24 &26 &19 &19 &25 \\\midrule
37 Physics & Physics &. &. &. &. &. &. &. &70 &25 &32 &17 &13 &17 &13 &15 \\\midrule
38 Production eng. & Production engineering &. &. &. &. &. &. &. &21 &18 &13 &14 & \textbf{22} & \textbf{39} &21 & \textbf{39} \\\midrule
39 Production eng. (RES) & Production engineering (RES) &. &. &. &. &. &. &. &31 &8 &17 &12 &8 &17 &20 &21 \\\midrule
40 Psychology & Psychology &. &. &. &. &. &. &. & \textbf{181} & \textbf{76} & \textbf{85} & \textbf{56} & \textbf{47} & \textbf{62} & \textbf{63} & \textbf{77} \\\midrule
41 Social science & Social sciences &. &. &. &. &. &. &. & \textbf{75} &36 & \textbf{49} & \textbf{43} &17 &20 &28 &24 \\\midrule
42 Social work & Social work &. &. &. &. &. &. &. & \textbf{127} & \textbf{56} & \textbf{81} & \textbf{54} &27 & \textbf{34} &28 & \textbf{38} \\\midrule
43 Statistics & Statistics &. &. &. &. &. &. &. &31 &5 &16 &1 &9 &4 &3 &5 \\\midrule


==> results/napply_2_p1.tex <==
1 & Accounting & \textbf{0.364} & Accounting &74 &50 & \textbf{71} & \textbf{41} & \textbf{31} & \textbf{37} & \textbf{50} & \textbf{50} \\\midrule
2 & Art &0.287 & Artistic education & & & & & & & & \\
 & & & Art &84 &26 &19 & & & & & \\
 & & & Art history & & & &9 & &5 &2 &4 \\
 & & & Visual arts (bach.) & & & &7 & & & & \\
 & & & Visual arts (license) & & & &10 & & & & \\
 & & & Visual arts & & & & &17 &16 &13 &13 \\\midrule
3 & Biology & \textbf{0.494} & Biology & \textbf{126} & \textbf{70} & \textbf{88} & \textbf{64} & \textbf{38} & \textbf{64} & \textbf{51} & \textbf{48} \\\midrule
4 & Biology (SGO) &0.260 & Biology  &66 &19 &37 &21 &19 &13 &19 &25 \\\midrule
5 & Business & \textbf{0.428} & Business & \textbf{111} & \textbf{53} & \textbf{85} & \textbf{59} & \textbf{54} & \textbf{54} & \textbf{67} & \textbf{75} \\\midrule
6 & Cartographic eng. &0.126 & Cartographic eng. &12 &2 &4 &3 &2 &8 &5 &14 \\\midrule
7 & Chemical eng. & \textbf{0.465} & Chemical eng. & \textbf{43} &45 & \textbf{42} & \textbf{34} &27 & \textbf{56} & \textbf{42} & \textbf{55} \\\midrule
8 & Chemistry & \textbf{0.352} & Chemistry &29 &11 & \textbf{24} & \textbf{16} & \textbf{24} & \textbf{13} &17 &9 \\\midrule
9 & Computer science & \textbf{0.325} & Information science & \textbf{111} &40 & \textbf{57} & \textbf{34} & \textbf{43} & \textbf{36} &38 & \\
 & & & Computer science & & & & & & & & \textbf{35} \\\midrule
10 & Dentistry & \textbf{0.404} & Dentistry & \textbf{57} &15 & \textbf{25} &17 &17 & \textbf{23} & \textbf{28} & \textbf{30} \\\midrule
11 & Economics &0.286 & Economics &77 &34 &40 &24 &32 &30 &26 &31 \\\midrule
12 & General eng. & \textbf{0.307} & Civil eng. &58 &26 & \textbf{35} & \textbf{30} &23 & \textbf{58} & \textbf{47} & \textbf{74} \\
 & & & Engineering & & & & & & & & \\
 & & & Electrical eng. &113 &54 & \textbf{87} & \textbf{56} &38 & \textbf{64} & \textbf{72} & \textbf{72} \\
 & & & Textile eng. & & & & & & & & \\\midrule
13 & Geography & \textbf{0.468} & Geography & \textbf{80} & \textbf{56} & \textbf{49} & \textbf{49} & \textbf{25} & \textbf{40} & \textbf{32} &20 \\\midrule
14 & Geog.\ Ed.\ (SGO) &0.275 & Geography  &73 &55 &35 &23 &17 &20 &21 &26 \\\midrule
15 & Geology & \textbf{0.321} & Geology & \textbf{14} &4 &12 &4 &7 & \textbf{20} &10 & \textbf{16} \\\midrule
16 & History & \textbf{0.457} & History & \textbf{174} & \textbf{81} & \textbf{114} & \textbf{84} & \textbf{54} & \textbf{55} & \textbf{53} & \textbf{55} \\\midrule
17 & Hist.\ Ed.\ (SGO) & \textbf{0.333} & History  & \textbf{71} &29 & \textbf{50} & \textbf{27} &24 &20 &9 &24 \\\midrule
18 & Industrial design & \textbf{0.456} & Industrial design & \textbf{33} &11 & \textbf{33} &17 & \textbf{18} & \textbf{33} & \textbf{33} & \textbf{36} \\\midrule
19 & Journalism & \textbf{0.481} & Social communication & & & & & & & & \\
 & & & Journalism & \textbf{94} & \textbf{30} & \textbf{54} & \textbf{33} & \textbf{33} & \textbf{36} & \textbf{38} & \textbf{44} \\
 & & & Public relations & \textbf{37} & \textbf{13} & \textbf{28} &21 & \textbf{23} & \textbf{25} & \textbf{34} & \textbf{35} \\\midrule
20 & Language (SGO) &0.205 & Language  &108 &26 &57 &24 &21 &15 &14 &16 \\\midrule
21 & Language I &0.259 & Language I & & & & & & & & \\
 & & & Literature/English &53 &17 &27 &9 &8 &15 &19 &10 \\
 & & & Port./German & &2 &1 &1 & &5 &1 &2 \\
 & & & Port./Japanese &8 &3 &6 &2 &1 &4 &1 &5 \\\midrule


==> results/napply_2_p2.tex <==
22 & Language II &0.293 & Language II & & & & & & & & \\
 & & & Port./France &15 &18 &7 &9 &1 &5 &8 &3 \\
 & & & Port./Italian &22 &13 &13 &9 &6 &4 &6 &7 \\
 & & & Port./Spanish &79 &19 &30 &24 &11 &11 &20 &15 \\\midrule
23 & Language III & \textbf{0.379} & Language III & & & & & & & & \\
 & & & Port./Greek & \textbf{7} &2 &4 &3 & &1 &1 &1 \\
 & & & Port./Latin & \textbf{11} &4 &8 &4 &1 &3 &4 &2 \\
 & & & Port./Literature & \textbf{123} & \textbf{37} & \textbf{67} &33 &27 &16 &20 & \textbf{25} \\\midrule
24 & Law & \textbf{0.460} & Law & \textbf{284} & \textbf{113} & \textbf{217} & \textbf{132} & \textbf{147} & \textbf{173} & \textbf{198} & \textbf{203} \\\midrule
25 & Math &0.158 & Math &133 &41 &47 &28 &23 &18 &16 &9 \\\midrule
26 & Math Ed.\ (SGO) &0.143 & Math  &35 &13 &18 &11 &10 &3 &8 &7 \\\midrule
27 & Mech. eng. & \textbf{0.353} & Mech. eng. & \textbf{31} &9 &16 & \textbf{17} & \textbf{24} & \textbf{27} & \textbf{38} & \textbf{31} \\\midrule
28 & Mech. eng. (NF) &0.186 & Mech. eng.  &16 &6 &16 &9 &11 &21 &18 &43 \\\midrule
29 & Medicine & \textbf{0.454} & Medicine & \textbf{135} & \textbf{61} & \textbf{73} & \textbf{83} & \textbf{65} & \textbf{106} & \textbf{145} & \textbf{189} \\\midrule
30 & Nursing & \textbf{0.431} & Nursing & \textbf{119} & \textbf{44} & \textbf{74} & \textbf{25} & \textbf{46} & \textbf{52} & \textbf{37} & \textbf{37} \\\midrule
31 & Nutrition & \textbf{0.411} & Nutrition & \textbf{93} &33 & \textbf{80} & \textbf{50} & \textbf{35} & \textbf{41} & \textbf{29} & \textbf{44} \\\midrule
32 & Oceanography &0.229 & Oceanography &13 &19 &17 &8 &6 &8 &9 &10 \\\midrule
33 & Teaching &0.234 & Teaching &284 &91 &137 &74 &32 &37 &40 &41 \\\midrule
34 & Teaching (DDC) &0.208 & Teaching  & & & &16 &9 &7 &12 &9 \\
 & & & Teaching I  &59 &19 &32 & & & & & \\
 & & & Teaching II  &27 &5 &11 & & & & & \\\midrule
35 & Philosophy &0.222 & Philosophy &70 &14 &30 &18 &13 &11 &15 &11 \\\midrule
36 & Physical ed. &0.206 & Physical education &105 &27 &51 &24 &26 &19 &19 &25 \\\midrule
37 & Physics &0.135 & Physics &70 &25 &32 &17 &13 &17 &13 &15 \\\midrule
38 & Prod. eng. & \textbf{0.384} & Prod. eng. &21 &18 &13 &14 & \textbf{22} & \textbf{39} &21 & \textbf{39} \\\midrule
39 & Prod. eng. (RES) &0.152 & Prod. eng.  &31 &8 &17 &12 &8 &17 &20 &21 \\\midrule
40 & Psychology & \textbf{0.480} & Psychology & \textbf{181} & \textbf{76} & \textbf{85} & \textbf{56} & \textbf{47} & \textbf{62} & \textbf{63} & \textbf{77} \\\midrule
41 & Social science & \textbf{0.408} & Social sciences & \textbf{75} &36 & \textbf{49} & \textbf{43} &17 &20 &28 &24 \\\midrule
42 & Social work & \textbf{0.432} & Social work & \textbf{127} & \textbf{56} & \textbf{81} & \textbf{54} &27 & \textbf{34} &28 & \textbf{38} \\\midrule
43 & Statistics &0.087 & Statistics &31 &5 &16 &1 &9 &4 &3 &5 \\\midrule


==> results/napply_3.tex <==
1 Accounting & Accounting &. &. &. &. &. &. &. & \textbf{47} &17 &25 &17 &13 &23 & \textbf{33} & \textbf{42} \\\midrule
2 Art & Art &. &. &. &. &. &. &. &53 &12 &10 &0 &0 &0 &0 &0 \\
  & Art history &. &. &. &. &. &. &. &0 &0 &0 &3 &0 &0 &6 &7 \\
  & Visual arts &. &. &. &. &. &. &. &0 &0 &0 &0 &6 &8 &14 &6 \\
  & Visual arts (bachelor) &. &. &. &. &. &. &. &0 &0 &0 &3 &0 &0 &0 &0 \\
  & Visual arts (license) &. &. &. &. &. &. &. &0 &0 &0 &2 &0 &0 &0 &0 \\\midrule
3 Biological sciences & Biological sciences &. &. &. &. &. &. &. & \textbf{64} & \textbf{28} & \textbf{28} & \textbf{32} &14 & \textbf{39} & \textbf{33} & \textbf{44} \\\midrule
4 Biological sciences (SGO) & Biological sciences (SGO) &. &. &. &. &. &. &. &28 &9 &13 &8 &4 &7 &7 &6 \\\midrule
5 Business & Business &. &. &. &. &. &. &. & \textbf{59} & \textbf{38} & \textbf{42} &17 &25 & \textbf{54} & \textbf{42} & \textbf{47} \\\midrule
6 Cartographic eng. & Cartographic engineering &. &. &. &. &. &. &. &4 &1 &2 &2 &0 &2 &9 &5 \\\midrule
7 Chemical eng. & Chemical engineering &. &. &. &. &. &. &. &26 &13 &18 &16 &16 & \textbf{34} & \textbf{43} & \textbf{47} \\\midrule
8 Chemistry & Chemistry &. &. &. &. &. &. &. & \textbf{19} &6 &10 &8 &2 &14 &8 &15 \\\midrule
9 Computer science & Computer science &. &. &. &. &. &. &. &0 &0 &0 &0 &0 &0 &0 &17 \\
  & Information science &. &. &. &. &. &. &. &63 &19 & \textbf{30} &20 &17 &14 &21 &0 \\\midrule
10 Dentistry & Dentistry &. &. &. &. &. &. &. & \textbf{42} &5 & \textbf{18} &12 &16 &14 & \textbf{24} & \textbf{24} \\\midrule
11 Economics & Economics &. &. &. &. &. &. &. &36 &14 &20 &5 &6 &25 &30 &22 \\\midrule
12 General eng. & Civil engineering &. &. &. &. &. &. &. &21 &7 &12 &11 &9 &25 & \textbf{31} & \textbf{70} \\
  & Electrical engineering &. &. &. &. &. &. &. & \textbf{61} &22 &30 &25 &13 &32 &40 & \textbf{62} \\\midrule
13 General language (SGO) & General language (SGO) &. &. &. &. &. &. &. &47 &15 &16 &6 &3 &10 &4 &9 \\\midrule
14 Geography & Geography &. &. &. &. &. &. &. & \textbf{49} &23 &18 &14 &19 &21 & \textbf{33} &22 \\\midrule
15 Geography (SGO) & Geography (SGO) &. &. &. &. &. &. &. &52 &21 &18 &12 &11 &7 &15 &11 \\\midrule
16 Geology & Geology &. &. &. &. &. &. &. &7 &4 &4 &2 &6 & \textbf{13} &12 & \textbf{13} \\\midrule
17 History & History &. &. &. &. &. &. &. & \textbf{124} & \textbf{37} & \textbf{39} & \textbf{37} &24 & \textbf{50} & \textbf{36} & \textbf{31} \\\midrule
18 History (SGO) & History (SGO) &. &. &. &. &. &. &. & \textbf{44} &10 &19 &11 &11 &16 &11 &9 \\\midrule
19 Industrial design & Industrial design &. &. &. &. &. &. &. & \textbf{25} &6 & \textbf{14} &7 &8 & \textbf{21} &8 & \textbf{18} \\\midrule
20 Journalism & Journalism &. &. &. &. &. &. &. & \textbf{67} & \textbf{13} & \textbf{25} &19 & \textbf{23} & \textbf{29} & \textbf{31} & \textbf{31} \\
  & Public relations &. &. &. &. &. &. &. & \textbf{36} & \textbf{22} & \textbf{22} &11 &8 & \textbf{25} & \textbf{30} & \textbf{32} \\\midrule
21 Language I & English/Literature &. &. &. &. &. &. &. &31 &8 &6 &4 &5 &11 &7 &12 \\
  & Portuguese/German &. &. &. &. &. &. &. &4 &1 &0 &2 &1 &1 &0 &0 \\
  & Portuguese/Japanese &. &. &. &. &. &. &. &6 &0 &1 &1 &0 &2 &2 &0 \\\midrule
22 Language II & Portuguese/France &. &. &. &. &. &. &. &10 &3 &2 &4 &4 &2 &5 &3 \\
  & Portuguese/Italian &. &. &. &. &. &. &. &7 &12 &3 &1 &2 &2 &2 &4 \\
  & Portuguese/Spanish &. &. &. &. &. &. &. &36 &9 &18 &17 &9 &6 &7 &8 \\\midrule
23 Language III & Portuguese/Greek &. &. &. &. &. &. &. &7 &0 &3 &1 &0 &1 &2 &1 \\
  & Portuguese/Latin &. &. &. &. &. &. &. &6 &4 &2 &5 &0 &3 &1 &0 \\
  & Portuguese/Literature &. &. &. &. &. &. &. & \textbf{71} &18 & \textbf{24} &12 &11 &13 &13 &19 \\\midrule
24 Law & Law &. &. &. &. &. &. &. & \textbf{271} & \textbf{89} & \textbf{138} & \textbf{122} & \textbf{125} & \textbf{174} & \textbf{192} & \textbf{247} \\\midrule
25 Math & Math &. &. &. &. &. &. &. &54 &16 &9 &15 &10 &5 &7 &6 \\\midrule
26 Math (SGO) & Math (SGO) &. &. &. &. &. &. &. &16 &2 &1 &1 &1 &1 &3 &3 \\\midrule
27 Mechanical eng. & Mechanical engineering &. &. &. &. &. &. &. & \textbf{28} &7 &10 &9 &11 & \textbf{22} & \textbf{18} & \textbf{27} \\\midrule
28 Mechanical eng. (NF) & Mechanical engineering (NF) &. &. &. &. &. &. &. &3 &1 &2 &2 &0 &6 &7 &8 \\\midrule
29 Medicine & Medicine &. &. &. &. &. &. &. & \textbf{123} & \textbf{38} & \textbf{53} & \textbf{58} & \textbf{48} & \textbf{114} & \textbf{120} & \textbf{187} \\\midrule
30 Nursing & Nursing &. &. &. &. &. &. &. & \textbf{109} &17 & \textbf{35} &19 &20 & \textbf{32} & \textbf{23} & \textbf{26} \\\midrule
31 Nutrition & Nutrition &. &. &. &. &. &. &. & \textbf{60} & \textbf{24} & \textbf{25} &10 &16 &22 &19 &28 \\\midrule
32 Oceanography & Oceanography &. &. &. &. &. &. &. &11 &6 &9 &2 &4 &2 &6 &2 \\\midrule
33 Pedagogy & Pedagogy &. &. &. &. &. &. &. &157 &40 &57 &25 &16 &27 &23 &34 \\\midrule
34 Pedagogy (DDC) & Pedagogy (DDC) &. &. &. &. &. &. &. &0 &0 &0 &12 &12 &15 &8 &11 \\
  & Pedagogy I (DDC) &. &. &. &. &. &. &. &55 &13 &17 &0 &0 &0 &0 &0 \\
  & Pedagogy II (DDC) &. &. &. &. &. &. &. &17 &8 &5 &0 &0 &0 &0 &0 \\\midrule
35 Philosophy & Philosophy &. &. &. &. &. &. &. &52 &11 &9 &4 &2 &14 &6 &4 \\\midrule
36 Physical education & Physical education &. &. &. &. &. &. &. &56 &6 &24 &9 &5 &6 &11 &12 \\\midrule
37 Physics & Physics &. &. &. &. &. &. &. &37 &7 &10 &8 &4 &9 &8 &4 \\\midrule
38 Production eng. & Production engineering &. &. &. &. &. &. &. &9 &6 &5 &3 &12 & \textbf{23} &10 & \textbf{36} \\\midrule
39 Production eng. (RES) & Production engineering (RES) &. &. &. &. &. &. &. &14 &5 &8 &2 &1 &5 &7 &7 \\\midrule
40 Psychology & Psychology &. &. &. &. &. &. &. & \textbf{123} & \textbf{32} & \textbf{37} & \textbf{28} &28 & \textbf{43} & \textbf{42} & \textbf{53} \\\midrule
41 Social science & Social sciences &. &. &. &. &. &. &. & \textbf{56} &19 &23 &22 &22 &15 & \textbf{34} &29 \\\midrule
42 Social work & Social work &. &. &. &. &. &. &. & \textbf{119} & \textbf{36} & \textbf{48} & \textbf{27} &30 & \textbf{41} &22 & \textbf{52} \\\midrule
43 Statistics & Statistics &. &. &. &. &. &. &. &21 &4 &8 &0 &1 &2 &3 &6 \\\midrule


==> results/ols.tex <==
Enrolled in UERJ&&0.277&\sym{***}&0.274&\sym{***}&0.262&\sym{***}&0.076&\sym{***}&0.039&\sym{*}\\
&&(0.021&)&(0.022&)&(0.021&)&(0.026&)&(0.024&)\\
Age&&&&&&0.000&&0.002&&0.002&\\
&&&&&&(0.003&)&(0.003&)&(0.003&)\\
Male&&&&&&0.193&\sym{***}&0.180&\sym{***}&0.105&\sym{***}\\
&&&&&&(0.023&)&(0.022&)&(0.021&)\\
White&&&&&&0.036&\sym{*}&0.033&&0.025&\\
&&&&&&(0.021&)&(0.021&)&(0.019&)\\
Admission score&&&&&&&&0.211&\sym{***}&0.242&\sym{***}\\
&&&&&&&&(0.017&)&(0.016&)\\
N&&13,224&&13,224&&13,223&&13,223&&13,223&\\


==> results/ols_alumni.tex <==
\addlinespace
Any alumni firm&&0.444&&&&0.298&&&\\
&&(0.004&)&&&(0.004&)&&\\
\addlinespace
Firm w/ 50+ alumni per 1000 workers&&&&0.398&&&&0.211&\\
&&&&(0.011&)&&&(0.010&)\\
\addlinespace
Firm w/ 25$-$50 alumni per 1000 workers&&&&0.589&&&&0.392&\\
&&&&(0.010&)&&&(0.009&)\\
\addlinespace
Firm w/ 10$-$25 alumni per 1000 workers&&&&0.639&&&&0.411&\\
&&&&(0.006&)&&&(0.006&)\\
\addlinespace
Firm w/ 5$-$10 alumni per 1000 workers&&&&0.488&&&&0.416&\\
&&&&(0.007&)&&&(0.007&)\\
\addlinespace
Firm w/ 1$-$5 alumni per 1000 workers&&&&0.439&&&&0.261&\\
&&&&(0.005&)&&&(0.005&)\\
\addlinespace
Firm w/ 0$-$1 alumni per 1000 workers&&&&0.303&&&&0.230&\\
&&&&(0.005&)&&&(0.006&)\\


==> results/ols_alumni_n.tex <==
\(N\)&&549,675&&549,675&&554,242&&554,242&\\


==> results/ols_alumni_type.tex <==
\addlinespace
Firm w/ pre-AA alumni only&&0.482&&&&0.346&&&\\
&&(0.007&)&&&(0.007&)&&\\
\addlinespace
Firm w/ both pre- and post-AA alumni&&0.480&&&&0.278&&&\\
&&(0.004&)&&&(0.004&)&&\\
\addlinespace
Firm w/ post-AA alumni only&&0.274&&&&0.245&&&\\
&&(0.005&)&&&(0.005&)&&\\
\addlinespace
Employment with general track alum only&&&&0.512&&&&0.334&\\
&&&&(0.004&)&&&(0.004&)\\
\addlinespace
Employment with both general and AA track&&&&0.431&&&&0.270&\\
&&&&(0.005&)&&&(0.005&)\\
\addlinespace
Employment with AA track alum only&&&&0.085&&&&0.106&\\
&&&&(0.009&)&&&(0.008&)\\


==> results/ols_alumni_type_n.tex <==
\(N\)&&549,675&&549,675&&554,242&&554,242&\\


==> results/ols_firm.tex <==
\addlinespace
1 general track alum (1995--2001 cohorts)&&0.298&\sym{***}&&&&&0.221&\sym{***}&0.116&\sym{***}\\
&&(0.005&)&&&&&(0.005&)&(0.005&)\\
\addlinespace
1 general track alum (2004--2011 cohorts)&&&&0.306&\sym{***}&&&0.209&\sym{***}&0.182&\sym{***}\\
&&&&(0.005&)&&&(0.006&)&(0.006&)\\
\addlinespace
1 AA track alum (2004--2011 cohorts)&&&&&&0.218&\sym{***}&0.017&\sym{***}&0.068&\sym{***}\\
&&&&&&(0.005&)&(0.006&)&(0.006&)\\


==> results/ols_firm000.tex <==
\addlinespace
Pre-AA alumni only&&2.422&&0.084&&0.229&&0.109&&0.452&&0.318&\\
&&(0.020&)&(0.004&)&(0.004&)&(0.003&)&(0.007&)&(0.006&)\\
\addlinespace
Both pre- and post-AA alumni&&4.060&&0.182&&0.460&&0.132&&0.466&&0.267&\\
&&(0.015&)&(0.003&)&(0.003&)&(0.002&)&(0.005&)&(0.005&)\\
\addlinespace
Post-AA alumni only&&2.016&&0.168&&0.132&&0.087&&0.267&&0.241&\\
&&(0.016&)&(0.004&)&(0.004&)&(0.002&)&(0.006&)&(0.006&)\\


==> results/ols_firm000_n.tex <==
\(N\)&&480,412&&480,412&&480,412&&474,192&&474,101&&478,217&\\


==> results/ols_firm001.tex <==
\addlinespace
1 general track alum (1995--2001 cohorts)&&0.298&\sym{***}&&&&&0.221&\sym{***}&0.116&\sym{***}\\
&&(0.005&)&&&&&(0.005&)&(0.005&)\\
\addlinespace
1 general track alum (2004--2011 cohorts)&&&&0.306&\sym{***}&&&0.209&\sym{***}&0.182&\sym{***}\\
&&&&(0.005&)&&&(0.006&)&(0.006&)\\
\addlinespace
1 AA track alum (2004--2011 cohorts)&&&&&&0.218&\sym{***}&0.017&\sym{***}&0.068&\sym{***}\\
&&&&&&(0.005&)&(0.006&)&(0.006&)\\


==> results/ols_firm001_n.tex <==
\(N\)&&478,217&&478,217&&478,217&&478,217&&477,918&\\


==> results/ols_firm025.tex <==
\addlinespace
25 general track alumni (1995--2001 cohorts)&&0.143&\sym{***}&&&&&0.164&\sym{***}&0.168&\sym{***}\\
&&(0.011&)&&&&&(0.012&)&(0.011&)\\
\addlinespace
25 general track alumni (2004--2011 cohorts)&&&&0.013&&&&$-$0.016&&0.136&\sym{***}\\
&&&&(0.013&)&&&(0.015&)&(0.014&)\\
\addlinespace
25 AA track alumni (2004--2011 cohorts)&&&&&&$-$0.082&\sym{***}&$-$0.136&\sym{***}&$-$0.004&\\
&&&&&&(0.016&)&(0.018&)&(0.018&)\\


==> results/ols_firm025_n.tex <==
\(N\)&&478,217&&478,217&&478,217&&478,217&&477,918&\\


==> results/ols_firm_n.tex <==
\(N\)&&478,217&&478,217&&478,217&&478,217&&477,918&\\


==> results/ols_firm_p001.tex <==
\addlinespace
1 general track alum (1995--2001 cohorts)&&0.298&\sym{***}&&&&&0.221&\sym{***}&0.116&\sym{***}\\
&&(0.005&)&&&&&(0.005&)&(0.005&)\\
\addlinespace
1 general track alum (2004--2011 cohorts)&&&&0.306&\sym{***}&&&0.209&\sym{***}&0.182&\sym{***}\\
&&&&(0.005&)&&&(0.006&)&(0.006&)\\
\addlinespace
1 AA track alum (2004--2011 cohorts)&&&&&&0.218&\sym{***}&0.017&\sym{***}&0.068&\sym{***}\\
&&&&&&(0.005&)&(0.006&)&(0.006&)\\


==> results/ols_firm_p001_n.tex <==
\(N\)&&478,217&&478,217&&478,217&&478,217&&477,918&\\


==> results/ols_peer.tex <==
\addlinespace
Pre-AA alumni only&&2.658&&0.094&&0.289&&0.143&&0.516&&0.327&\\
&&(0.016&)&(0.004&)&(0.004&)&(0.002&)&(0.005&)&(0.005&)\\
\addlinespace
Both pre- and post-AA alumni&&4.230&&0.202&&0.498&&0.129&&0.486&&0.282&\\
&&(0.015&)&(0.003&)&(0.003&)&(0.002&)&(0.005&)&(0.005&)\\
\addlinespace
Post-AA alumni only&&2.081&&0.160&&0.139&&0.049&&0.199&&0.195&\\
&&(0.019&)&(0.004&)&(0.004&)&(0.003&)&(0.006&)&(0.006&)\\


==> results/ols_peer_n.tex <==
\(N\)&&480,412&&480,412&&480,412&&474,192&&474,101&&478,217&\\


==> results/peer_any_decline.tex <==
Co-employment w/ only UERJ decliners&&0.102&&0.006&&0.131&&0.004&&0.071&&0.040&\sym{*}\\
&&&&(0.017&)&&&(0.024&)&&&(0.024&)\\


==> results/peer_any_enrol_aa.tex <==
Same cohort (AA track)&&&&&&0.165&&0.076&\sym{**}&0.197&&0.059&\sym{**}\\
&&&&&&&&(0.030&)&&&(0.028&)\\


==> results/peer_any_enrol_any.tex <==
Enrollee from any cohort&&0.551&&0.102&\sym{***}&0.533&&0.097&\sym{**}&0.434&&0.139&\sym{***}\\
&&&&(0.036&)&&&(0.041&)&&&(0.035&)\\


==> results/peer_any_enrol_diff.tex <==
Enrollee from different cohort&&0.533&&0.087&\sym{**}&0.523&&0.088&\sym{**}&0.426&&0.115&\sym{***}\\
&&&&(0.036&)&&&(0.041&)&&&(0.035&)\\


==> results/peer_any_enrol_reg.tex <==
Same cohort (regular track)&&0.321&&0.084&\sym{**}&0.193&&0.115&\sym{***}&0.169&&0.053&\sym{**}\\
&&&&(0.035&)&&&(0.033&)&&&(0.027&)\\


==> results/peer_any_enrol_same.tex <==
Enrollee from same cohort&&0.321&&0.084&\sym{**}&0.253&&0.114&\sym{***}&0.249&&0.093&\sym{***}\\
&&&&(0.035&)&&&(0.036&)&&&(0.031&)\\


==> results/peer_any_grad_aa.tex <==
AA track alum (2004--2011 cohorts)&&0.171&&$-$0.026&&0.297&&0.086&\sym{**}&0.286&&0.102&\sym{***}\\
&&&&(0.028&)&&&(0.037&)&&&(0.033&)\\


==> results/peer_any_grad_any.tex <==
Alum from any cohort&&0.464&&0.022&&0.448&&0.044&&0.375&&0.136&\sym{***}\\
&&&&(0.034&)&&&(0.038&)&&&(0.049&)\\


==> results/peer_any_grad_both.tex <==
Both pre- and post-AA alumni&&0.240&&$-$0.023&&0.254&&0.094&\sym{***}&0.259&&0.064&\\
&&&&(0.031&)&&&(0.034&)&&&(0.044&)\\


==> results/peer_any_grad_diff.tex <==
Alum from different cohort&&0.450&&0.020&&0.439&&0.029&&0.367&&0.124&\sym{***}\\
&&&&(0.032&)&&&(0.037&)&&&(0.047&)\\


==> results/peer_any_grad_post.tex <==
Post-AA alumni only&&0.033&&$-$0.004&&0.114&&$-$0.020&&0.088&&0.028&\\
&&&&(0.010&)&&&(0.021&)&&&(0.030&)\\


==> results/peer_any_grad_pre.tex <==
Pre-AA alumni only&&0.191&&0.031&&0.080&&$-$0.013&&0.027&&0.046&\sym{*}\\
&&&&(0.021&)&&&(0.020&)&&&(0.024&)\\


==> results/peer_any_grad_reg.tex <==
Same cohort (regular track)&&0.278&&0.080&\sym{**}&0.151&&0.113&\sym{***}&0.131&&0.045&\sym{*}\\
&&&&(0.033&)&&&(0.029&)&&&(0.024&)\\


==> results/peer_any_grad_same.tex <==
Alum from same cohort&&0.246&&0.021&&0.193&&0.063&\sym{**}&0.208&&0.067&\\
&&&&(0.025&)&&&(0.030&)&&&(0.043&)\\


==> results/peer_any_other.tex <==
Admit to program/cohort who didn't enroll&&0.218&&0.031&&0.185&&0.023&&0.152&&0.009&\\
&&&&(0.031&)&&&(0.033&)&&&(0.032&)\\


==> results/peer_any_uerj.tex <==
UERJ enrollee&&0.247&&0.078&\sym{**}&0.190&&0.117&\sym{***}&0.209&&0.037&\\
&&&&(0.033&)&&&(0.034&)&&&(0.034&)\\


==> results/peer_any_uerj_aa.tex <==
UERJ enrollee from AA track&&&&&&0.119&&0.057&\sym{**}&0.181&&0.016&\\
&&&&&&&&(0.027&)&&&(0.032&)\\


==> results/peer_any_uerj_next.tex <==
Enrollee in \emph{next} cohort of same program&&0.174&&0.041&&0.172&&$-$0.003&&0.180&&$-$0.037&\\
&&&&(0.028&)&&&(0.031&)&&&(0.033&)\\


==> results/peer_any_uerj_reg.tex <==
UERJ enrollee from regular track&&0.247&&0.078&\sym{**}&0.141&&0.101&\sym{***}&0.131&&0.013&\\
&&&&(0.033&)&&&(0.030&)&&&(0.028&)\\


==> results/peer_lwage.tex <==
\addlinespace
Alum from any cohort&&0.373&\sym{***}&&&&&&&0.336&\sym{***}&0.219&\sym{***}\\
&&(0.004&)&&&&&&&(0.004&)&(0.005&)\\
\addlinespace
Alum from same cohort&&&&0.298&\sym{***}&&&&&&&&\\
&&&&(0.005&)&&&&&&&&\\
\addlinespace
Alum from different cohort&&&&&&0.366&\sym{***}&&&&&&\\
&&&&&&(0.004&)&&&&&&\\
\addlinespace
Co-employment w/ UERJ decliners&&&&&&&&0.304&\sym{***}&0.098&\sym{***}&0.026&\sym{***}\\
&&&&&&&&(0.004&)&(0.005&)&(0.005&)\\
\addlinespace
Log establishment size&&&&&&&&&&&&0.057&\sym{***}\\
&&&&&&&&&&&&(0.001&)\\
\addlinespace
Public firm&&&&&&&&&&&&$-$0.118&\sym{***}\\
&&&&&&&&&&&&(0.006&)\\


==> results/peer_lwage_n.tex <==
\(N\)&&478,503&&478,503&&478,503&&478,503&&478,503&&478,503&\\


==> results/peer_n.tex <==
\(N\)&&2,028&&23,433&&2,179&&25,357&&350&&5,748&\\


==> results/prog_list_ctrl.tex <==
Art (RIO), Biological sciences (SGO), Cartographic engineering (RIO), Economics (RIO), General language (SGO), Geography (SGO), Language (English, German, Japanese) (RIO), Language (Spanish, French, Italian) (RIO), Math (RIO), Math (SGO), Mechanical engineering (NF), Oceanography (RIO), Pedagogy (DDC), Pedagogy (RIO), Philosophy (RIO), Physical education (RIO), Physics (RIO), Production engineering (RES), and Statistics (RIO).


==> results/prog_list_trt.tex <==
Accounting (RIO), Biological sciences (RIO), Business administration (RIO), Chemical engineering (RIO), Chemistry (RIO), Computer science (RIO), Dentistry (RIO), General engineering (RIO), Geography (RIO), Geology (RIO), History (RIO), History (SGO), Industrial design (RIO), Journalism (RIO), Language (Greek, Latin, Literature) (RIO), Law (RIO), Mechanical engineering (RIO), Medicine (RIO), Nursing (RIO), Nutrition (RIO), Production engineering (RIO), Psychology (RIO), Social science (RIO), and Social work (RIO).


==> results/rd_anytrack_n10.tex <==
\(N\) (AA track)&&2,242&&27,635&&2,039&&27,482&&277&&3,695&\\


==> results/rd_anytrack_n6.tex <==
\(N\) (AA track)&&2,029&&28,066&&2,698&&36,404&&396&&5,372&\\


==> results/rd_bus_earn_mean10.tex <==
Business&&2,141.009&&$-$272.403&&1,817.477&&10.649&&916.795&&327.743&\\
&&&&(321.195&)&&&(446.266&)&&&(239.378&)\\


==> results/rd_bus_grad_by10.tex <==
Business&&0.000&&0.701&\sym{***}&0.000&&0.692&\sym{***}&0.000&&0.724&\sym{***}\\
&&&&(0.065&)&&&(0.058&)&&&(0.072&)\\


==> results/rd_bus_lwage10.tex <==
Business&&3.674&&$-$0.011&&3.579&&$-$0.054&&2.921&&0.240&\\
&&&&(0.175&)&&&(0.240&)&&&(0.220&)\\


==> results/rd_college_any10.tex <==
Enrolled in any college&&0.877&&0.007&&0.887&&0.027&&0.791&&0.026&\\
&&&&(0.021&)&&&(0.022&)&&&(0.036&)\\


==> results/rd_college_any6.tex <==
Enrolled in any college&&0.831&&0.009&&0.867&&0.023&&0.770&&0.018&\\
&&&&(0.023&)&&&(0.024&)&&&(0.029&)\\


==> results/rd_college_degree10.tex <==
Any college degree, 6-9 years later&&0.822&&0.035&&0.845&&0.009&&0.679&&0.057&\\
&&&&(0.025&)&&&(0.025&)&&&(0.044&)\\


==> results/rd_college_degree10_het3.tex <==
Any college degree, 6-9 years later&&$-$0.017&&0.067&&0.180&\sym{*}&$-$0.069&&0.097&\\
&&(0.177&)&(0.075&)&(0.102&)&(0.098&)&(0.091&)\\


==> results/rd_college_degree6.tex <==
Any college degree, 6-9 years later&&0.731&&0.044&&0.785&&0.006&&0.636&&$-$0.002&\\
&&&&(0.032&)&&&(0.029&)&&&(0.038&)\\


==> results/rd_college_degree6_het3.tex <==
Any college degree, 6-9 years later&&0.014&&0.011&&$-$0.102&&0.019&&0.017&\\
&&(0.134&)&(0.066&)&(0.092&)&(0.085&)&(0.078&)\\


==> results/rd_degree_ever10.tex <==
Ever earned a college degree&&0.911&&0.012&&0.839&&0.026&&0.713&&0.010&\\
&&&&(0.017&)&&&(0.025&)&&&(0.033&)\\


==> results/rd_degree_ever10_het3.tex <==
Ever earned a college degree&&$-$0.030&&0.023&&$-$0.030&&0.032&&0.025&\\
&&(0.125&)&(0.057&)&(0.078&)&(0.077&)&(0.068&)\\


==> results/rd_degree_ever6.tex <==
Ever earned a college degree&&0.911&&0.012&&0.839&&0.026&&0.713&&0.010&\\
&&&&(0.017&)&&&(0.025&)&&&(0.033&)\\


==> results/rd_degree_ever6_het3.tex <==
Ever earned a college degree&&$-$0.030&&0.023&&$-$0.030&&0.032&&0.025&\\
&&(0.125&)&(0.057&)&(0.078&)&(0.077&)&(0.068&)\\


==> results/rd_dif_ind_firm_p000_uerj10.tex <==
Firm w/ any alum and in top 10 industry&&0.465&&0.113&\sym{***}&0.413&&0.070&\sym{*}&0.386&&0.057&\\
&&&&(0.037&)&&&(0.036&)&&&(0.041&)\\


==> results/rd_dif_ind_firm_p000_uerj6.tex <==
Firm w/ any alum and in top 10 industry&&0.450&&0.111&\sym{***}&0.433&&0.082&\sym{**}&0.356&&0.131&\sym{***}\\
&&&&(0.033&)&&&(0.034&)&&&(0.037&)\\


==> results/rd_dif_ind_nofirm_p000_uerj10.tex <==
Firm w/o any alum and in top 10 industry&&0.176&&$-$0.003&&0.207&&0.010&&0.282&&$-$0.061&\\
&&&&(0.029&)&&&(0.032&)&&&(0.038&)\\


==> results/rd_dif_ind_nofirm_p000_uerj6.tex <==
Firm w/o any alum and in top 10 industry&&0.219&&$-$0.033&&0.222&&$-$0.028&&0.268&&$-$0.080&\sym{**}\\
&&&&(0.027&)&&&(0.030&)&&&(0.034&)\\


==> results/rd_dif_ind_nopeer_any_grad_any10.tex <==
No alum from any cohort and in top 10 industry&&0.244&&0.003&&0.257&&0.020&&0.329&&$-$0.058&\\
&&&&(0.028&)&&&(0.032&)&&&(0.037&)\\


==> results/rd_dif_ind_nopeer_any_grad_any6.tex <==
No alum from any cohort and in top 10 industry&&0.285&&$-$0.007&&0.285&&$-$0.031&&0.323&&$-$0.083&\sym{**}\\
&&&&(0.033&)&&&(0.033&)&&&(0.036&)\\


==> results/rd_dif_ind_peer_any_grad_any10.tex <==
Alum from any cohort and in top 10 industry&&0.397&&0.100&\sym{***}&0.364&&0.064&\sym{**}&0.339&&0.066&\sym{*}\\
&&&&(0.032&)&&&(0.033&)&&&(0.036&)\\


==> results/rd_dif_ind_peer_any_grad_any6.tex <==
Alum from any cohort and in top 10 industry&&0.384&&0.098&\sym{***}&0.370&&0.079&\sym{**}&0.301&&0.134&\sym{***}\\
&&&&(0.035&)&&&(0.033&)&&&(0.035&)\\


==> results/rd_earn_dec10.tex <==
December earnings&&2195.293&&$-$127.500&&1859.660&&$-$48.892&&1080.925&&183.945&\sym{*}\\
&&&&(128.122&)&&&(124.013&)&&&(101.352&)\\


==> results/rd_earn_dec6.tex <==
December earnings&&1480.678&&27.796&&1489.572&&$-$212.615&\sym{**}&867.735&&121.743&\sym{**}\\
&&&&(87.986&)&&&(94.253&)&&&(49.943&)\\


==> results/rd_earn_mean10.tex <==
Monthly earnings (2019 USD)&&2,005.191&&$-$84.946&&1,757.947&&$-$99.418&&1,041.942&&56.577&\\
&&&&(94.587&)&&&(109.084&)&&&(75.202&)\\


==> results/rd_earn_mean10_1.tex <==
Monthly earnings (2019 USD)&&$-$84.105&&$-$83.191&&30.639&&$-$115.173&&$-$85.290&\\
&&(94.586&)&(145.009&)&(73.007&)&(135.201&)&(94.117&)\\


==> results/rd_earn_mean10_2.tex <==
Monthly earnings (2019 USD)&&$-$102.941&&$-$231.406&&$-$53.098&&$-$33.774&&$-$100.881&\\
&&(109.073&)&(152.445&)&(89.843&)&(135.372&)&(108.029&)\\


==> results/rd_earn_mean10_het_aa.tex <==
Monthly earnings (2019 USD)&&37.737&&79.456&&26.215&&95.455&&148.320&&101.785&\\
&&(79.470&)&(133.529&)&(150.950&)&(83.812&)&(166.719&)&(180.614&)\\


==> results/rd_earn_mean10_het_aaf.tex <==
Monthly earnings (2019 USD)&&233.633&&43.341&&$-$139.594&&63.304&\\
&&(158.928&)&(160.279&)&(163.390&)&(127.643&)\\


==> results/rd_earn_mean10_het_gen.tex <==
Monthly earnings (2019 USD)&&224.497&&$-$70.038&&$-$135.233&&$-$55.991&&101.482&&55.567&&124.023&&118.760&&108.352&&$-$337.930&\\
&&(165.980&)&(197.008&)&(183.367&)&(127.920&)&(139.544&)&(322.886&)&(163.636&)&(215.240&)&(155.813&)&(382.584&)\\


==> results/rd_earn_mean6.tex <==
Monthly earnings (2019 USD)&&1,356.069&&0.295&&1,390.819&&$-$153.473&\sym{**}&816.821&&110.230&\sym{**}\\
&&&&(75.313&)&&&(77.290&)&&&(49.546&)\\


==> results/rd_earn_mean6_1.tex <==
Monthly earnings (2019 USD)&&0.440&&103.639&&66.956&&$-$30.020&&$-$2.036&\\
&&(75.269&)&(114.267&)&(57.390&)&(92.678&)&(74.054&)\\


==> results/rd_earn_mean6_2.tex <==
Monthly earnings (2019 USD)&&$-$163.811&\sym{**}&$-$223.150&\sym{**}&$-$75.055&&$-$106.698&&$-$157.841&\sym{**}\\
&&(77.383&)&(105.344&)&(63.181&)&(97.113&)&(76.054&)\\


==> results/rd_earn_mean6_het_aa.tex <==
Monthly earnings (2019 USD)&&109.677&\sym{*}&89.337&&72.744&&75.737&&18.654&&79.434&\\
&&(56.031&)&(84.528&)&(108.673&)&(54.515&)&(102.980&)&(94.744&)\\


==> results/rd_earn_mean6_het_aaf.tex <==
Monthly earnings (2019 USD)&&211.265&\sym{*}&105.882&&55.910&&87.951&\\
&&(116.896&)&(87.709&)&(113.028&)&(78.088&)\\


==> results/rd_earn_mean6_het_gen.tex <==
Monthly earnings (2019 USD)&&$-$163.477&&$-$192.921&&$-$222.168&\sym{*}&$-$37.808&&$-$225.958&\sym{**}&198.425&&$-$239.665&\sym{*}&$-$114.015&&$-$188.005&\sym{*}&4.759&\\
&&(110.557&)&(152.983&)&(129.046&)&(89.698&)&(93.842&)&(258.677&)&(125.429&)&(135.318&)&(97.153&)&(239.141&)\\


==> results/rd_enrol.tex <==
Enrolled in UERJ program&&0.003&&0.313&\sym{***}&0.008&&0.292&\sym{***}&0.004&&0.689&\sym{***}\\
&&&&(0.010&)&&&(0.006&)&&&(0.014&)\\


==> results/rd_enrol_1.tex <==
Enrolled in UERJ program&&0.313&\sym{***}&0.354&\sym{***}&0.311&\sym{***}&0.253&\sym{***}&0.310&\sym{***}\\
&&(0.010&)&(0.014&)&(0.008&)&(0.021&)&(0.010&)\\


==> results/rd_enrol_2.tex <==
Enrolled in UERJ program&&0.292&\sym{***}&0.288&\sym{***}&0.295&\sym{***}&0.296&\sym{***}&0.292&\sym{***}\\
&&(0.006&)&(0.008&)&(0.005&)&(0.008&)&(0.006&)\\


==> results/rd_enrol_het_aa.tex <==
Enrolled in UERJ program&&0.668&\sym{***}&0.737&\sym{***}&0.688&\sym{***}&0.700&\sym{***}&0.780&\sym{***}&0.710&\sym{***}\\
&&(0.018&)&(0.020&)&(0.022&)&(0.017&)&(0.023&)&(0.029&)\\


==> results/rd_enrol_het_aaf.tex <==
Enrolled in UERJ program&&0.711&\sym{***}&0.723&\sym{***}&0.707&\sym{***}&0.650&\sym{***}\\
&&(0.028&)&(0.034&)&(0.028&)&(0.023&)\\


==> results/rd_enrol_het_gen.tex <==
Enrolled in UERJ program&&0.293&\sym{***}&0.291&\sym{***}&0.291&\sym{***}&0.292&\sym{***}&0.291&\sym{***}&0.322&\sym{***}&0.305&\sym{***}&0.281&\sym{***}&0.301&\sym{***}&0.243&\sym{***}\\
&&(0.010&)&(0.016&)&(0.009&)&(0.009&)&(0.009&)&(0.024&)&(0.011&)&(0.012&)&(0.009&)&(0.027&)\\


==> results/rd_est_shr_coll.tex <==
Firm share of employees w/ college degree&&0.429&&0.031&\sym{*}&0.502&&$-$0.022&&0.405&&0.016&\\
&&&&(0.018&)&&&(0.022&)&&&(0.023&)\\


==> results/rd_est_shr_coll10.tex <==
Firm share of employees w/ college degree&&0.503&&0.027&&0.551&&0.002&&0.477&&0.029&\\
&&&&(0.018&)&&&(0.019&)&&&(0.028&)\\


==> results/rd_est_shr_coll6.tex <==
Firm share of employees w/ college degree&&0.428&&0.030&\sym{*}&0.507&&$-$0.008&&0.414&&0.008&\\
&&&&(0.018&)&&&(0.018&)&&&(0.023&)\\


==> results/rd_est_shr_white.tex <==
Prop. of co-workers who are white&&0.716&&0.021&&0.636&&0.012&&0.592&&$-$0.004&\\
&&&&(0.019&)&&&(0.019&)&&&(0.024&)\\


==> results/rd_est_shr_white10.tex <==
Prop. of co-workers who are white&&0.702&&0.046&\sym{***}&0.615&&0.022&&0.574&&0.017&\\
&&&&(0.017&)&&&(0.021&)&&&(0.025&)\\


==> results/rd_est_shr_white6.tex <==
Prop. of co-workers who are white&&0.716&&0.019&&0.629&&0.000&&0.582&&0.023&\\
&&&&(0.019&)&&&(0.017&)&&&(0.022&)\\


==> results/rd_firm_any_alum10.tex <==
Employed at firm with any &&0.649&&0.059&\sym{*}&0.573&&0.028&&0.498&&0.080&\sym{*}\\
\quad UERJ alum&&&&(0.033&)&&&(0.037&)&&&(0.044&)\\


==> results/rd_firm_any_alum6.tex <==
Employed at firm with any  &&0.600&&0.118&\sym{***}&0.572&&0.070&\sym{**}&0.477&&0.137&\sym{***}\\
\quad UERJ alum&&&&(0.033&)&&&(0.034&)&&&(0.038&)\\


==> results/rd_firm_any_alum_aa10.tex <==
Employed at firm with any &&0.411&&0.032&&0.384&&0.056&&0.383&&0.082&\sym{*}\\
\quad AA track alum&&&&(0.034&)&&&(0.036&)&&&(0.044&)\\


==> results/rd_firm_any_alum_aa6.tex <==
Employed at firm with any &&0.375&&0.036&&0.402&&0.076&\sym{**}&0.386&&0.129&\sym{***}\\
\quad AA track alum&&&&(0.031&)&&&(0.033&)&&&(0.037&)\\


==> results/rd_firm_any_alum_gen10.tex <==
Employed at firm with any &&0.629&&0.060&&0.550&&0.014&&0.451&&0.086&\sym{**}\\
\quad general track alum&&&&(0.037&)&&&(0.038&)&&&(0.039&)\\


==> results/rd_firm_any_alum_gen6.tex <==
Employed at firm with any &&0.579&&0.129&\sym{***}&0.540&&0.076&\sym{**}&0.437&&0.106&\sym{***}\\
\quad general track alum&&&&(0.035&)&&&(0.034&)&&&(0.035&)\\


==> results/rd_firm_n10_bus.tex <==
\(N\) (any alum)&&573&&5,816&&404&&4,973&&81&&1,039&\\


==> results/rd_firm_n10_gov.tex <==
\(N\) (any alum)&&1,003&&10,413&&761&&9,649&&117&&1,587&\\


==> results/rd_firm_n10_hea.tex <==
\(N\) (any alum)&&441&&4,323&&475&&5,520&&42&&766&\\


==> results/rd_firm_n10_hum.tex <==
\(N\) (any alum)&&621&&6,587&&481&&7,134&&86&&1,471&\\


==> results/rd_firm_n10_nsci.tex <==
\(N\) (any alum)&&607&&6,596&&679&&9,944&&68&&903&\\


==> results/rd_firm_n10_priv.tex <==
\(N\) (any alum)&&1,239&&12,909&&1,278&&17,921&&160&&2,583&\\


==> results/rd_firm_n6_bus.tex <==
\(N\) (any alum)&&539&&6,519&&514&&6,035&&116&&1,333&\\


==> results/rd_firm_n6_gov.tex <==
\(N\) (any alum)&&742&&9,429&&781&&9,656&&128&&1,621&\\


==> results/rd_firm_n6_hea.tex <==
\(N\) (any alum)&&366&&4,361&&600&&6,503&&58&&886&\\


==> results/rd_firm_n6_hum.tex <==
\(N\) (any alum)&&570&&7,245&&651&&9,113&&126&&1,637&\\


==> results/rd_firm_n6_nsci.tex <==
\(N\) (any alum)&&554&&7,361&&933&&12,476&&96&&1,204&\\


==> results/rd_firm_n6_priv.tex <==
\(N\) (any alum)&&1,287&&16,057&&1,917&&24,470&&268&&3,409&\\


==> results/rd_firmtrack_n10.tex <==
\(N\) (AA track)&&2,242&&27,647&&2,039&&27,535&&277&&3,730&\\


==> results/rd_firmtrack_n6.tex <==
\(N\) (AA track)&&2,029&&28,526&&2,698&&36,705&&396&&5,073&\\


==> results/rd_gov_firm.tex <==
Publicly-owned firm&&0.365&&0.015&&0.293&&0.028&&0.334&&0.036&\\
&&&&(0.036&)&&&(0.035&)&&&(0.042&)\\


==> results/rd_gov_firm10.tex <==
Publicly-owned firm&&0.447&&$-$0.013&&0.373&&0.037&&0.422&&0.032&\\
&&&&(0.035&)&&&(0.034&)&&&(0.038&)\\


==> results/rd_gov_firm6.tex <==
Publicly-owned firm&&0.366&&0.016&&0.289&&0.005&&0.323&&0.051&\\
&&&&(0.036&)&&&(0.030&)&&&(0.039&)\\


==> results/rd_grad.tex <==
Graduated from UERJ program&&0.002&&0.228&\sym{***}&0.003&&0.196&\sym{***}&0.004&&0.457&\sym{***}\\
&&&&(0.008&)&&&(0.006&)&&&(0.015&)\\


==> results/rd_grad_by10.tex <==
Graduated from UERJ program&&0.002&&0.718&\sym{***}&0.003&&0.693&\sym{***}&0.003&&0.661&\sym{***}\\
&&&&(0.017&)&&&(0.014&)&&&(0.021&)\\


==> results/rd_grad_by10_1.tex <==
Graduated from UERJ program&&0.718&\sym{***}&0.729&\sym{***}&0.729&\sym{***}&0.709&\sym{***}&0.720&\sym{***}\\
&&(0.017&)&(0.022&)&(0.015&)&(0.038&)&(0.017&)\\


==> results/rd_grad_by10_2.tex <==
Graduated from UERJ program&&0.693&\sym{***}&0.658&\sym{***}&0.709&\sym{***}&0.736&\sym{***}&0.694&\sym{***}\\
&&(0.014&)&(0.019&)&(0.012&)&(0.019&)&(0.014&)\\


==> results/rd_grad_by10_het_aa.tex <==
Graduated from UERJ program&&0.663&\sym{***}&0.655&\sym{***}&0.578&\sym{***}&0.734&\sym{***}&0.706&\sym{***}&0.667&\sym{***}\\
&&(0.027&)&(0.034&)&(0.036&)&(0.027&)&(0.037&)&(0.048&)\\


==> results/rd_grad_by10_het_aaf.tex <==
Graduated from UERJ program&&0.803&\sym{***}&0.557&\sym{***}&0.479&\sym{***}&0.718&\sym{***}\\
&&(0.036&)&(0.053&)&(0.049&)&(0.036&)\\


==> results/rd_grad_by10_het_gen.tex <==
Graduated from UERJ program&&0.666&\sym{***}&0.633&\sym{***}&0.654&\sym{***}&0.741&\sym{***}&0.681&\sym{***}&0.601&\sym{***}&0.700&\sym{***}&0.611&\sym{***}&0.667&\sym{***}&0.610&\sym{***}\\
&&(0.024&)&(0.039&)&(0.020&)&(0.018&)&(0.023&)&(0.062&)&(0.025&)&(0.037&)&(0.021&)&(0.087&)\\


==> results/rd_grad_by6.tex <==
Graduated from UERJ program&&0.002&&0.711&\sym{***}&0.003&&0.677&\sym{***}&0.004&&0.640&\sym{***}\\
&&&&(0.017&)&&&(0.013&)&&&(0.018&)\\


==> results/rd_grad_by6_1.tex <==
Graduated from UERJ program&&0.711&\sym{***}&0.708&\sym{***}&0.719&\sym{***}&0.714&\sym{***}&0.713&\sym{***}\\
&&(0.017&)&(0.022&)&(0.015&)&(0.037&)&(0.017&)\\


==> results/rd_grad_by6_2.tex <==
Graduated from UERJ program&&0.677&\sym{***}&0.647&\sym{***}&0.684&\sym{***}&0.715&\sym{***}&0.677&\sym{***}\\
&&(0.013&)&(0.017&)&(0.011&)&(0.016&)&(0.013&)\\


==> results/rd_grad_by6_het_aa.tex <==
Graduated from UERJ program&&0.648&\sym{***}&0.627&\sym{***}&0.574&\sym{***}&0.685&\sym{***}&0.674&\sym{***}&0.625&\sym{***}\\
&&(0.023&)&(0.026&)&(0.031&)&(0.021&)&(0.027&)&(0.039&)\\


==> results/rd_grad_by6_het_aaf.tex <==
Graduated from UERJ program&&0.794&\sym{***}&0.525&\sym{***}&0.418&\sym{***}&0.714&\sym{***}\\
&&(0.030&)&(0.047&)&(0.039&)&(0.030&)\\


==> results/rd_grad_by6_het_gen.tex <==
Graduated from UERJ program&&0.681&\sym{***}&0.608&\sym{***}&0.627&\sym{***}&0.728&\sym{***}&0.672&\sym{***}&0.556&\sym{***}&0.710&\sym{***}&0.610&\sym{***}&0.668&\sym{***}&0.663&\sym{***}\\
&&(0.019&)&(0.030&)&(0.017&)&(0.016&)&(0.019&)&(0.052&)&(0.020&)&(0.025&)&(0.017&)&(0.069&)\\


==> results/rd_grad_degree_ever10.tex <==
Ever earned a graduate degree&&0.107&&$-$0.004&&0.069&&$-$0.017&&0.051&&$-$0.006&\\
&&&&(0.020&)&&&(0.017&)&&&(0.015&)\\


==> results/rd_grad_degree_ever10_het3.tex <==
Ever earned a graduate degree&&$-$0.082&\sym{*}&0.007&&$-$0.002&&$-$0.017&&0.013&\\
&&(0.044&)&(0.038&)&(0.042&)&(0.030&)&(0.025&)\\


==> results/rd_grad_degree_ever6.tex <==
Ever earned a graduate degree&&0.107&&$-$0.004&&0.069&&$-$0.017&&0.051&&$-$0.006&\\
&&&&(0.020&)&&&(0.017&)&&&(0.015&)\\


==> results/rd_grad_degree_ever6_het3.tex <==
Ever earned a graduate degree&&$-$0.082&\sym{*}&0.007&&$-$0.002&&$-$0.017&&0.013&\\
&&(0.044&)&(0.038&)&(0.042&)&(0.030&)&(0.025&)\\


==> results/rd_hea_earn_mean10.tex <==
Health&&1,562.531&&$-$51.214&&1,710.640&&$-$206.845&&1,241.718&&243.571&\\
&&&&(158.744&)&&&(199.739&)&&&(159.063&)\\


==> results/rd_hea_grad_by10.tex <==
Health&&0.003&&0.882&\sym{***}&0.000&&0.873&\sym{***}&0.012&&0.803&\sym{***}\\
&&&&(0.025&)&&&(0.024&)&&&(0.036&)\\


==> results/rd_hea_lwage10.tex <==
Health&&3.607&&0.162&&3.888&&$-$0.034&&3.294&&0.172&\\
&&&&(0.101&)&&&(0.136&)&&&(0.127&)\\


==> results/rd_hum_earn_mean10.tex <==
Humanities&&1,306.508&&9.033&&1,413.584&&16.748&&908.999&&17.347&\\
&&&&(218.515&)&&&(277.283&)&&&(157.375&)\\


==> results/rd_hum_grad_by10.tex <==
Humanities&&0.008&&0.604&\sym{***}&0.003&&0.555&\sym{***}&0.000&&0.556&\sym{***}\\
&&&&(0.046&)&&&(0.047&)&&&(0.053&)\\


==> results/rd_hum_lwage10.tex <==
Humanities&&3.245&&$-$0.072&&3.396&&0.133&&2.923&&0.025&\\
&&&&(0.161&)&&&(0.183&)&&&(0.145&)\\


==> results/rd_in_rais10.tex <==
Formal employment&&0.693&&0.032&&0.686&&$-$0.026&&0.714&&0.037&\\
&&&&(0.027&)&&&(0.031&)&&&(0.039&)\\


==> results/rd_in_rais10_1.tex <==
Formal employment &&0.032&&0.033&&0.042&\sym{**}&$-$0.003&&$-$0.008&\\
&&(0.027&)&(0.039&)&(0.021&)&(0.039&)&(0.014&)\\


==> results/rd_in_rais10_2.tex <==
Formal employment &&$-$0.026&&0.008&&$-$0.007&&$-$0.035&&$-$0.008&\\
&&(0.031&)&(0.043&)&(0.026&)&(0.037&)&(0.021&)\\


==> results/rd_in_rais10_het_aa.tex <==
Formal employment &&0.040&&0.015&&0.093&&$-$0.007&&0.122&&$-$0.010&\\
&&(0.047&)&(0.057&)&(0.066&)&(0.048&)&(0.086&)&(0.100&)\\


==> results/rd_in_rais10_het_aaf.tex <==
Formal employment &&$-$0.046&&$-$0.016&&0.122&&0.038&\\
&&(0.073&)&(0.086&)&(0.080&)&(0.065&)\\


==> results/rd_in_rais10_het_gen.tex <==
Formal employment &&0.009&&$-$0.079&&$-$0.064&&0.029&&0.001&&$-$0.119&&$-$0.028&&$-$0.033&&0.012&&$-$0.011&\\
&&(0.056&)&(0.091&)&(0.042&)&(0.043&)&(0.047&)&(0.133&)&(0.061&)&(0.084&)&(0.045&)&(0.217&)\\


==> results/rd_in_rais6.tex <==
Formal employment&&0.627&&0.064&\sym{**}&0.672&&$-$0.031&&0.729&&$-$0.002&\\
&&&&(0.029&)&&&(0.027&)&&&(0.026&)\\


==> results/rd_in_rais6_1.tex <==
Formal employment &&0.064&\sym{**}&0.104&\sym{**}&0.072&\sym{***}&0.059&&0.016&\\
&&(0.029&)&(0.042&)&(0.022&)&(0.043&)&(0.019&)\\


==> results/rd_in_rais6_2.tex <==
Formal employment &&$-$0.030&&$-$0.029&&$-$0.025&&$-$0.061&\sym{*}&0.012&\\
&&(0.027&)&(0.038&)&(0.022&)&(0.033&)&(0.016&)\\


==> results/rd_in_rais6_het_aa.tex <==
Formal employment &&0.025&&$-$0.031&&0.012&&$-$0.008&&0.059&&0.028&\\
&&(0.032&)&(0.041&)&(0.053&)&(0.034&)&(0.054&)&(0.064&)\\


==> results/rd_in_rais6_het_aaf.tex <==
Formal employment &&$-$0.045&&0.127&\sym{*}&$-$0.057&&$-$0.023&\\
&&(0.062&)&(0.070&)&(0.064&)&(0.051&)\\


==> results/rd_in_rais6_het_gen.tex <==
Formal employment &&0.016&&$-$0.010&&$-$0.063&&$-$0.000&&0.013&&$-$0.053&&0.033&&$-$0.044&&$-$0.003&&$-$0.051&\\
&&(0.038&)&(0.068&)&(0.038&)&(0.036&)&(0.034&)&(0.096&)&(0.042&)&(0.052&)&(0.036&)&(0.149&)\\


==> results/rd_ind_wage16.tex <==
Industry wage 1&&3.177&&$-$0.012&&3.164&&$-$0.017&&3.124&&$-$0.002&\\
&&&&(0.015&)&&&(0.019&)&&&(0.021&)\\


==> results/rd_ind_wage26.tex <==
Industry wage 2&&3.187&&$-$0.013&&3.151&&$-$0.050&\sym{*}&3.064&&0.027&\\
&&&&(0.031&)&&&(0.028&)&&&(0.030&)\\


==> results/rd_ind_wage36.tex <==
Industry wage 3&&3.205&&0.017&&3.185&&$-$0.047&&3.020&&0.023&\\
&&&&(0.029&)&&&(0.033&)&&&(0.035&)\\


==> results/rd_ind_wage56.tex <==
Industry wage 5&&3.219&&0.009&&3.201&&$-$0.023&&3.000&&0.044&\\
&&&&(0.031&)&&&(0.037&)&&&(0.036&)\\


==> results/rd_iv_grad.tex <==
Graduated from UERJ program&&0.721&\sym{***}&0.686&\sym{***}&0.658&\sym{***}&0.655&\sym{***}&0.657&\sym{***}\\
&&(0.017&)&(0.013&)&(0.022&)&(0.026&)&(0.017&)\\


==> results/rd_iv_lwage10.tex <==
Log hourly wage&&0.004&&$-$0.051&&0.047&&0.224&\sym{*}&0.121&\\
&&(0.052&)&(0.074&)&(0.122&)&(0.136&)&(0.091&)\\


==> results/rd_iv_lwage6.tex <==
Log hourly wage&&0.013&&$-$0.093&&0.123&\sym{*}&0.204&\sym{**}&0.152&\sym{***}\\
&&(0.044&)&(0.058&)&(0.066&)&(0.090&)&(0.053&)\\


==> results/rd_learn_annual10.tex <==
Log annual earnings&&11.006&&$-$0.001&&10.867&&$-$0.015&&10.439&&$-$0.065&\\
&&&&(0.020&)&&&(0.020&)&&&(0.058&)\\


==> results/rd_learn_annual6.tex <==
Log annual earnings&&10.535&&$-$0.013&&10.537&&$-$0.011&&10.015&&0.038&\\
&&&&(0.022&)&&&(0.019&)&&&(0.048&)\\


==> results/rd_learn_annual_tot10.tex <==
Log total annual earnings&&11.193&&0.003&&11.021&&$-$0.013&&10.625&&$-$0.060&\\
&&&&(0.019&)&&&(0.019&)&&&(0.059&)\\


==> results/rd_learn_annual_tot6.tex <==
Log total annual earnings&&10.698&&$-$0.004&&10.681&&$-$0.019&&10.188&&0.079&\\
&&&&(0.021&)&&&(0.019&)&&&(0.054&)\\


==> results/rd_learn_dec10.tex <==
Log December earnings&&8.777&&$-$0.003&&8.704&&$-$0.048&&8.203&&0.041&\\
&&&&(0.053&)&&&(0.059&)&&&(0.069&)\\


==> results/rd_learn_dec6.tex <==
Log December earnings&&8.390&&0.014&&8.478&&$-$0.098&\sym{**}&7.953&&0.094&\sym{*}\\
&&&&(0.050&)&&&(0.048&)&&&(0.050&)\\


==> results/rd_learn_final10.tex <==
Log last earnings received by worker&&5.993&&$-$0.011&&8.554&&$-$0.017&&8.049&&0.046&\\
&&&&(0.031&)&&&(0.020&)&&&(0.055&)\\


==> results/rd_learn_final6.tex <==
Log last earnings received by worker&&2.566&&0.005&&8.063&&$-$0.023&&7.458&&0.143&\sym{**}\\
&&&&(0.017&)&&&(0.025&)&&&(0.061&)\\


==> results/rd_learn_mean10.tex <==
Log average monthly earnings&&8.694&&0.023&&8.651&&$-$0.036&&8.162&&$-$0.023&\\
&&&&(0.052&)&&&(0.056&)&&&(0.066&)\\


==> results/rd_learn_mean6.tex <==
Log average monthly earnings&&8.315&&0.003&&8.405&&$-$0.074&&7.899&&0.076&\\
&&&&(0.044&)&&&(0.048&)&&&(0.047&)\\


==> results/rd_lest_mean_wage.tex <==
Firm mean hourly wage (log)&&3.225&&0.019&&3.414&&$-$0.074&&2.996&&0.116&\sym{*}\\
&&&&(0.046&)&&&(0.060&)&&&(0.067&)\\


==> results/rd_lest_size.tex <==
Firm number of employees (log)&&6.635&&$-$0.040&&6.352&&0.361&\sym{**}&6.389&&0.100&\\
&&&&(0.195&)&&&(0.182&)&&&(0.241&)\\


==> results/rd_lest_size10.tex <==
Firm number of employees (log)&&6.807&&$-$0.253&&6.425&&0.190&&6.453&&0.286&\\
&&&&(0.183&)&&&(0.194&)&&&(0.226&)\\


==> results/rd_lest_size6.tex <==
Firm number of employees (log)&&6.363&&$-$0.066&&6.047&&0.170&&6.025&&0.016&\\
&&&&(0.188&)&&&(0.163&)&&&(0.206&)\\


==> results/rd_lfirm_size.tex <==
Log firm number of employees&&8.140&&$-$0.389&\sym{*}&7.894&&$-$0.229&&7.743&&$-$0.020&\\
&&&&(0.216&)&&&(0.231&)&&&(0.305&)\\


==> results/rd_lfirm_size10.tex <==
Log firm number of employees&&$-$0.148&\sym{**}&$-$0.024&&0.140&&0.267&&0.193&\\
&&(0.061&)&(0.078&)&(0.284&)&(0.373&)&(0.225&)\\


==> results/rd_lfirm_size6.tex <==
Log firm number of employees&&$-$0.114&\sym{*}&$-$0.046&&$-$0.029&&$-$0.178&&$-$0.074&\\
&&(0.059&)&(0.060&)&(0.194&)&(0.263&)&(0.156&)\\


==> results/rd_lhired_hours10.tex <==
Log hired hours&&0.001&&$-$0.007&&$-$0.020&&0.000&&$-$0.011&\\
&&(0.006&)&(0.009&)&(0.026&)&(0.037&)&(0.021&)\\


==> results/rd_lhired_hours6.tex <==
Log hired hours&&0.011&&$-$0.002&&$-$0.021&&$-$0.046&\sym{*}&$-$0.029&\sym{*}\\
&&(0.008&)&(0.007&)&(0.019&)&(0.028&)&(0.016&)\\


==> results/rd_lwage10.tex <==
Log hourly wage&&3.636&&0.005&&3.637&&0.005&&3.052&&0.024&\\
&&&&(0.054&)&&&(0.058&)&&&(0.063&)\\


==> results/rd_lwage10_1.tex <==
Log hourly wage&&0.005&&$-$0.037&&0.018&&0.006&&0.004&\\
&&(0.054&)&(0.077&)&(0.041&)&(0.060&)&(0.054&)\\


==> results/rd_lwage10_2.tex <==
Log hourly wage&&0.011&&$-$0.072&&$-$0.022&&0.049&&0.010&\\
&&(0.057&)&(0.081&)&(0.048&)&(0.068&)&(0.057&)\\


==> results/rd_lwage10_het_aa.tex <==
Log hourly wage&&$-$0.015&&0.066&&0.031&&0.058&&0.054&&$-$0.045&\\
&&(0.084&)&(0.126&)&(0.123&)&(0.076&)&(0.176&)&(0.169&)\\


==> results/rd_lwage10_het_aaf.tex <==
Log hourly wage&&0.220&\sym{*}&$-$0.021&&$-$0.073&&$-$0.048&\\
&&(0.133&)&(0.151&)&(0.140&)&(0.114&)\\


==> results/rd_lwage10_het_gen.tex <==
Log hourly wage&&0.025&&$-$0.018&&0.109&&$-$0.041&&0.090&&$-$0.113&&0.033&&0.078&&0.015&&$-$0.069&\\
&&(0.090&)&(0.144&)&(0.085&)&(0.070&)&(0.092&)&(0.182&)&(0.111&)&(0.131&)&(0.098&)&(0.329&)\\


==> results/rd_lwage6.tex <==
Log hourly wage&&3.237&&$-$0.003&&3.387&&$-$0.079&&2.813&&0.132&\sym{***}\\
&&&&(0.050&)&&&(0.049&)&&&(0.044&)\\


==> results/rd_lwage6_1.tex <==
Log hourly wage&&$-$0.004&&0.012&&0.027&&$-$0.004&&$-$0.006&\\
&&(0.050&)&(0.074&)&(0.038&)&(0.055&)&(0.049&)\\


==> results/rd_lwage6_2.tex <==
Log hourly wage&&$-$0.080&&$-$0.123&\sym{*}&$-$0.038&&$-$0.046&&$-$0.081&\sym{*}\\
&&(0.049&)&(0.069&)&(0.041&)&(0.057&)&(0.049&)\\


==> results/rd_lwage6_het_aa.tex <==
Log hourly wage&&0.077&&0.153&\sym{*}&0.062&&0.138&\sym{**}&0.053&&0.091&\\
&&(0.060&)&(0.080&)&(0.091&)&(0.059&)&(0.094&)&(0.113&)\\


==> results/rd_lwage6_het_aaf.tex <==
Log hourly wage&&0.199&\sym{*}&0.116&&0.005&&0.093&\\
&&(0.102&)&(0.121&)&(0.110&)&(0.087&)\\


==> results/rd_lwage6_het_gen.tex <==
Log hourly wage&&$-$0.128&\sym{*}&0.119&&$-$0.156&\sym{*}&$-$0.029&&$-$0.079&&0.051&&$-$0.159&\sym{*}&$-$0.021&&$-$0.126&\sym{*}&0.128&\\
&&(0.074&)&(0.100&)&(0.081&)&(0.070&)&(0.065&)&(0.161&)&(0.084&)&(0.093&)&(0.067&)&(0.244&)\\


==> results/rd_n.tex <==
\(N\) (applicants)&&17,519&&47,013&&3,920&&2,310&&6,230&\\


==> results/rd_n_college_degree10.tex <==
\(N\)&&2,242&&27,575&&2,039&&35,551&&277&&3,787&\\


==> results/rd_n_college_degree6.tex <==
\(N\)&&2,029&&23,251&&2,698&&33,837&&396&&5,119&\\


==> results/rd_n_degree_ever10.tex <==
\(N\) (ever college degree)&&2,417&&32,718&&2,925&&36,617&&415&&5,978&\\


==> results/rd_n_degree_ever6.tex <==
\(N\) (ever college degree)&&2,417&&32,718&&2,925&&36,617&&415&&5,978&\\


==> results/rd_n_enrol.tex <==
\(N\)&&3,234&&17,519&&4,012&&47,838&&543&&6,121&\\


==> results/rd_n_enrol_1.tex <==
\(N\)&&17,519&&8,880&&25,848&&9,101&&17,519&\\


==> results/rd_n_enrol_2.tex <==
\(N\)&&47,838&&24,477&&69,856&&36,957&&47,838&\\


==> results/rd_n_enrol_het_aa.tex <==
\(N\)&&4,208&&2,664&&2,614&&4,639&&1,916&&1,589&\\


==> results/rd_n_enrol_het_aaf.tex <==
\(N\)&&1,512&&1,025&&1,374&&2,550&\\


==> results/rd_n_enrol_het_gen.tex <==
\(N\)&&17,325&&7,446&&22,096&&22,356&&22,636&&3,683&&14,806&&12,942&&21,638&&2,599&\\


==> results/rd_n_in_rais10.tex <==
\(N\) (formal employment)&&3,234&&39,134&&2,974&&41,138&&388&&4,320&\\


==> results/rd_n_in_rais10_1.tex <==
\(N\) (employment regression)&&39,133&&21,003&&53,108&&31,666&&39,133&\\


==> results/rd_n_in_rais10_2.tex <==
\(N\) (employment regression)&&41,128&&21,285&&59,285&&34,320&&41,128&\\


==> results/rd_n_in_rais10_het_aa.tex <==
\(N\) (employment regression)&&3,107&&1,765&&1,617&&2,919&&841&&789&\\


==> results/rd_n_in_rais10_het_aaf.tex <==
\(N\) (employment regression)&&1,114&&782&&906&&1,898&\\


==> results/rd_n_in_rais10_het_gen.tex <==
\(N\) (employment regression)&&13,136&&5,322&&21,835&&20,812&&18,206&&1,934&&9,923&&6,849&&18,738&&1,792&\\


==> results/rd_n_in_rais6.tex <==
\(N\) (formal employment)&&3,234&&37,794&&4,012&&55,030&&543&&8,147&\\


==> results/rd_n_in_rais6_1.tex <==
\(N\) (employment regression)&&37,794&&20,162&&51,674&&29,030&&37,794&\\


==> results/rd_n_in_rais6_2.tex <==
\(N\) (employment regression)&&55,110&&28,308&&80,093&&45,622&&55,110&\\


==> results/rd_n_in_rais6_het_aa.tex <==
\(N\) (employment regression)&&5,313&&3,038&&2,298&&4,799&&1,912&&1,651&\\


==> results/rd_n_in_rais6_het_aaf.tex <==
\(N\) (employment regression)&&1,512&&1,025&&1,374&&2,550&\\


==> results/rd_n_in_rais6_het_gen.tex <==
\(N\) (employment regression)&&25,465&&9,101&&26,572&&29,771&&32,566&&3,935&&21,100&&15,183&&29,568&&3,060&\\


==> results/rd_n_lwage10.tex <==
\(N\) (log hourly wage)&&2,237&&24,273&&2,021&&26,407&&273&&3,746&\\


==> results/rd_n_lwage10_1.tex <==
\(N\) (wage regression)&&24,273&&12,851&&33,695&&24,847&&24,273&\\


==> results/rd_n_lwage10_2.tex <==
\(N\) (wage regression)&&26,540&&13,748&&38,220&&23,707&&26,540&\\


==> results/rd_n_lwage10_het_aa.tex <==
\(N\) (wage regression)&&2,149&&977&&1,207&&2,507&&390&&499&\\


==> results/rd_n_lwage10_het_aaf.tex <==
\(N\) (wage regression)&&822&&575&&671&&1,346&\\


==> results/rd_n_lwage10_het_gen.tex <==
\(N\) (wage regression)&&8,743&&3,518&&13,219&&16,600&&9,529&&1,549&&5,832&&5,482&&7,742&&1,349&\\


==> results/rd_n_lwage6.tex <==
\(N\) (log hourly wage)&&2,027&&24,564&&2,694&&32,972&&394&&6,100&\\


==> results/rd_n_lwage6_1.tex <==
\(N\) (wage regression)&&24,567&&13,140&&33,612&&24,481&&24,567&\\


==> results/rd_n_lwage6_2.tex <==
\(N\) (wage regression)&&32,966&&16,930&&47,911&&31,844&&32,966&\\


==> results/rd_n_lwage6_het_aa.tex <==
\(N\) (wage regression)&&3,499&&1,765&&1,827&&3,367&&1,225&&1,119&\\


==> results/rd_n_lwage6_het_aaf.tex <==
\(N\) (wage regression)&&1,098&&798&&1,026&&1,869&\\


==> results/rd_n_lwage6_het_gen.tex <==
\(N\) (wage regression)&&14,710&&7,976&&13,297&&15,566&&19,283&&2,637&&10,624&&10,086&&16,818&&1,882&\\


==> results/rd_n_panel10.tex <==
\(N\) (applicant/years)&&3,234&&39,133&&2,974&&41,128&&388&&4,320&\\


==> results/rd_n_panel6.tex <==
\(N\) (applicant/years)&&3,234&&37,794&&4,012&&55,110&&543&&8,147&\\


==> results/rd_n_rais10.tex <==
\(N\) (wage observations)&&3,234&&24,287&&2,974&&25,446&&388&&4,138&\\


==> results/rd_n_rais6.tex <==
\(N\) (wage observations)&&3,234&&25,648&&4,012&&32,760&&543&&5,906&\\


==> results/rd_nodif_ind_firm_p000_uerj10.tex <==
Firm w/ any alum and not top 10 industry&&0.185&&$-$0.061&\sym{**}&0.160&&$-$0.045&&0.112&&0.023&\\
&&&&(0.029&)&&&(0.028&)&&&(0.030&)\\


==> results/rd_nodif_ind_firm_p000_uerj6.tex <==
Firm w/ any alum and not top 10 industry&&0.149&&0.004&&0.139&&$-$0.012&&0.121&&0.006&\\
&&&&(0.024&)&&&(0.025&)&&&(0.027&)\\


==> results/rd_nodif_ind_nofirm_p000_uerj10.tex <==
Firm w/o any alum and not top 10 industry&&0.175&&$-$0.049&\sym{*}&0.219&&$-$0.035&&0.220&&$-$0.019&\\
&&&&(0.029&)&&&(0.033&)&&&(0.038&)\\


==> results/rd_nodif_ind_nofirm_p000_uerj6.tex <==
Firm w/o any alum and not top 10 industry&&0.181&&$-$0.082&\sym{***}&0.206&&$-$0.042&&0.255&&$-$0.057&\sym{*}\\
&&&&(0.026&)&&&(0.029&)&&&(0.034&)\\


==> results/rd_nodif_ind_nopeer_any_grad_any10.tex <==
No alum from any cohort and not top 10 industry&&0.212&&$-$0.055&\sym{**}&0.252&&$-$0.068&\sym{**}&0.242&&$-$0.034&\\
&&&&(0.027&)&&&(0.032&)&&&(0.036&)\\


==> results/rd_nodif_ind_nopeer_any_grad_any6.tex <==
No alum from any cohort and not top 10 industry&&0.222&&$-$0.097&\sym{***}&0.242&&$-$0.061&\sym{**}&0.285&&$-$0.052&\\
&&&&(0.030&)&&&(0.031&)&&&(0.035&)\\


==> results/rd_nodif_ind_peer_any_grad_any10.tex <==
Alum from any cohort and not top 10 industry&&0.147&&$-$0.047&\sym{**}&0.127&&$-$0.016&&0.090&&0.026&\\
&&&&(0.024&)&&&(0.024&)&&&(0.025&)\\


==> results/rd_nodif_ind_peer_any_grad_any6.tex <==
Alum from any cohort and not top 10 industry&&0.109&&0.006&&0.103&&0.012&&0.091&&0.002&\\
&&&&(0.023&)&&&(0.023&)&&&(0.024&)\\


==> results/rd_notop_ind_firm_p000_uerj10.tex <==
Firm w/ any alum and in not top 10 industry&&0.062&&$-$0.029&&0.051&&0.007&&0.014&&0.007&\\
&&&&(0.019&)&&&(0.018&)&&&(0.016&)\\


==> results/rd_notop_ind_firm_p000_uerj6.tex <==
Firm w/ any alum and in not top 10 industry&&0.041&&0.013&&0.052&&$-$0.011&&0.018&&0.019&\\
&&&&(0.015&)&&&(0.016&)&&&(0.015&)\\


==> results/rd_notop_ind_nofirm_p000_uerj10.tex <==
Firm w/o any alum and in not top 10 industry&&0.087&&$-$0.020&&0.112&&$-$0.046&\sym{*}&0.101&&$-$0.041&\\
&&&&(0.021&)&&&(0.025&)&&&(0.030&)\\


==> results/rd_notop_ind_nofirm_p000_uerj6.tex <==
Firm w/o any alum and in not top 10 industry&&0.084&&$-$0.045&\sym{**}&0.097&&$-$0.028&&0.111&&$-$0.014&\\
&&&&(0.019&)&&&(0.022&)&&&(0.026&)\\


==> results/rd_notop_ind_nopeer_any_grad_any10.tex <==
No alum from any cohort and not top 10 industry&&0.100&&$-$0.016&&0.122&&$-$0.027&&0.101&&$-$0.038&\\
&&&&(0.019&)&&&(0.024&)&&&(0.028&)\\


==> results/rd_notop_ind_nopeer_any_grad_any6.tex <==
No alum from any cohort and not top 10 industry&&0.097&&$-$0.044&\sym{**}&0.109&&$-$0.043&\sym{*}&0.116&&$-$0.007&\\
&&&&(0.021&)&&&(0.023&)&&&(0.027&)\\


==> results/rd_notop_ind_peer_any_grad_any10.tex <==
Alum from any cohort and not top 10 industry&&0.049&&$-$0.016&&0.041&&$-$0.007&&0.014&&0.006&\\
&&&&(0.015&)&&&(0.015&)&&&(0.012&)\\


==> results/rd_notop_ind_peer_any_grad_any6.tex <==
Alum from any cohort and not top 10 industry&&0.029&&$-$0.000&&0.039&&0.004&&0.013&&0.010&\\
&&&&(0.014&)&&&(0.015&)&&&(0.013&)\\


==> results/rd_nsci_earn_mean10.tex <==
Natural sciences&&2,193.274&&41.254&&1,709.673&&$-$461.246&\sym{**}&961.058&&$-$153.081&\\
&&&&(237.112&)&&&(223.651&)&&&(163.135&)\\


==> results/rd_nsci_grad_by10.tex <==
Naturalsciences&&0.000&&0.573&\sym{***}&0.007&&0.542&\sym{***}&0.000&&0.482&\sym{***}\\
&&&&(0.039&)&&&(0.030&)&&&(0.048&)\\


==> results/rd_nsci_lwage10.tex <==
Naturalsciences&&3.757&&0.035&&3.513&&$-$0.123&&2.923&&$-$0.055&\\
&&&&(0.139&)&&&(0.133&)&&&(0.133&)\\


==> results/rd_occ_wage110.tex <==
Occupation wage 1&&0.111&&$-$0.005&&0.161&&0.002&&0.038&&$-$0.049&\\
&&&&(0.023&)&&&(0.023&)&&&(0.039&)\\


==> results/rd_occ_wage16.tex <==
Occupation wage 1&&3.187&&0.039&&3.270&&$-$0.001&&3.112&&0.005&\\
&&&&(0.026&)&&&(0.027&)&&&(0.034&)\\


==> results/rd_occ_wage210.tex <==
Occupation wage 2&&0.166&&0.032&&0.207&&$-$0.003&&0.012&&$-$0.022&\\
&&&&(0.026&)&&&(0.028&)&&&(0.039&)\\


==> results/rd_occ_wage26.tex <==
Occupation wage 2&&3.247&&0.063&\sym{*}&3.314&&$-$0.003&&3.071&&0.025&\\
&&&&(0.032&)&&&(0.032&)&&&(0.037&)\\


==> results/rd_occ_wage310.tex <==
Occupation wage 3&&0.204&&0.010&&0.289&&0.002&&0.011&&$-$0.037&\\
&&&&(0.030&)&&&(0.036&)&&&(0.045&)\\


==> results/rd_occ_wage36.tex <==
Occupation wage 3&&3.233&&0.029&&3.382&&$-$0.042&&3.061&&0.037&\\
&&&&(0.032&)&&&(0.037&)&&&(0.041&)\\


==> results/rd_occ_wage510.tex <==
Occupation wage 5&&0.287&&0.002&&0.318&&$-$0.015&&$-$0.027&&$-$0.070&\\
&&&&(0.038&)&&&(0.041&)&&&(0.049&)\\


==> results/rd_occ_wage56.tex <==
Occupation wage 5&&3.280&&0.023&&3.396&&$-$0.062&&3.004&&0.041&\\
&&&&(0.036&)&&&(0.041&)&&&(0.042&)\\


==> results/rd_occ_wage610.tex <==
Occupation wage 6&&0.290&&0.010&&0.318&&$-$0.015&&$-$0.031&&$-$0.050&\\
&&&&(0.038&)&&&(0.041&)&&&(0.049&)\\


==> results/rd_occ_wage66.tex <==
Occupation wage 6&&3.276&&0.020&&3.399&&$-$0.053&&2.998&&0.050&\\
&&&&(0.037&)&&&(0.041&)&&&(0.042&)\\


==> results/rd_pcttrack_n10.tex <==
\(N\) (AA track)&&2,242&&28,941&&2,039&&40,005&&277&&3,818&\\


==> results/rd_pcttrack_n6.tex <==
\(N\) (AA track)&&2,029&&32,665&&2,698&&38,670&&396&&5,242&\\


==> results/rd_peer_any_decline10.tex <==
Co-employment w/ only UERJ decliners&&0.177&&0.004&&0.190&&0.010&&0.126&&0.047&\\
&&&&(0.025&)&&&(0.031&)&&&(0.033&)\\


==> results/rd_peer_any_decline6.tex <==
Co-employment w/ only UERJ decliners&&0.178&&$-$0.006&&0.213&&$-$0.044&&0.149&&0.030&\\
&&&&(0.028&)&&&(0.028&)&&&(0.028&)\\


==> results/rd_peer_any_grad_aa10.tex <==
Alum from AA track&&0.269&&$-$0.017&&0.323&&0.063&\sym{**}&0.310&&0.080&\\
&&&&(0.031&)&&&(0.032&)&&&(0.050&)\\


==> results/rd_peer_any_grad_aa6.tex <==
Alum from AA track&&0.171&&$-$0.010&&0.320&&0.067&\sym{**}&0.306&&0.094&\sym{***}\\
&&&&(0.024&)&&&(0.031&)&&&(0.030&)\\


==> results/rd_peer_any_grad_after10.tex <==
Alum hired after applicant&&0.407&&0.029&&0.308&&0.062&\sym{*}&0.325&&0.030&\\
&&&&(0.034&)&&&(0.036&)&&&(0.045&)\\


==> results/rd_peer_any_grad_after6.tex <==
Alum hired after applicant&&0.312&&0.036&&0.256&&0.045&&0.247&&0.046&\\
&&&&(0.033&)&&&(0.032&)&&&(0.034&)\\


==> results/rd_peer_any_grad_any10.tex <==
Alum from any cohort&&0.544&&0.052&&0.491&&0.048&&0.430&&0.092&\sym{**}\\
&&&&(0.033&)&&&(0.035&)&&&(0.039&)\\


==> results/rd_peer_any_grad_any10_bus.tex <==
Business&&0.670&&$-$0.025&&0.621&&0.039&&0.494&&$-$0.066&\\
&&&&(0.046&)&&&(0.046&)&&&(0.089&)\\


==> results/rd_peer_any_grad_any10_gov.tex <==
Gov't Firm&&0.761&&0.039&&0.715&&0.018&&0.735&&$-$0.007&\\
&&&&(0.037&)&&&(0.044&)&&&(0.054&)\\


==> results/rd_peer_any_grad_any10_hea.tex <==
Health&&0.594&&0.096&&0.669&&0.184&\sym{**}&0.500&&0.205&\sym{***}\\
&&&&(0.073&)&&&(0.082&)&&&(0.078&)\\


==> results/rd_peer_any_grad_any10_hum.tex <==
Humanities&&0.446&&0.043&&0.393&&$-$0.032&&0.488&&0.080&\\
&&&&(0.071&)&&&(0.087&)&&&(0.071&)\\


==> results/rd_peer_any_grad_any10_nsci.tex <==
Natural science&&0.488&&0.176&\sym{**}&0.358&&0.054&&0.235&&0.169&\sym{**}\\
&&&&(0.088&)&&&(0.081&)&&&(0.077&)\\


==> results/rd_peer_any_grad_any10_priv.tex <==
Private Firm&&0.368&&0.078&&0.358&&0.035&&0.206&&0.135&\sym{***}\\
&&&&(0.048&)&&&(0.047&)&&&(0.042&)\\


==> results/rd_peer_any_grad_any6.tex <==
Alum from any cohort&&0.493&&0.104&\sym{***}&0.473&&0.092&\sym{***}&0.391&&0.135&\sym{***}\\
&&&&(0.036&)&&&(0.035&)&&&(0.038&)\\


==> results/rd_peer_any_grad_any6_bus.tex <==
Business&&0.584&&0.062&&0.582&&0.005&&0.440&&0.163&\sym{*}\\
&&&&(0.051&)&&&(0.052&)&&&(0.084&)\\


==> results/rd_peer_any_grad_any6_gov.tex <==
Gov't Firm&&0.749&&0.027&&0.722&&0.027&&0.797&&0.042&\\
&&&&(0.044&)&&&(0.050&)&&&(0.056&)\\


==> results/rd_peer_any_grad_any6_hea.tex <==
Health&&0.527&&0.161&\sym{*}&0.683&&0.121&\sym{*}&0.483&&0.308&\sym{***}\\
&&&&(0.088&)&&&(0.069&)&&&(0.071&)\\


==> results/rd_peer_any_grad_any6_hum.tex <==
Humanities&&0.393&&0.068&&0.341&&0.081&&0.397&&0.059&\\
&&&&(0.075&)&&&(0.086&)&&&(0.071&)\\


==> results/rd_peer_any_grad_any6_nsci.tex <==
Natural science&&0.484&&0.177&\sym{*}&0.370&&0.193&\sym{**}&0.271&&0.064&\\
&&&&(0.094&)&&&(0.079&)&&&(0.076&)\\


==> results/rd_peer_any_grad_any6_priv.tex <==
Private Firm&&0.345&&0.147&\sym{***}&0.371&&0.108&\sym{**}&0.198&&0.154&\sym{***}\\
&&&&(0.048&)&&&(0.043&)&&&(0.040&)\\


==> results/rd_peer_any_grad_anyp10.tex <==
Co-employment any program&&0.828&&0.014&&0.780&&0.059&\sym{*}&0.722&&0.067&\sym{*}\\
&&&&(0.028&)&&&(0.031&)&&&(0.040&)\\


==> results/rd_peer_any_grad_anyp6.tex <==
Co-employment any program&&0.788&&0.001&&0.765&&0.085&\sym{***}&0.679&&0.073&\sym{**}\\
&&&&(0.031&)&&&(0.031&)&&&(0.035&)\\


==> results/rd_peer_any_grad_before10.tex <==
Alum hired before applicant&&0.389&&0.036&&0.390&&$-$0.002&&0.329&&0.067&\\
&&&&(0.034&)&&&(0.036&)&&&(0.042&)\\


==> results/rd_peer_any_grad_before6.tex <==
Alum hired before applicant&&0.345&&0.041&&0.372&&0.069&\sym{**}&0.313&&0.103&\sym{***}\\
&&&&(0.033&)&&&(0.032&)&&&(0.034&)\\


==> results/rd_peer_any_grad_both10.tex <==
Both pre- and post-AA alumni&&0.315&&$-$0.028&&0.282&&0.083&\sym{***}&0.278&&0.058&\\
&&&&(0.035&)&&&(0.032&)&&&(0.042&)\\


==> results/rd_peer_any_grad_both6.tex <==
Both pre- and post-AA alumni&&0.212&&$-$0.011&&0.282&&0.035&&0.253&&0.035&\\
&&&&(0.031&)&&&(0.030&)&&&(0.033&)\\


==> results/rd_peer_any_grad_diff10.tex <==
Alum from different cohort&&0.531&&0.054&\sym{*}&0.480&&0.033&&0.422&&0.066&\sym{*}\\
&&&&(0.032&)&&&(0.034&)&&&(0.039&)\\


==> results/rd_peer_any_grad_diff6.tex <==
Alum from different cohort&&0.474&&0.081&\sym{**}&0.461&&0.083&\sym{**}&0.391&&0.104&\sym{***}\\
&&&&(0.035&)&&&(0.035&)&&&(0.037&)\\


==> results/rd_peer_any_grad_diffg_diffp10.tex <==
Co-employment different program, different field&&0.760&&$-$0.021&&0.680&&0.064&&0.664&&0.040&\\
&&&&(0.033&)&&&(0.041&)&&&(0.050&)\\


==> results/rd_peer_any_grad_diffg_diffp6.tex <==
Co-employment different program, different field&&0.696&&$-$0.042&&0.664&&0.064&\sym{*}&0.629&&0.038&\\
&&&&(0.031&)&&&(0.035&)&&&(0.041&)\\


==> results/rd_peer_any_grad_diffp10.tex <==
Co-employment different program&&0.810&&0.015&&0.753&&0.073&\sym{*}&0.693&&0.067&\\
&&&&(0.031&)&&&(0.038&)&&&(0.047&)\\


==> results/rd_peer_any_grad_diffp6.tex <==
Co-employment different program&&0.762&&$-$0.016&&0.741&&0.080&\sym{**}&0.669&&0.036&\\
&&&&(0.032&)&&&(0.035&)&&&(0.036&)\\


==> results/rd_peer_any_grad_diffp_m110.tex <==
enrol&&0.462&&0.017&&0.475&&$-$0.009&&0.455&&0.071&\\
&&&&(0.029&)&&&(0.041&)&&&(0.051&)\\


==> results/rd_peer_any_grad_diffp_m16.tex <==
enrol&&0.425&&$-$0.000&&0.412&&0.008&&0.396&&0.042&\\
&&&&(0.031&)&&&(0.029&)&&&(0.041&)\\


==> results/rd_peer_any_grad_diffp_m210.tex <==
enrol&&0.382&&$-$0.025&&0.470&&0.001&&0.466&&$-$0.002&\\
&&&&(0.030&)&&&(0.041&)&&&(0.050&)\\


==> results/rd_peer_any_grad_diffp_m26.tex <==
enrol&&0.336&&0.002&&0.349&&$-$0.021&&0.338&&0.022&\\
&&&&(0.026&)&&&(0.030&)&&&(0.034&)\\


==> results/rd_peer_any_grad_diffp_m310.tex <==
enrol&&0.426&&$-$0.065&\sym{**}&0.403&&0.008&&0.419&&0.103&\sym{**}\\
&&&&(0.031&)&&&(0.037&)&&&(0.048&)\\


==> results/rd_peer_any_grad_diffp_m36.tex <==
enrol&&0.353&&$-$0.041&&0.261&&0.007&&0.275&&0.042&\\
&&&&(0.033&)&&&(0.029&)&&&(0.033&)\\


==> results/rd_peer_any_grad_diffp_p010.tex <==
enrol&&0.601&&$-$0.049&&0.468&&0.047&&0.469&&0.063&\\
&&&&(0.038&)&&&(0.041&)&&&(0.056&)\\


==> results/rd_peer_any_grad_diffp_p06.tex <==
enrol&&0.552&&$-$0.015&&0.463&&0.079&\sym{**}&0.452&&0.072&\sym{*}\\
&&&&(0.038&)&&&(0.034&)&&&(0.042&)\\


==> results/rd_peer_any_grad_diffp_p110.tex <==
enrol&&0.523&&$-$0.013&&0.376&&0.000&&0.282&&0.033&\\
&&&&(0.034&)&&&(0.037&)&&&(0.038&)\\


==> results/rd_peer_any_grad_diffp_p16.tex <==
enrol&&0.495&&$-$0.018&&0.406&&0.037&&0.326&&0.007&\\
&&&&(0.029&)&&&(0.034&)&&&(0.033&)\\


==> results/rd_peer_any_grad_diffp_p210.tex <==
enrol&&0.435&&$-$0.019&&0.296&&0.003&&0.224&&0.043&\\
&&&&(0.030&)&&&(0.033&)&&&(0.033&)\\


==> results/rd_peer_any_grad_diffp_p26.tex <==
enrol&&0.432&&$-$0.044&\sym{*}&0.336&&0.009&&0.283&&0.034&\\
&&&&(0.025&)&&&(0.026&)&&&(0.028&)\\


==> results/rd_peer_any_grad_diffp_p310.tex <==
enrol&&0.373&&$-$0.028&&0.280&&0.009&&0.339&&0.030&\\
&&&&(0.028&)&&&(0.029&)&&&(0.040&)\\


==> results/rd_peer_any_grad_diffp_p36.tex <==
enrol&&0.360&&0.009&&0.335&&0.033&&0.346&&0.051&\\
&&&&(0.028&)&&&(0.031&)&&&(0.038&)\\


==> results/rd_peer_any_grad_gen10.tex <==
Alum from post-AA general track&&0.293&&$-$0.026&&0.348&&0.078&\sym{**}&0.336&&0.056&\\
&&&&(0.035&)&&&(0.032&)&&&(0.041&)\\


==> results/rd_peer_any_grad_gen6.tex <==
Alum from post-AA general track&&0.187&&$-$0.002&&0.344&&0.082&\sym{**}&0.283&&0.084&\sym{**}\\
&&&&(0.031&)&&&(0.033&)&&&(0.041&)\\


==> results/rd_peer_any_grad_m110.tex <==
Co-employment w/ alum cohort c = -1&&0.430&&0.032&&0.484&&0.006&&0.397&&0.067&\\
&&&&(0.031&)&&&(0.041&)&&&(0.048&)\\


==> results/rd_peer_any_grad_m16.tex <==
Co-employment w/ alum cohort c = -1&&0.421&&0.011&&0.451&&0.024&&0.412&&0.065&\sym{*}\\
&&&&(0.032&)&&&(0.032&)&&&(0.037&)\\


==> results/rd_peer_any_grad_m210.tex <==
Co-employment w/ alum cohort c = -2&&0.363&&$-$0.006&&0.488&&0.006&&0.426&&0.020&\\
&&&&(0.029&)&&&(0.039&)&&&(0.049&)\\


==> results/rd_peer_any_grad_m26.tex <==
Co-employment w/ alum cohort c = -2&&0.338&&0.007&&0.375&&0.026&&0.343&&0.039&\\
&&&&(0.025&)&&&(0.031&)&&&(0.033&)\\


==> results/rd_peer_any_grad_m310.tex <==
Co-employment w/ alum cohort c = -3&&0.409&&$-$0.019&&0.429&&0.029&&0.412&&0.120&\sym{**}\\
&&&&(0.026&)&&&(0.037&)&&&(0.051&)\\


==> results/rd_peer_any_grad_m36.tex <==
Co-employment w/ alum cohort c = -3&&0.366&&$-$0.013&&0.281&&0.036&&0.280&&0.050&\\
&&&&(0.032&)&&&(0.029&)&&&(0.034&)\\


==> results/rd_peer_any_grad_p010.tex <==
Co-employment w/ alum cohort c = +0&&0.571&&$-$0.019&&0.474&&0.070&\sym{*}&0.390&&0.094&\sym{*}\\
&&&&(0.036&)&&&(0.038&)&&&(0.050&)\\


==> results/rd_peer_any_grad_p06.tex <==
Co-employment w/ alum cohort c = +0&&0.540&&0.026&&0.496&&0.119&\sym{***}&0.434&&0.087&\sym{**}\\
&&&&(0.038&)&&&(0.032&)&&&(0.041&)\\


==> results/rd_peer_any_grad_p110.tex <==
Co-employment w/ alum cohort c = +1&&0.496&&0.000&&0.367&&0.021&&0.231&&0.042&\\
&&&&(0.034&)&&&(0.035&)&&&(0.037&)\\


==> results/rd_peer_any_grad_p16.tex <==
Co-employment w/ alum cohort c = +1&&0.487&&$-$0.009&&0.424&&0.049&&0.313&&0.055&\sym{*}\\
&&&&(0.031&)&&&(0.033&)&&&(0.030&)\\


==> results/rd_peer_any_grad_p210.tex <==
Co-employment w/ alum cohort c = +2&&0.413&&0.007&&0.292&&0.010&&0.181&&0.061&\sym{*}\\
&&&&(0.031&)&&&(0.032&)&&&(0.032&)\\


==> results/rd_peer_any_grad_p26.tex <==
Co-employment w/ alum cohort c = +2&&0.414&&$-$0.026&&0.342&&0.014&&0.258&&0.052&\sym{*}\\
&&&&(0.027&)&&&(0.027&)&&&(0.031&)\\


==> results/rd_peer_any_grad_p310.tex <==
Co-employment w/ alum cohort c = +3&&0.358&&$-$0.018&&0.279&&0.019&&0.260&&0.015&\\
&&&&(0.028&)&&&(0.027&)&&&(0.038&)\\


==> results/rd_peer_any_grad_p36.tex <==
Co-employment w/ alum cohort c = +3&&0.343&&0.038&&0.347&&0.057&\sym{*}&0.308&&0.036&\\
&&&&(0.028&)&&&(0.032&)&&&(0.033&)\\


==> results/rd_peer_any_grad_post10.tex <==
Post-AA alumni only&&0.066&&$-$0.007&&0.168&&0.002&&0.144&&0.055&\\
&&&&(0.018&)&&&(0.031&)&&&(0.037&)\\


==> results/rd_peer_any_grad_post6.tex <==
Post-AA alumni only&&0.041&&$-$0.002&&0.182&&0.046&\sym{*}&0.146&&0.117&\sym{***}\\
&&&&(0.015&)&&&(0.025&)&&&(0.034&)\\


==> results/rd_peer_any_grad_pre10.tex <==
Alum from pre-AA general track&&0.500&&0.060&\sym{*}&0.365&&0.046&&0.310&&0.078&\sym{*}\\
&&&&(0.035&)&&&(0.036&)&&&(0.044&)\\


==> results/rd_peer_any_grad_pre6.tex <==
Alum from pre-AA general track&&0.462&&0.104&\sym{***}&0.352&&0.033&&0.288&&0.078&\sym{**}\\
&&&&(0.035&)&&&(0.033&)&&&(0.033&)\\


==> results/rd_peer_any_grad_same10.tex <==
Alum from same cohort&&0.305&&0.030&&0.224&&0.074&\sym{**}&0.235&&0.068&\sym{*}\\
&&&&(0.030&)&&&(0.030&)&&&(0.039&)\\


==> results/rd_peer_any_grad_same6.tex <==
Alum from same cohort&&0.278&&0.062&\sym{**}&0.219&&0.099&\sym{***}&0.205&&0.091&\sym{***}\\
&&&&(0.031&)&&&(0.027&)&&&(0.027&)\\


==> results/rd_peer_any_grad_sameg_diffp10.tex <==
Co-employment different program, same field&&0.680&&0.017&&0.623&&0.078&\sym{**}&0.531&&0.098&\sym{*}\\
&&&&(0.032&)&&&(0.040&)&&&(0.050&)\\


==> results/rd_peer_any_grad_sameg_diffp6.tex <==
Co-employment different program, same field&&0.643&&0.020&&0.625&&0.052&&0.520&&0.106&\sym{***}\\
&&&&(0.039&)&&&(0.033&)&&&(0.035&)\\


==> results/rd_peer_any_grad_samep10.tex <==
Co-employment same program&&0.544&&0.052&&0.491&&0.048&&0.430&&0.092&\sym{**}\\
&&&&(0.033&)&&&(0.035&)&&&(0.039&)\\


==> results/rd_peer_any_grad_samep6.tex <==
Co-employment same program&&0.493&&0.104&\sym{***}&0.473&&0.092&\sym{***}&0.391&&0.135&\sym{***}\\
&&&&(0.036&)&&&(0.035&)&&&(0.038&)\\


==> results/rd_peer_any_grad_samep_m110.tex <==
Same program, c = -1&&0.244&&0.040&&0.209&&0.058&\sym{**}&0.249&&0.041&\\
&&&&(0.029&)&&&(0.027&)&&&(0.039&)\\


==> results/rd_peer_any_grad_samep_m16.tex <==
Same program, c = -1&&0.206&&0.041&&0.185&&0.034&&0.172&&0.039&\\
&&&&(0.028&)&&&(0.026&)&&&(0.029&)\\


==> results/rd_peer_any_grad_samep_m210.tex <==
Same program, c = -2&&0.191&&0.047&\sym{*}&0.203&&0.035&&0.224&&0.029&\\
&&&&(0.025&)&&&(0.028&)&&&(0.042&)\\


==> results/rd_peer_any_grad_samep_m26.tex <==
Same program, c = -2&&0.155&&0.030&&0.135&&0.040&\sym{*}&0.146&&0.023&\\
&&&&(0.026&)&&&(0.021&)&&&(0.027&)\\


==> results/rd_peer_any_grad_samep_m310.tex <==
Same program, c = -3&&0.207&&0.008&&0.170&&0.066&\sym{**}&0.173&&0.069&\sym{**}\\
&&&&(0.029&)&&&(0.028&)&&&(0.034&)\\


==> results/rd_peer_any_grad_samep_m36.tex <==
Same program, c = -3&&0.151&&$-$0.001&&0.093&&0.028&&0.098&&0.051&\sym{**}\\
&&&&(0.026&)&&&(0.019&)&&&(0.022&)\\


==> results/rd_peer_any_grad_samep_p010.tex <==
Same program, c = +0&&0.305&&0.030&&0.224&&0.074&\sym{**}&0.235&&0.068&\sym{*}\\
&&&&(0.030&)&&&(0.030&)&&&(0.039&)\\


==> results/rd_peer_any_grad_samep_p06.tex <==
Same program, c = +0&&0.278&&0.062&\sym{**}&0.219&&0.099&\sym{***}&0.205&&0.091&\sym{***}\\
&&&&(0.031&)&&&(0.027&)&&&(0.027&)\\


==> results/rd_peer_any_grad_samep_p110.tex <==
Same program, c = +1&&0.267&&0.023&&0.166&&0.001&&0.119&&0.021&\\
&&&&(0.030&)&&&(0.028&)&&&(0.033&)\\


==> results/rd_peer_any_grad_samep_p16.tex <==
Same program, c = +1&&0.256&&0.031&&0.191&&0.012&&0.149&&0.052&\sym{**}\\
&&&&(0.034&)&&&(0.027&)&&&(0.025&)\\


==> results/rd_peer_any_grad_samep_p210.tex <==
Same program, c = +2&&0.217&&0.034&&0.122&&0.012&&0.097&&0.037&\\
&&&&(0.028&)&&&(0.022&)&&&(0.028&)\\


==> results/rd_peer_any_grad_samep_p26.tex <==
Same program, c = +2&&0.215&&0.037&&0.142&&0.024&&0.131&&0.016&\\
&&&&(0.028&)&&&(0.024&)&&&(0.025&)\\


==> results/rd_peer_any_grad_samep_p310.tex <==
Same program, c = +3&&0.185&&0.013&&0.134&&0.050&\sym{**}&0.155&&$-$0.006&\\
&&&&(0.022&)&&&(0.025&)&&&(0.036&)\\


==> results/rd_peer_any_grad_samep_p36.tex <==
Same program, c = +3&&0.174&&0.025&&0.160&&0.077&\sym{***}&0.159&&0.040&\\
&&&&(0.026&)&&&(0.027&)&&&(0.026&)\\


==> results/rd_peer_n10.tex <==
\(N\) (any cohort)&&2,242&&27,492&&2,039&&31,289&&277&&4,718&\\


==> results/rd_peer_n10_bus.tex <==
\(N\) (any cohort)&&573&&6,870&&404&&5,657&&81&&1,173&\\


==> results/rd_peer_n10_gov.tex <==
\(N\) (any cohort)&&1,003&&12,237&&761&&10,895&&117&&1,786&\\


==> results/rd_peer_n10_hea.tex <==
\(N\) (any cohort)&&441&&5,060&&475&&6,251&&42&&869&\\


==> results/rd_peer_n10_hum.tex <==
\(N\) (any cohort)&&621&&7,682&&481&&8,105&&86&&1,671&\\


==> results/rd_peer_n10_nsci.tex <==
\(N\) (any cohort)&&607&&7,880&&679&&11,276&&68&&1,005&\\


==> results/rd_peer_n10_priv.tex <==
\(N\) (any cohort)&&1,239&&15,255&&1,278&&20,394&&160&&2,925&\\


==> results/rd_peer_n6.tex <==
\(N\) (any cohort)&&2,029&&23,565&&2,698&&32,909&&396&&5,009&\\


==> results/rd_peer_n6_bus.tex <==
\(N\) (any cohort)&&539&&6,022&&514&&5,792&&116&&1,317&\\


==> results/rd_peer_n6_gov.tex <==
\(N\) (any cohort)&&742&&8,703&&781&&9,305&&128&&1,599&\\


==> results/rd_peer_n6_hea.tex <==
\(N\) (any cohort)&&366&&4,030&&600&&6,285&&58&&883&\\


==> results/rd_peer_n6_hum.tex <==
\(N\) (any cohort)&&570&&6,759&&651&&8,789&&126&&1,618&\\


==> results/rd_peer_n6_nsci.tex <==
\(N\) (any cohort)&&554&&6,754&&933&&12,043&&96&&1,191&\\


==> results/rd_peer_n6_priv.tex <==
\(N\) (any cohort)&&1,287&&14,862&&1,917&&23,603&&268&&3,380&\\


==> results/rd_peer_n_grad_diffg_diffp10.tex <==
Co-employment different program, different field&&87.255&&$-$26.083&\sym{*}&89.037&&7.066&&146.628&&42.918&\\
&&&&(14.692&)&&&(25.747&)&&&(43.296&)\\


==> results/rd_peer_n_grad_diffg_diffp6.tex <==
Co-employment different program, different field&&62.888&&$-$11.596&&62.447&&$-$3.543&&126.561&&4.073&\\
&&&&(13.765&)&&&(14.619&)&&&(33.375&)\\


==> results/rd_peer_n_grad_diffp10.tex <==
Co-employment different program&&165.165&&$-$14.241&&137.770&&$-$8.932&&319.357&&3.802&\\
&&&&(32.848&)&&&(39.486&)&&&(64.728&)\\


==> results/rd_peer_n_grad_diffp6.tex <==
Co-employment different program&&110.428&&$-$19.229&&102.649&&19.042&&243.543&&$-$28.659&\\
&&&&(18.217&)&&&(26.583&)&&&(48.325&)\\


==> results/rd_peer_n_grad_diffp_m110.tex <==
enrol&&14.447&&0.785&&9.072&&1.006&&23.130&&2.605&\\
&&&&(2.865&)&&&(2.587&)&&&(4.991&)\\


==> results/rd_peer_n_grad_diffp_m16.tex <==
enrol&&11.287&&0.050&&5.352&&0.120&&13.674&&$-$1.700&\\
&&&&(2.334&)&&&(1.527&)&&&(2.855&)\\


==> results/rd_peer_n_grad_diffp_m210.tex <==
enrol&&12.404&&0.756&&7.359&&1.119&&17.841&&1.451&\\
&&&&(2.385&)&&&(2.173&)&&&(4.021&)\\


==> results/rd_peer_n_grad_diffp_m26.tex <==
enrol&&7.861&&0.809&&3.777&&0.915&&9.356&&$-$1.644&\\
&&&&(1.595&)&&&(1.148&)&&&(2.121&)\\


==> results/rd_peer_n_grad_diffp_m310.tex <==
enrol&&13.446&&$-$3.452&&5.654&&0.911&&13.379&&1.692&\\
&&&&(2.900&)&&&(1.702&)&&&(3.236&)\\


==> results/rd_peer_n_grad_diffp_m36.tex <==
enrol&&7.147&&$-$1.135&&2.496&&0.478&&6.227&&$-$0.546&\\
&&&&(1.577&)&&&(0.845&)&&&(1.383&)\\


==> results/rd_peer_n_grad_diffp_p010.tex <==
enrol&&18.233&&$-$0.630&&10.517&&1.026&&26.690&&2.232&\\
&&&&(3.544&)&&&(3.089&)&&&(5.562&)\\


==> results/rd_peer_n_grad_diffp_p06.tex <==
enrol&&15.102&&$-$1.238&&7.034&&0.566&&17.770&&$-$1.496&\\
&&&&(3.111&)&&&(1.978&)&&&(3.772&)\\


==> results/rd_peer_n_grad_diffp_p110.tex <==
enrol&&15.664&&$-$2.046&&8.769&&$-$0.656&&14.527&&0.152&\\
&&&&(3.308&)&&&(2.998&)&&&(4.649&)\\


==> results/rd_peer_n_grad_diffp_p16.tex <==
enrol&&14.076&&$-$2.727&&6.399&&0.529&&12.295&&$-$2.366&\\
&&&&(3.049&)&&&(2.040&)&&&(2.536&)\\


==> results/rd_peer_n_grad_diffp_p210.tex <==
enrol&&12.887&&$-$3.441&&6.853&&0.856&&10.978&&$-$0.633&\\
&&&&(2.831&)&&&(2.630&)&&&(3.781&)\\


==> results/rd_peer_n_grad_diffp_p26.tex <==
enrol&&11.762&&$-$2.869&&5.494&&1.543&&10.111&&$-$2.938&\\
&&&&(2.294&)&&&(1.761&)&&&(2.748&)\\


==> results/rd_peer_n_grad_diffp_p310.tex <==
enrol&&10.736&&$-$3.109&&7.369&&$-$1.747&&19.650&&$-$0.838&\\
&&&&(2.236&)&&&(2.547&)&&&(4.623&)\\


==> results/rd_peer_n_grad_diffp_p36.tex <==
enrol&&10.167&&$-$3.826&\sym{*}&5.993&&1.775&&14.813&&$-$1.399&\\
&&&&(2.081&)&&&(1.732&)&&&(3.880&)\\


==> results/rd_peer_n_grad_m110.tex <==
Co-employment w/ alum cohort c = -1&&4.661&&0.601&&3.344&&0.817&&5.123&&0.007&\\
&&&&(0.799&)&&&(0.759&)&&&(1.022&)\\


==> results/rd_peer_n_grad_m16.tex <==
Co-employment w/ alum cohort c = -1&&5.501&&0.795&&4.011&&0.127&&8.268&&$-$0.982&\\
&&&&(0.979&)&&&(0.951&)&&&(1.524&)\\


==> results/rd_peer_n_grad_m210.tex <==
Co-employment w/ alum cohort c = -2&&4.897&&$-$0.776&&3.992&&$-$0.596&&6.195&&0.561&\\
&&&&(0.853&)&&&(1.042&)&&&(1.470&)\\


==> results/rd_peer_n_grad_m26.tex <==
Co-employment w/ alum cohort c = -2&&5.188&&0.264&&3.563&&0.274&&7.583&&$-$0.330&\\
&&&&(1.042&)&&&(0.972&)&&&(1.717&)\\


==> results/rd_peer_n_grad_m310.tex <==
Co-employment w/ alum cohort c = -3&&5.535&&1.067&&4.051&&0.337&&8.596&&1.344&\\
&&&&(0.935&)&&&(1.154&)&&&(1.963&)\\


==> results/rd_peer_n_grad_m36.tex <==
Co-employment w/ alum cohort c = -3&&5.959&&$-$0.385&&2.459&&0.708&&5.374&&$-$0.490&\\
&&&&(1.116&)&&&(0.779&)&&&(1.381&)\\


==> results/rd_peer_n_grad_p010.tex <==
Co-employment w/ alum cohort c = +0&&5.840&&1.337&&3.285&&$-$0.130&&4.534&&0.489&\\
&&&&(0.921&)&&&(0.670&)&&&(1.101&)\\


==> results/rd_peer_n_grad_p06.tex <==
Co-employment w/ alum cohort c = +0&&6.205&&0.556&&4.176&&0.625&&6.652&&$-$0.716&\\
&&&&(1.099&)&&&(0.760&)&&&(1.372&)\\


==> results/rd_peer_n_grad_p110.tex <==
Co-employment w/ alum cohort c = +1&&4.927&&0.535&&2.615&&$-$0.547&&2.253&&0.025&\\
&&&&(0.805&)&&&(0.554&)&&&(0.752&)\\


==> results/rd_peer_n_grad_p16.tex <==
Co-employment w/ alum cohort c = +1&&5.144&&0.557&&3.114&&$-$0.462&&4.136&&$-$0.719&\\
&&&&(0.958&)&&&(0.623&)&&&(0.925&)\\


==> results/rd_peer_n_grad_p210.tex <==
Co-employment w/ alum cohort c = +2&&4.087&&$-$0.289&&2.020&&$-$0.134&&1.491&&0.383&\\
&&&&(0.595&)&&&(0.478&)&&&(0.634&)\\


==> results/rd_peer_n_grad_p26.tex <==
Co-employment w/ alum cohort c = +2&&4.218&&0.188&&2.112&&0.437&&2.389&&0.400&\\
&&&&(0.769&)&&&(0.560&)&&&(0.672&)\\


==> results/rd_peer_n_grad_p310.tex <==
Co-employment w/ alum cohort c = +3&&3.217&&$-$0.563&&2.099&&0.401&&2.289&&$-$0.072&\\
&&&&(0.574&)&&&(0.460&)&&&(0.571&)\\


==> results/rd_peer_n_grad_p36.tex <==
Co-employment w/ alum cohort c = +3&&3.292&&0.605&&2.516&&0.757&&2.917&&$-$0.058&\\
&&&&(0.728&)&&&(0.508&)&&&(0.876&)\\


==> results/rd_peer_n_grad_sameg_diffp10.tex <==
Co-employment different program, same field&&78.770&&$-$20.768&&49.053&&10.263&&173.155&&$-$43.652&\\
&&&&(21.239&)&&&(22.588&)&&&(39.384&)\\


==> results/rd_peer_n_grad_sameg_diffp6.tex <==
Co-employment different program, same field&&47.924&&$-$4.741&&40.737&&17.833&&117.705&&$-$31.098&\\
&&&&(13.554&)&&&(17.085&)&&&(27.061&)\\


==> results/rd_peer_n_grad_samep10.tex <==
Co-employment same program&&10.237&&0.568&&8.048&&3.638&\sym{**}&11.206&&0.530&\\
&&&&(1.653&)&&&(1.642&)&&&(2.051&)\\


==> results/rd_peer_n_grad_samep6.tex <==
Co-employment same program&&7.588&&0.382&&6.929&&2.765&\sym{**}&9.790&&2.230&\\
&&&&(1.088&)&&&(1.339&)&&&(1.572&)\\


==> results/rd_peer_n_grad_samep_m110.tex <==
Same program, c = -1&&1.016&&0.139&&0.588&&0.412&\sym{***}&0.942&&0.033&\\
&&&&(0.186&)&&&(0.133&)&&&(0.178&)\\


==> results/rd_peer_n_grad_samep_m16.tex <==
Same program, c = -1&&0.834&&0.189&&0.527&&0.197&\sym{*}&0.621&&0.117&\\
&&&&(0.150&)&&&(0.108&)&&&(0.146&)\\


==> results/rd_peer_n_grad_samep_m210.tex <==
Same program, c = -2&&0.786&&0.169&&0.544&&0.383&\sym{***}&0.845&&0.017&\\
&&&&(0.177&)&&&(0.114&)&&&(0.206&)\\


==> results/rd_peer_n_grad_samep_m26.tex <==
Same program, c = -2&&0.545&&0.048&&0.341&&0.202&\sym{***}&0.492&&0.113&\\
&&&&(0.131&)&&&(0.075&)&&&(0.134&)\\


==> results/rd_peer_n_grad_samep_m310.tex <==
Same program, c = -3&&0.871&&0.140&&0.423&&0.181&\sym{*}&0.444&&0.187&\\
&&&&(0.195&)&&&(0.097&)&&&(0.140&)\\


==> results/rd_peer_n_grad_samep_m36.tex <==
Same program, c = -3&&0.499&&$-$0.061&&0.189&&0.072&\sym{*}&0.202&&0.119&\sym{**}\\
&&&&(0.130&)&&&(0.042&)&&&(0.056&)\\


==> results/rd_peer_n_grad_samep_p010.tex <==
Same program, c = +0&&1.286&&0.103&&0.673&&0.356&\sym{***}&1.058&&0.149&\\
&&&&(0.231&)&&&(0.124&)&&&(0.184&)\\


==> results/rd_peer_n_grad_samep_p06.tex <==
Same program, c = +0&&1.162&&0.057&&0.750&&0.575&\sym{***}&0.929&&0.297&\\
&&&&(0.180&)&&&(0.145&)&&&(0.196&)\\


==> results/rd_peer_n_grad_samep_p110.tex <==
Same program, c = +1&&1.150&&$-$0.001&&0.502&&0.203&\sym{*}&0.412&&0.151&\\
&&&&(0.199&)&&&(0.122&)&&&(0.162&)\\


==> results/rd_peer_n_grad_samep_p16.tex <==
Same program, c = +1&&1.092&&0.114&&0.557&&0.098&&0.508&&0.137&\\
&&&&(0.160&)&&&(0.137&)&&&(0.125&)\\


==> results/rd_peer_n_grad_samep_p210.tex <==
Same program, c = +2&&0.910&&0.012&&0.389&&0.154&&0.292&&0.252&\sym{**}\\
&&&&(0.163&)&&&(0.104&)&&&(0.127&)\\


==> results/rd_peer_n_grad_samep_p26.tex <==
Same program, c = +2&&0.935&&0.056&&0.383&&0.271&\sym{**}&0.437&&0.234&\sym{**}\\
&&&&(0.151&)&&&(0.109&)&&&(0.110&)\\


==> results/rd_peer_n_grad_samep_p310.tex <==
Same program, c = +3&&0.697&&0.046&&0.448&&0.207&&0.823&&$-$0.072&\\
&&&&(0.141&)&&&(0.126&)&&&(0.169&)\\


==> results/rd_peer_n_grad_samep_p36.tex <==
Same program, c = +3&&0.718&&0.147&&0.446&&0.260&\sym{**}&0.712&&0.181&\\
&&&&(0.150&)&&&(0.109&)&&&(0.139&)\\


==> results/rd_peertrack_n10.tex <==
\(N\) (AA track)&&2,242&&25,644&&2,039&&31,511&&277&&3,087&\\


==> results/rd_peertrack_n6.tex <==
\(N\) (AA track)&&2,029&&27,588&&2,698&&36,712&&396&&6,347&\\


==> results/rd_prof.tex <==
Professional occupation&&0.616&&0.063&\sym{*}&0.606&&0.074&\sym{**}&0.443&&0.030&\\
&&&&(0.038&)&&&(0.035&)&&&(0.043&)\\


==> results/rd_prof10.tex <==
Professional occupation&&0.682&&0.022&&0.670&&0.032&&0.518&&$-$0.003&\\
&&&&(0.031&)&&&(0.035&)&&&(0.046&)\\


==> results/rd_prof6.tex <==
Professional occupation&&0.523&&0.079&\sym{*}&0.667&&$-$0.043&&0.633&&$-$0.009&\\
&&&&(0.044&)&&&(0.051&)&&&(0.099&)\\


==> results/rd_rio_muni.tex <==
Worked in Rio de Janeiro&&0.773&&$-$0.012&&0.755&&0.074&\sym{**}&0.794&&$-$0.015&\\
&&&&(0.026&)&&&(0.036&)&&&(0.031&)\\


==> results/rd_rio_muni10.tex <==
Worked in Rio de Janeiro&&0.748&&$-$0.014&&0.705&&0.019&&0.726&&0.005&\\
&&&&(0.031&)&&&(0.037&)&&&(0.040&)\\


==> results/rd_rio_muni6.tex <==
Worked in Rio de Janeiro&&0.704&&$-$0.016&&0.666&&0.068&&0.583&&0.265&\sym{**}\\
&&&&(0.044&)&&&(0.053&)&&&(0.118&)\\


==> results/rd_rio_st.tex <==
Worked in state of RJ&&0.898&&0.000&&0.890&&0.016&&0.937&&$-$0.003&\\
&&&&(0.022&)&&&(0.024&)&&&(0.019&)\\


==> results/rd_rio_st10.tex <==
Worked in state of RJ&&0.866&&0.006&&0.833&&0.028&&0.913&&$-$0.004&\\
&&&&(0.023&)&&&(0.026&)&&&(0.028&)\\


==> results/rd_rio_st6.tex <==
Worked in state of RJ&&0.868&&$-$0.032&&0.850&&$-$0.023&&0.783&&0.141&\sym{*}\\
&&&&(0.035&)&&&(0.043&)&&&(0.085&)\\


==> results/rd_ssci_earn_mean10.tex <==
Social sciences&&2,524.086&&$-$252.707&&2,120.115&&184.389&&1,062.426&&$-$45.814&\\
&&&&(190.772&)&&&(205.618&)&&&(151.932&)\\


==> results/rd_ssci_grad_by10.tex <==
Socialsciences&&0.001&&0.761&\sym{***}&0.002&&0.734&\sym{***}&0.000&&0.715&\sym{***}\\
&&&&(0.031&)&&&(0.022&)&&&(0.041&)\\


==> results/rd_ssci_lwage10.tex <==
Socialsciences&&3.732&&$-$0.099&&3.687&&0.071&&3.073&&$-$0.141&\\
&&&&(0.089&)&&&(0.083&)&&&(0.122&)\\


==> results/rd_top_ind.tex <==
Most common industry&&0.363&&0.051&&0.344&&0.075&\sym{**}&0.366&&0.066&\sym{*}\\
&&&&(0.036&)&&&(0.036&)&&&(0.040&)\\


==> results/rd_top_ind2.tex <==
Most common industry (2 digit)&&0.363&&0.051&&0.344&&0.075&\sym{**}&0.366&&0.066&\sym{*}\\
&&&&(0.036&)&&&(0.036&)&&&(0.040&)\\


==> results/rd_top_ind210.tex <==
Most common industry (2 digit)&&0.368&&0.001&&0.355&&0.047&&0.390&&0.026&\\
&&&&(0.032&)&&&(0.032&)&&&(0.040&)\\


==> results/rd_top_ind26.tex <==
Most common industry (2 digit)&&0.314&&0.044&&0.357&&0.046&&0.367&&$-$0.014&\\
&&&&(0.047&)&&&(0.051&)&&&(0.094&)\\


==> results/rd_top_ind5.tex <==
Worked in modal industry for UERJ alumni&&0.233&&0.048&&0.203&&0.052&\sym{**}&0.269&&0.057&\sym{*}\\
&&&&(0.032&)&&&(0.026&)&&&(0.032&)\\


==> results/rd_top_ind510.tex <==
Worked in modal industry for UERJ alumni&&0.264&&0.004&&0.205&&0.032&&0.292&&0.006&\\
&&&&(0.030&)&&&(0.029&)&&&(0.037&)\\


==> results/rd_top_ind56.tex <==
Worked in modal industry for UERJ alumni&&0.187&&0.057&&0.167&&0.039&&0.183&&0.018&\\
&&&&(0.044&)&&&(0.037&)&&&(0.070&)\\


==> results/rd_top_ind_firm_p000_uerj10.tex <==
Firm w/ any alum and in top 10 industry&&0.587&&0.081&\sym{**}&0.522&&0.018&&0.484&&0.073&\sym{*}\\
&&&&(0.037&)&&&(0.038&)&&&(0.043&)\\


==> results/rd_top_ind_firm_p000_uerj6.tex <==
Firm w/ any alum and in top 10 industry&&0.558&&0.103&\sym{***}&0.520&&0.082&\sym{**}&0.460&&0.118&\sym{***}\\
&&&&(0.033&)&&&(0.035&)&&&(0.038&)\\


==> results/rd_top_ind_nofirm_p000_uerj10.tex <==
Firm w/o any alum and in top 10 industry&&0.264&&$-$0.032&&0.315&&0.022&&0.401&&$-$0.039&\\
&&&&(0.033&)&&&(0.037&)&&&(0.043&)\\


==> results/rd_top_ind_nofirm_p000_uerj6.tex <==
Firm w/o any alum and in top 10 industry&&0.316&&$-$0.070&\sym{**}&0.331&&$-$0.043&&0.412&&$-$0.122&\sym{***}\\
&&&&(0.031&)&&&(0.033&)&&&(0.038&)\\


==> results/rd_top_ind_nopeer_any_grad_any10.tex <==
No alum from any cohort and in top 10 industry&&0.356&&$-$0.036&&0.387&&$-$0.021&&0.469&&$-$0.054&\\
&&&&(0.032&)&&&(0.036&)&&&(0.040&)\\


==> results/rd_top_ind_nopeer_any_grad_any6.tex <==
No alum from any cohort and in top 10 industry&&0.411&&$-$0.061&\sym{*}&0.418&&$-$0.049&&0.492&&$-$0.128&\sym{***}\\
&&&&(0.036&)&&&(0.036&)&&&(0.039&)\\


==> results/rd_top_ind_peer_any_grad_any10.tex <==
Alum from any cohort and in top 10 industry&&0.495&&0.069&\sym{**}&0.450&&0.055&&0.415&&0.086&\sym{**}\\
&&&&(0.033&)&&&(0.034&)&&&(0.039&)\\


==> results/rd_top_ind_peer_any_grad_any6.tex <==
Alum from any cohort and in top 10 industry&&0.464&&0.105&\sym{***}&0.434&&0.087&\sym{**}&0.379&&0.125&\sym{***}\\
&&&&(0.036&)&&&(0.035&)&&&(0.038&)\\


==> results/rd_wage10.tex <==
Hourly wage&&12.837&&0.271&&13.227&&0.404&&6.669&&2.230&\sym{*}\\
&&&&(1.024&)&&&(1.468&)&&&(1.261&)\\


==> results/rd_wage6.tex <==
Hourly wage&&8.535&&0.007&&10.100&&$-$0.413&&5.527&&1.354&\sym{**}\\
&&&&(0.486&)&&&(0.901&)&&&(0.680&)\\


==> results/rd_works_difind10.tex <==
enrol&&0.640&&0.107&\sym{***}&0.621&&0.077&\sym{**}&0.668&&$-$0.013&\\
&&&&(0.034&)&&&(0.037&)&&&(0.049&)\\


==> results/rd_works_difind6.tex <==
enrol&&0.669&&0.087&\sym{***}&0.655&&0.039&&0.624&&0.069&\sym{*}\\
&&&&(0.034&)&&&(0.037&)&&&(0.040&)\\


==> results/rd_works_topind10.tex <==
enrol&&0.851&&0.042&&0.837&&0.052&\sym{*}&0.884&&$-$0.007&\\
&&&&(0.028&)&&&(0.030&)&&&(0.040&)\\


==> results/rd_works_topind6.tex <==
enrol&&0.875&&0.041&\sym{*}&0.852&&0.037&\sym{*}&0.871&&0.015&\\
&&&&(0.025&)&&&(0.022&)&&&(0.026&)\\


==> results/rdaa_earn_dec10.tex <==
enrol&&4617.559&&692.615&\sym{*}&4616.471&&585.524&&4630.704&&1487.237&\sym{**}\\
&&&&(394.479&)&&&(436.372&)&&&(655.956&)\\


==> results/rdaa_earn_dec6.tex <==
Dec earnings, 6-9 yrs&&3787.545&&523.885&\sym{**}&3669.748&&555.110&&3997.505&&459.865&\\
&&&&(243.691&)&&&(355.422&)&&&(314.790&)\\


==> results/rdaa_earn_mean10.tex <==
enrol&&4437.622&&324.932&&4443.594&&254.368&&4362.690&&724.711&\\
&&&&(362.203&)&&&(400.025&)&&&(603.156&)\\


==> results/rdaa_earn_mean6.tex <==
Average monthly earnings, 6-9 yrs&&3493.691&&353.054&&3358.177&&492.500&&3729.942&&117.251&\\
&&&&(219.523&)&&&(307.461&)&&&(309.087&)\\


==> results/rdaa_est_mean_wage10.tex <==
enrol&&30.979&&3.229&&31.023&&4.279&&30.426&&$-$7.004&\\
&&&&(3.677&)&&&(4.002&)&&&(9.175&)\\


==> results/rdaa_est_mean_wage6.tex <==
Firm mean hourly wage, 6-9 yrs&&27.857&&6.985&\sym{**}&26.834&&3.811&&29.634&&10.653&\\
&&&&(3.366&)&&&(3.411&)&&&(6.493&)\\


==> results/rdaa_firm_aa10.tex <==
AA track only, 10-13 yrs&&0.317&&0.100&\sym{**}&0.306&&0.111&\sym{**}&0.453&&0.021&\\
&&&&(0.050&)&&&(0.055&)&&&(0.087&)\\


==> results/rdaa_firm_aa6.tex <==
AA track only, 6-9 yrs&&0.297&&0.087&\sym{**}&0.274&&0.122&\sym{**}&0.336&&0.049&\\
&&&&(0.036&)&&&(0.050&)&&&(0.051&)\\


==> results/rdaa_firm_both10.tex <==
Both tracks, 10-13 yrs&&0.275&&0.111&\sym{**}&0.265&&0.127&\sym{**}&0.391&&$-$0.002&\\
&&&&(0.048&)&&&(0.053&)&&&(0.085&)\\


==> results/rdaa_firm_both6.tex <==
Both tracks, 6-9 yrs&&0.265&&0.063&\sym{*}&0.245&&0.111&\sym{**}&0.301&&0.003&\\
&&&&(0.034&)&&&(0.048&)&&&(0.049&)\\


==> results/rdaa_firm_gen10.tex <==
General track only, 10-13 yrs&&0.121&&$-$0.011&&0.126&&$-$0.016&&0.063&&0.033&\\
&&&&(0.035&)&&&(0.039&)&&&(0.057&)\\


==> results/rdaa_firm_gen6.tex <==
General track only, 6-9 yrs&&0.097&&$-$0.016&&0.100&&$-$0.023&&0.092&&$-$0.009&\\
&&&&(0.025&)&&&(0.035&)&&&(0.035&)\\


==> results/rdaa_firm_p000_aa10.tex <==
firmp000aa+10-13 yrs&&0.317&&0.099&\sym{**}&0.306&&0.112&\sym{**}&0.453&&0.002&\\
&&&&(0.050&)&&&(0.056&)&&&(0.088&)\\


==> results/rdaa_firm_p000_aa6.tex <==
firmp000aa+6-9 yrs&&0.298&&0.083&\sym{**}&0.273&&0.127&\sym{**}&0.342&&0.032&\\
&&&&(0.036&)&&&(0.051&)&&&(0.052&)\\


==> results/rdaa_firm_p000_all10.tex <==
firmp000all+10-13 yrs&&0.459&&0.088&\sym{*}&0.454&&0.101&\sym{*}&0.516&&0.003&\\
&&&&(0.052&)&&&(0.058&)&&&(0.094&)\\


==> results/rdaa_firm_p000_all6.tex <==
firmp000all+6-9 yrs&&0.407&&0.067&\sym{*}&0.386&&0.110&\sym{**}&0.442&&0.019&\\
&&&&(0.038&)&&&(0.053&)&&&(0.054&)\\


==> results/rdaa_firm_p000_gen10.tex <==
firmp000gen+10-13 yrs&&0.422&&0.091&\sym{*}&0.418&&0.108&\sym{*}&0.469&&$-$0.025&\\
&&&&(0.052&)&&&(0.058&)&&&(0.094&)\\


==> results/rdaa_firm_p000_gen6.tex <==
firmp000gen+6-9 yrs&&0.383&&0.045&&0.362&&0.101&\sym{*}&0.418&&$-$0.025&\\
&&&&(0.038&)&&&(0.053&)&&&(0.054&)\\


==> results/rdaa_firm_p000_post10.tex <==
firmp000post+10-13 yrs&&0.107&&$-$0.015&&0.108&&$-$0.036&&0.094&&0.152&\sym{**}\\
&&&&(0.031&)&&&(0.034&)&&&(0.063&)\\


==> results/rdaa_firm_p000_post6.tex <==
firmp000post+6-9 yrs&&0.083&&0.028&&0.073&&$-$0.008&&0.100&&0.081&\sym{**}\\
&&&&(0.023&)&&&(0.030&)&&&(0.038&)\\


==> results/rdaa_firm_p000_pre10.tex <==
firmp000pre+10-13 yrs&&0.351&&0.103&\sym{**}&0.346&&0.137&\sym{**}&0.422&&$-$0.149&\\
&&&&(0.051&)&&&(0.057&)&&&(0.091&)\\


==> results/rdaa_firm_p000_pre6.tex <==
firmp000pre+6-9 yrs&&0.324&&0.039&&0.313&&0.118&\sym{**}&0.342&&$-$0.062&\\
&&&&(0.037&)&&&(0.052&)&&&(0.051&)\\


==> results/rdaa_firm_p001_aa10.tex <==
firmp001aa+10-13 yrs&&0.099&&0.042&&0.094&&0.043&&0.156&&0.034&\\
&&&&(0.033&)&&&(0.036&)&&&(0.070&)\\


==> results/rdaa_firm_p001_aa6.tex <==
firmp001aa+6-9 yrs&&0.106&&0.085&\sym{***}&0.078&&0.103&\sym{***}&0.155&&0.063&\\
&&&&(0.026&)&&&(0.034&)&&&(0.041&)\\


==> results/rdaa_firm_p001_all10.tex <==
firmp001all+10-13 yrs&&0.305&&0.086&\sym{*}&0.310&&0.085&&0.250&&0.102&\\
&&&&(0.047&)&&&(0.053&)&&&(0.084&)\\


==> results/rdaa_firm_p001_all6.tex <==
firmp001all+6-9 yrs&&0.265&&0.124&\sym{***}&0.260&&0.150&\sym{***}&0.275&&0.093&\sym{*}\\
&&&&(0.036&)&&&(0.049&)&&&(0.050&)\\


==> results/rdaa_firm_p001_gen10.tex <==
firmp001gen+10-13 yrs&&0.246&&0.046&&0.249&&0.049&&0.219&&0.031&\\
&&&&(0.044&)&&&(0.049&)&&&(0.083&)\\


==> results/rdaa_firm_p001_gen6.tex <==
firmp001gen+6-9 yrs&&0.220&&0.089&\sym{***}&0.216&&0.109&\sym{**}&0.227&&0.064&\\
&&&&(0.033&)&&&(0.046&)&&&(0.047&)\\


==> results/rdaa_firm_p001_post10.tex <==
firmp001post+10-13 yrs&&0.178&&0.041&&0.173&&0.037&&0.234&&0.080&\\
&&&&(0.039&)&&&(0.043&)&&&(0.080&)\\


==> results/rdaa_firm_p001_post6.tex <==
firmp001post+6-9 yrs&&0.163&&0.093&\sym{***}&0.130&&0.099&\sym{**}&0.220&&0.090&\sym{*}\\
&&&&(0.030&)&&&(0.040&)&&&(0.047&)\\


==> results/rdaa_firm_p001_pre10.tex <==
firmp001pre+10-13 yrs&&0.175&&0.050&&0.173&&0.067&&0.188&&$-$0.081&\\
&&&&(0.040&)&&&(0.045&)&&&(0.076&)\\


==> results/rdaa_firm_p001_pre6.tex <==
firmp001pre+6-9 yrs&&0.166&&0.077&\sym{**}&0.169&&0.112&\sym{***}&0.161&&0.033&\\
&&&&(0.030&)&&&(0.043&)&&&(0.042&)\\


==> results/rdaa_firm_p005_aa10.tex <==
5 AA track alumni (2004--2011 cohorts), 10-13 yrs&&0.038&&0.009&&0.037&&0.012&&0.047&&$-$0.007&\\
&&&&(0.022&)&&&(0.024&)&&&(0.042&)\\


==> results/rdaa_firm_p005_aa6.tex <==
5 AA track alumni (2004--2011 cohorts), 6-9 yrs&&0.042&&0.042&\sym{**}&0.034&&0.054&\sym{**}&0.054&&0.027&\\
&&&&(0.018&)&&&(0.024&)&&&(0.028&)\\


==> results/rdaa_firm_p005_all10.tex <==
, 10-13 yrs&&0.117&&0.010&&0.117&&0.002&&0.109&&0.074&\\
&&&&(0.038&)&&&(0.042&)&&&(0.076&)\\


==> results/rdaa_firm_p005_all6.tex <==
, 6-9 yrs&&0.118&&0.047&&0.109&&0.051&&0.133&&0.039&\\
&&&&(0.030&)&&&(0.041&)&&&(0.043&)\\


==> results/rdaa_firm_p005_gen10.tex <==
, 10-13 yrs&&0.083&&0.001&&0.082&&0.007&&0.094&&$-$0.036&\\
&&&&(0.034&)&&&(0.037&)&&&(0.064&)\\


==> results/rdaa_firm_p005_gen6.tex <==
, 6-9 yrs&&0.086&&0.024&&0.082&&0.027&&0.092&&0.019&\\
&&&&(0.026&)&&&(0.037&)&&&(0.037&)\\


==> results/rdaa_firm_p010_aa10.tex <==
10 AA track alumni (2004--2011 cohorts), 10-13 yrs&&0.026&&$-$0.002&&0.026&&$-$0.006&&0.031&&0.021&\\
&&&&(0.014&)&&&(0.015&)&&&(0.029&)\\


==> results/rdaa_firm_p010_aa6.tex <==
10 AA track alumni (2004--2011 cohorts), 6-9 yrs&&0.028&&0.027&\sym{**}&0.023&&0.034&\sym{**}&0.037&&0.015&\\
&&&&(0.012&)&&&(0.016&)&&&(0.020&)\\


==> results/rdaa_firm_p010_all10.tex <==
, 10-13 yrs&&0.091&&$-$0.054&&0.091&&$-$0.051&&0.094&&$-$0.079&\\
&&&&(0.035&)&&&(0.039&)&&&(0.067&)\\


==> results/rdaa_firm_p010_all6.tex <==
, 6-9 yrs&&0.086&&$-$0.019&&0.082&&$-$0.014&&0.092&&$-$0.023&\\
&&&&(0.027&)&&&(0.037&)&&&(0.038&)\\


==> results/rdaa_firm_p010_gen10.tex <==
, 10-13 yrs&&0.065&&$-$0.022&&0.063&&$-$0.019&&0.094&&$-$0.035&\\
&&&&(0.030&)&&&(0.034&)&&&(0.056&)\\


==> results/rdaa_firm_p010_gen6.tex <==
, 6-9 yrs&&0.066&&0.003&&0.063&&0.006&&0.072&&$-$0.000&\\
&&&&(0.023&)&&&(0.032&)&&&(0.032&)\\


==> results/rdaa_firm_p025_aa10.tex <==
25 AA track alumni (2004--2011 cohorts), 10-13 yrs&&0.004&&0.001&&0.003&&0.001&&0.016&&0.003&\\
&&&&(0.007&)&&&(0.008&)&&&(0.018&)\\


==> results/rdaa_firm_p025_aa6.tex <==
25 AA track alumni (2004--2011 cohorts), 6-9 yrs&&0.003&&0.014&\sym{*}&0.001&&0.019&\sym{*}&0.007&&0.007&\\
&&&&(0.007&)&&&(0.010&)&&&(0.011&)\\


==> results/rdaa_firm_p025_all10.tex <==
, 10-13 yrs&&0.018&&0.021&&0.015&&0.019&&0.047&&0.036&\\
&&&&(0.017&)&&&(0.019&)&&&(0.035&)\\


==> results/rdaa_firm_p025_all6.tex <==
, 6-9 yrs&&0.026&&0.020&&0.011&&0.033&\sym{*}&0.052&&0.001&\\
&&&&(0.014&)&&&(0.018&)&&&(0.022&)\\


==> results/rdaa_firm_p025_gen10.tex <==
, 10-13 yrs&&0.014&&0.005&&0.011&&0.007&&0.047&&$-$0.008&\\
&&&&(0.014&)&&&(0.015&)&&&(0.027&)\\


==> results/rdaa_firm_p025_gen6.tex <==
, 6-9 yrs&&0.024&&0.009&&0.009&&0.026&\sym{*}&0.050&&$-$0.015&\\
&&&&(0.011&)&&&(0.015&)&&&(0.018&)\\


==> results/rdaa_firm_p050_aa10.tex <==
50 AA track alumni (2004--2011 cohorts), 10-13 yrs&&0.000&&$-$0.000&&0.000&&$-$0.000&&0.000&&0.001&\\
&&&&(0.004&)&&&(0.004&)&&&(0.012&)\\


==> results/rdaa_firm_p050_aa6.tex <==
50 AA track alumni (2004--2011 cohorts), 6-9 yrs&&0.000&&0.002&&0.000&&$-$0.001&&0.000&&0.006&\\
&&&&(0.005&)&&&(0.007&)&&&(0.005&)\\


==> results/rdaa_firm_p050_all10.tex <==
, 10-13 yrs&&0.008&&0.005&&0.005&&0.002&&0.047&&0.021&\\
&&&&(0.011&)&&&(0.013&)&&&(0.025&)\\


==> results/rdaa_firm_p050_all6.tex <==
, 6-9 yrs&&0.016&&0.016&\sym{*}&0.001&&0.020&&0.041&&0.012&\\
&&&&(0.010&)&&&(0.013&)&&&(0.016&)\\


==> results/rdaa_firm_p050_gen10.tex <==
, 10-13 yrs&&0.006&&$-$0.005&&0.005&&$-$0.005&&0.016&&$-$0.001&\\
&&&&(0.009&)&&&(0.010&)&&&(0.015&)\\


==> results/rdaa_firm_p050_gen6.tex <==
, 6-9 yrs&&0.006&&0.014&\sym{*}&0.000&&0.022&\sym{**}&0.017&&0.005&\\
&&&&(0.008&)&&&(0.011&)&&&(0.011&)\\


==> results/rdaa_in_rais10.tex <==
enrol&&0.663&&0.020&&0.672&&0.023&&0.561&&0.001&\\
&&&&(0.038&)&&&(0.042&)&&&(0.073&)\\


==> results/rdaa_in_rais6.tex <==
Formal employment, 6-9 yrs&&0.603&&$-$0.007&&0.658&&$-$0.015&&0.526&&0.001&\\
&&&&(0.028&)&&&(0.039&)&&&(0.040&)\\


==> results/rdaa_learn_dec10.tex <==
enrol&&8.200&&0.059&&8.192&&0.050&&8.295&&0.096&\\
&&&&(0.070&)&&&(0.077&)&&&(0.127&)\\


==> results/rdaa_learn_dec6.tex <==
Log Dec earnings, 6-9 yrs&&7.997&&0.089&\sym{*}&7.949&&0.117&&8.082&&0.043&\\
&&&&(0.052&)&&&(0.072&)&&&(0.073&)\\


==> results/rdaa_learn_mean10.tex <==
Log average monthly earnings, 10-13 yrs&&8.158&&0.052&&8.151&&0.049&&8.243&&0.044&\\
&&&&(0.066&)&&&(0.073&)&&&(0.115&)\\


==> results/rdaa_learn_mean6.tex <==
learnmean+6-9 yrs&&8.125&&$-$0.008&&8.209&&$-$0.089&\sym{*}&7.701&&0.105&\sym{**}\\
&&&&(0.052&)&&&(0.047&)&&&(0.042&)\\


==> results/rdaa_lest_mean_wage10.tex <==
Log firm mean hourly wage, 10-13 yrs&&3.211&&0.070&&3.210&&0.092&&3.221&&$-$0.106&\\
&&&&(0.078&)&&&(0.086&)&&&(0.133&)\\


==> results/rdaa_lest_mean_wage6.tex <==
lestmeanwage+6-9 yrs&&3.167&&0.070&&3.377&&$-$0.106&\sym{*}&2.935&&0.033&\\
&&&&(0.057&)&&&(0.056&)&&&(0.060&)\\


==> results/rdaa_lwage10.tex <==
Log hourly wage, 10-13 yrs&&3.050&&0.061&&3.047&&0.051&&3.088&&0.129&\\
&&&&(0.067&)&&&(0.074&)&&&(0.111&)\\


==> results/rdaa_lwage6.tex <==
lwage+6-9 yrs&&3.055&&0.017&&3.185&&$-$0.113&\sym{**}&2.626&&0.071&\\
&&&&(0.059&)&&&(0.051&)&&&(0.054&)\\


==> results/rdaa_n_panel10.tex <==
\(N\) (applicant/years, 10$-$13 yrs)&&1,280&&15,516&&1,166&&13,683&&114&&1,833&\\


==> results/rdaa_n_panel6.tex <==
\(N\) (applicant/years, 6$-$9 yrs)&&2,076&&26,223&&1,204&&14,340&&872&&11,883&\\


==> results/rdaa_n_rais10.tex <==
\(N\) (wage observations, 10$-$13 yrs)&&838&&11,161&&777&&10,003&&61&&1,158&\\


==> results/rdaa_n_rais6.tex <==
\(N\) (wage observations, 6$-$9 yrs)&&2,023&&21,640&&2,690&&34,576&&396&&4,739&\\


==> results/rdaa_peer_any_grad_aa10.tex <==
peeranygradaa+10 yrs&&0.136&&$-$0.005&&0.246&&0.043&&0.231&&0.076&\sym{*}\\
&&&&(0.020&)&&&(0.031&)&&&(0.043&)\\


==> results/rdaa_peer_any_grad_aa6.tex <==
peeranygradaa+6 yrs&&0.095&&0.014&&0.235&&0.070&\sym{**}&0.222&&0.053&\\
&&&&(0.019&)&&&(0.028&)&&&(0.035&)\\


==> results/rdaa_peer_any_grad_any10.tex <==
peeranygradany+10 yrs&&0.437&&0.034&&0.424&&0.038&&0.343&&0.125&\sym{***}\\
&&&&(0.039&)&&&(0.034&)&&&(0.046&)\\


==> results/rdaa_peer_any_grad_any6.tex <==
peeranygradany+6 yrs&&0.371&&0.129&\sym{***}&0.394&&0.097&\sym{***}&0.316&&0.079&\sym{**}\\
&&&&(0.033&)&&&(0.034&)&&&(0.037&)\\


==> results/rdaa_peer_any_grad_both10.tex <==
peeranygradboth+10 yrs&&0.427&&0.044&&0.392&&0.044&&0.310&&0.099&\sym{**}\\
&&&&(0.039&)&&&(0.033&)&&&(0.046&)\\


==> results/rdaa_peer_any_grad_both6.tex <==
peeranygradboth+6 yrs&&0.364&&0.126&\sym{***}&0.359&&0.102&\sym{***}&0.288&&0.021&\\
&&&&(0.033&)&&&(0.034&)&&&(0.042&)\\


==> results/rdaa_peer_any_grad_diff10.tex <==
peeranygraddiff+10-13 yrs&&0.367&&0.103&\sym{**}&0.357&&0.121&\sym{**}&0.484&&$-$0.037&\\
&&&&(0.050&)&&&(0.056&)&&&(0.090&)\\


==> results/rdaa_peer_any_grad_diff6.tex <==
peeranygraddiff+6-9 yrs&&0.328&&0.046&&0.321&&0.073&&0.340&&0.017&\\
&&&&(0.036&)&&&(0.050&)&&&(0.050&)\\


==> results/rdaa_peer_any_grad_gen10.tex <==
peeranygradgen+10 yrs&&0.151&&$-$0.001&&0.275&&0.052&&0.220&&0.055&\\
&&&&(0.022&)&&&(0.032&)&&&(0.039&)\\


==> results/rdaa_peer_any_grad_gen6.tex <==
peeranygradgen+6 yrs&&0.102&&0.020&&0.252&&0.099&\sym{***}&0.210&&0.007&\\
&&&&(0.022&)&&&(0.031&)&&&(0.039&)\\


==> results/rdaa_peer_any_grad_post10.tex <==
peeranygradpost+10-13 yrs&&0.348&&0.074&&0.339&&0.085&&0.453&&0.006&\\
&&&&(0.049&)&&&(0.055&)&&&(0.091&)\\


==> results/rdaa_peer_any_grad_post6.tex <==
peeranygradpost+6-9 yrs&&0.298&&0.052&&0.288&&0.065&&0.316&&0.042&\\
&&&&(0.035&)&&&(0.049&)&&&(0.050&)\\


==> results/rdaa_peer_any_grad_pre10.tex <==
peeranygradpre+10 yrs&&0.410&&0.057&&0.319&&0.058&\sym{*}&0.278&&0.040&\\
&&&&(0.038&)&&&(0.033&)&&&(0.048&)\\


==> results/rdaa_peer_any_grad_pre6.tex <==
peeranygradpre+6 yrs&&0.354&&0.109&\sym{***}&0.288&&0.032&&0.235&&0.029&\\
&&&&(0.032&)&&&(0.032&)&&&(0.033&)\\


==> results/rdaa_peer_any_grad_same10.tex <==
peeranygradsame+10-13 yrs&&0.208&&0.067&&0.198&&0.084&\sym{*}&0.328&&$-$0.047&\\
&&&&(0.043&)&&&(0.048&)&&&(0.075&)\\


==> results/rdaa_peer_any_grad_same6.tex <==
peeranygradsame+6-9 yrs&&0.175&&0.043&&0.163&&0.077&\sym{*}&0.196&&$-$0.004&\\
&&&&(0.029&)&&&(0.040&)&&&(0.040&)\\


==> results/rdaa_uerj_firm10.tex <==
uerjfirm+10 yrs&&0.283&&0.081&\sym{**}&0.369&&0.058&\sym{*}&0.318&&0.094&\sym{**}\\
&&&&(0.032&)&&&(0.034&)&&&(0.043&)\\


==> results/rdaa_uerj_firm6.tex <==
uerjfirm+6 yrs&&0.172&&0.084&\sym{***}&0.332&&0.082&\sym{***}&0.283&&0.052&\\
&&&&(0.025&)&&&(0.032&)&&&(0.034&)\\


==> results/rddiff_college_degree.tex <==
Any college degree, 6-9 years later&&0.035&&0.009&&0.057&&$-$0.010&&0.003&&0.059&\\
&&(0.025&)&(0.025&)&(0.044&)&(0.029&)&(0.029&)&(0.040&)\\


==> results/rddiff_est_shr_coll.tex <==
Firm share of employees w/ college degree&&0.027&&$-$0.003&&0.002&&0.011&&0.029&&0.021&\\
&&(0.018&)&(0.017&)&(0.019&)&(0.019&)&(0.028&)&(0.024&)\\


==> results/rddiff_est_shr_white.tex <==
Prop. of co-workers who are white&&0.000&&0.025&&0.025&&0.023&&0.017&&$-$0.007&\\
&&(0.017&)&(0.021&)&(0.021&)&(0.022&)&(0.029&)&(0.028&)\\


==> results/rddiff_firm_p000_both.tex <==
Both pre- and post-AA alumni&&0.032&&$-$0.041&&$-$0.074&\sym{**}&0.086&\sym{**}&0.073&\sym{*}&$-$0.013&\\
&&(0.030&)&(0.034&)&(0.031&)&(0.034&)&(0.042&)&(0.035&)\\


==> results/rddiff_firm_p000_other.tex <==
Firm w/ only UERJ decliners&&0.008&&0.010&&0.002&&0.030&&$-$0.002&&$-$0.032&\\
&&(0.022&)&(0.023&)&(0.023&)&(0.021&)&(0.024&)&(0.026&)\\


==> results/rddiff_firm_p000_post.tex <==
Post-AA alumni only&&0.095&\sym{***}&0.108&\sym{***}&0.014&&0.079&\sym{*}&0.043&&$-$0.036&\\
&&(0.030&)&(0.033&)&(0.033&)&(0.041&)&(0.050&)&(0.047&)\\


==> results/rddiff_firm_p000_pre.tex <==
Pre-AA alumni only&&$-$0.012&&$-$0.025&&$-$0.013&&$-$0.011&&$-$0.017&&$-$0.006&\\
&&(0.015&)&(0.015&)&(0.015&)&(0.018&)&(0.021&)&(0.019&)\\


==> results/rddiff_firm_p000_uerj.tex <==
Firm w/ any alum&&0.052&&0.025&&0.080&\sym{*}&$-$0.063&\sym{*}&$-$0.046&&$-$0.057&\\
&&(0.036&)&(0.038&)&(0.044&)&(0.034&)&(0.036&)&(0.042&)\\


==> results/rddiff_firm_p000_uerj_after.tex <==
Firm w/ alum hired after applicant&&0.047&&0.068&\sym{*}&0.067&&$-$0.036&&$-$0.008&&$-$0.047&\\
&&(0.033&)&(0.036&)&(0.042&)&(0.031&)&(0.033&)&(0.038&)\\


==> results/rddiff_firm_p000_uerj_before.tex <==
Firm w/ alum hired before applicant&&0.050&&0.001&&0.052&&0.008&&$-$0.063&\sym{*}&$-$0.060&\\
&&(0.037&)&(0.036&)&(0.047&)&(0.035&)&(0.036&)&(0.043&)\\


==> results/rddiff_firm_p001_uerj.tex <==
Firm w/ 1 alum per 1000 employees&&0.096&\sym{***}&0.028&&0.107&\sym{***}&$-$0.033&&$-$0.024&&$-$0.057&\\
&&(0.033&)&(0.037&)&(0.039&)&(0.032&)&(0.036&)&(0.041&)\\


==> results/rddiff_firm_p005_uerj.tex <==
Firm w/ 5 alumni per 1000 employees&&0.105&\sym{***}&0.076&\sym{**}&0.037&&0.006&&$-$0.043&&$-$0.068&\sym{*}\\
&&(0.029&)&(0.034&)&(0.038&)&(0.027&)&(0.036&)&(0.036&)\\


==> results/rddiff_firm_p010_uerj.tex <==
Firm w/ 10 alumni per 1000 employees&&0.066&\sym{***}&0.059&\sym{*}&$-$0.008&&$-$0.034&&$-$0.040&&$-$0.073&\sym{**}\\
&&(0.024&)&(0.032&)&(0.031&)&(0.024&)&(0.032&)&(0.031&)\\


==> results/rddiff_firm_p01_alum.tex <==
Employed at firm with 10+ alumni / 1000 workers&&0.065&\sym{***}&0.056&\sym{*}&0.000&&$-$0.027&&$-$0.046&&$-$0.062&\sym{**}\\
&&(0.024&)&(0.032&)&(0.030&)&(0.024&)&(0.032&)&(0.031&)\\


==> results/rddiff_firm_p025_uerj.tex <==
Firm w/ 25 alumni per 1000 employees&&0.027&&0.031&&0.013&&$-$0.038&\sym{*}&$-$0.055&\sym{**}&$-$0.037&\sym{*}\\
&&(0.020&)&(0.023&)&(0.019&)&(0.020&)&(0.024&)&(0.019&)\\


==> results/rddiff_firm_p050_uerj.tex <==
Firm w/ 50 alumni per 1000 employees&&0.028&\sym{**}&0.025&\sym{**}&0.005&&$-$0.007&&$-$0.030&\sym{**}&$-$0.023&\\
&&(0.011&)&(0.013&)&(0.016&)&(0.013&)&(0.014&)&(0.016&)\\


==> results/rddiff_firm_rel_apply_alum.tex <==
\# UERJ alumni / 1000 workers at firm (demeaned)&&3.179&\sym{***}&4.552&&$-$0.821&&$-$0.326&&$-$2.727&&$-$6.007&\sym{*}\\
&&(1.159&)&(2.819&)&(1.601&)&(1.434&)&(2.782&)&(3.105&)\\


==> results/rddiff_firmwage_n.tex <==
\(N\) (firm mean wage)&&24,701&&21,071&&3,133&&55,046&&52,158&&7,439&\\


==> results/rddiff_gov_firm.tex <==
Publicly-owned firm&&0.002&&$-$0.020&&0.165&&0.162&&$-$0.455&&$-$0.470&\\
&&(0.087&)&(0.098&)&(0.133&)&(0.138&)&(0.382&)&(0.351&)\\


==> results/rddiff_grad_by.tex <==
Graduated from UERJ program&&0.718&\sym{***}&0.693&\sym{***}&0.661&\sym{***}&0.007&&0.016&\sym{*}&0.021&\\
&&(0.017&)&(0.014&)&(0.021&)&(0.005&)&(0.009&)&(0.014&)\\


==> results/rddiff_im_apply_pct_alum.tex <==
\# UERJ alumni / 1000 workers in labor market&&0.433&&0.316&&2.382&\sym{***}&$-$1.213&\sym{*}&$-$0.402&&$-$2.257&\sym{*}\\
&&(0.693&)&(0.940&)&(0.894&)&(0.712&)&(0.877&)&(1.289&)\\


==> results/rddiff_ind_wage1.tex <==
Industry wage 1&&$-$0.008&&0.004&&$-$0.010&&0.007&&$-$0.013&&$-$0.010&\\
&&(0.016&)&(0.015&)&(0.017&)&(0.019&)&(0.026&)&(0.024&)\\


==> results/rddiff_ind_wage2.tex <==
Industry wage 2&&$-$0.002&&0.012&&$-$0.030&&0.020&&0.020&&$-$0.007&\\
&&(0.029&)&(0.026&)&(0.032&)&(0.027&)&(0.036&)&(0.029&)\\


==> results/rddiff_ind_wage3.tex <==
Industry wage 3&&0.027&&0.010&&0.003&&0.051&&0.023&&0.000&\\
&&(0.030&)&(0.026&)&(0.038&)&(0.032&)&(0.042&)&(0.035&)\\


==> results/rddiff_ind_wage4.tex <==
Industry mean wage (log)&&0.035&&0.027&&0.018&&0.025&&0.051&&$-$0.026&\\
&&(0.035&)&(0.040&)&(0.044&)&(0.030&)&(0.035&)&(0.037&)\\


==> results/rddiff_ind_wage5.tex <==
Industry wage 5&&0.035&&0.025&&0.027&&0.049&&0.018&&$-$0.026&\\
&&(0.035&)&(0.030&)&(0.040&)&(0.035&)&(0.044&)&(0.037&)\\


==> results/rddiff_lest_mean_wage.tex <==
Firm mean wage (log)&&0.093&\sym{*}&$-$0.053&&0.049&&0.076&&0.042&&$-$0.057&\\
&&(0.053&)&(0.062&)&(0.071&)&(0.047&)&(0.057&)&(0.064&)\\


==> results/rddiff_lest_size.tex <==
Firm number of employees (log)&&$-$0.253&&$-$0.186&&0.190&&0.020&&0.286&&0.270&\\
&&(0.183&)&(0.157&)&(0.194&)&(0.172&)&(0.226&)&(0.210&)\\


==> results/rddiff_muni_wage.tex <==
Municipality mean wage (log)&&$-$0.025&&$-$0.027&&0.017&&$-$0.034&\sym{*}&$-$0.014&&0.022&\\
&&(0.021&)&(0.020&)&(0.023&)&(0.019&)&(0.018&)&(0.023&)\\


==> results/rddiff_n.tex <==
\(N\)&&27,448&&30,816&&4,718&&51,012&&63,739&&9,727&\\


==> results/rddiff_n_in_rais.tex <==
\(N\) (formal employment)&&39,134&&41,138&&4,320&&76,928&&96,168&&12,467&\\


==> results/rddiff_occ_wage1.tex <==
Occupation wage 1&&$-$0.011&&$-$0.050&\sym{*}&0.008&&0.009&&$-$0.066&&$-$0.071&\sym{*}\\
&&(0.028&)&(0.027&)&(0.027&)&(0.028&)&(0.044&)&(0.038&)\\


==> results/rddiff_occ_wage2.tex <==
Occupation wage 2&&0.029&&$-$0.034&&0.001&&0.004&&$-$0.020&&$-$0.044&\\
&&(0.029&)&(0.029&)&(0.030&)&(0.032&)&(0.040&)&(0.041&)\\


==> results/rddiff_occ_wage3.tex <==
Occupation wage 3&&0.009&&$-$0.019&&0.001&&0.043&&$-$0.061&&$-$0.098&\sym{**}\\
&&(0.033&)&(0.031&)&(0.040&)&(0.038&)&(0.053&)&(0.047&)\\


==> results/rddiff_occ_wage4.tex <==
Occupation mean wage (log)&&$-$0.009&&0.025&&$-$0.071&&$-$0.037&&0.087&\sym{**}&$-$0.124&\sym{***}\\
&&(0.033&)&(0.041&)&(0.053&)&(0.031&)&(0.040&)&(0.046&)\\


==> results/rddiff_occ_wage5.tex <==
Occupation wage 5&&$-$0.016&&$-$0.039&&$-$0.001&&0.062&&$-$0.078&&$-$0.119&\sym{**}\\
&&(0.038&)&(0.035&)&(0.044&)&(0.041&)&(0.054&)&(0.047&)\\


==> results/rddiff_occ_wage6.tex <==
Occupation wage 6&&$-$0.004&&$-$0.023&&0.000&&0.054&&$-$0.065&&$-$0.115&\sym{**}\\
&&(0.037&)&(0.035&)&(0.044&)&(0.041&)&(0.055&)&(0.048&)\\


==> results/rddiff_peer_any_decline.tex <==
Co-employment w/ only UERJ decliners&&$-$0.044&&0.010&&0.054&&0.030&&0.043&&0.013&\\
&&(0.028&)&(0.030&)&(0.034&)&(0.028&)&(0.032&)&(0.036&)\\


==> results/rddiff_peer_any_grad_after.tex <==
Alum hired after applicant&&0.029&&0.062&\sym{*}&0.030&&$-$0.007&&0.018&&$-$0.016&\\
&&(0.034&)&(0.036&)&(0.045&)&(0.036&)&(0.036&)&(0.041&)\\


==> results/rddiff_peer_any_grad_any.tex <==
Alum from any cohort&&0.052&&0.048&&0.092&\sym{**}&$-$0.052&&$-$0.044&&$-$0.043&\\
&&(0.033&)&(0.035&)&(0.039&)&(0.035&)&(0.038&)&(0.040&)\\


==> results/rddiff_peer_any_grad_before.tex <==
Alum hired before applicant&&0.036&&$-$0.002&&0.067&&$-$0.006&&$-$0.071&\sym{**}&$-$0.036&\\
&&(0.034&)&(0.036&)&(0.042&)&(0.033&)&(0.035&)&(0.037&)\\


==> results/rddiff_peer_any_grad_both.tex <==
Both pre- and post-AA alumni&&0.035&&0.073&\sym{**}&0.038&&0.035&&0.047&&0.012&\\
&&(0.030&)&(0.034&)&(0.032&)&(0.033&)&(0.043&)&(0.036&)\\


==> results/rddiff_peer_any_grad_diff.tex <==
Alum from different cohort&&0.054&\sym{*}&0.033&&0.066&\sym{*}&$-$0.027&&$-$0.050&&$-$0.038&\\
&&(0.032&)&(0.034&)&(0.039&)&(0.034&)&(0.037&)&(0.040&)\\


==> results/rddiff_peer_any_grad_post.tex <==
Post-AA alumni only&&0.046&\sym{*}&0.017&&$-$0.029&&0.117&\sym{***}&0.046&&$-$0.071&\sym{*}\\
&&(0.025&)&(0.026&)&(0.029&)&(0.034&)&(0.039&)&(0.040&)\\


==> results/rddiff_peer_any_grad_pre.tex <==
Pre-AA alumni only&&0.012&&$-$0.026&&$-$0.038&&0.052&\sym{**}&0.054&\sym{**}&0.003&\\
&&(0.022&)&(0.024&)&(0.026&)&(0.025&)&(0.028&)&(0.029&)\\


==> results/rddiff_peer_any_grad_same.tex <==
Alum from same cohort&&0.030&&0.074&\sym{**}&0.068&\sym{*}&$-$0.031&&$-$0.025&&$-$0.023&\\
&&(0.030&)&(0.030&)&(0.039&)&(0.029&)&(0.030&)&(0.035&)\\


==> results/rddiff_peer_n.tex <==
\(N\) (any cohort)&&27,492&&31,289&&4,718&&51,057&&64,198&&9,727&\\


==> results/rddiff_prof.tex <==
Professional occupation&&$-$0.105&&$-$0.184&&0.122&&0.165&&$-$0.783&&$-$0.774&\sym{*}\\
&&(0.113&)&(0.120&)&(0.116&)&(0.124&)&(0.502&)&(0.418&)\\


==> results/rddiff_rio_muni.tex <==
Worked in Rio de Janeiro&&$-$0.027&&$-$0.012&&$-$0.293&\sym{**}&$-$0.360&\sym{**}&0.463&&0.198&\\
&&(0.095&)&(0.103&)&(0.135&)&(0.141&)&(0.638&)&(0.542&)\\


==> results/rddiff_rio_st.tex <==
Worked in state of RJ&&$-$0.125&&$-$0.093&&$-$0.154&&$-$0.131&&0.137&&$-$0.005&\\
&&(0.101&)&(0.104&)&(0.108&)&(0.114&)&(0.455&)&(0.406&)\\


==> results/rddiff_top_ind2.tex <==
Most common industry (2 digit)&&$-$0.122&&$-$0.166&&0.090&&0.044&&$-$0.996&&$-$0.981&\sym{*}\\
&&(0.116&)&(0.122&)&(0.117&)&(0.125&)&(0.694&)&(0.563&)\\


==> results/rddiff_top_ind5.tex <==
Worked in modal industry for UERJ alumni&&$-$0.134&&$-$0.191&\sym{*}&0.212&\sym{**}&0.173&&$-$0.497&&$-$0.516&\\
&&(0.102&)&(0.108&)&(0.103&)&(0.107&)&(0.437&)&(0.372&)\\


==> results/topenr_age.tex <==
Age at application&&20.974&&22.802&&20.595&&22.154&\\


==> results/topenr_black_rais.tex <==
Black&&0.021&&0.028&&0.059&&0.084&\\


==> results/topenr_brown_rais.tex <==
Brown&&0.136&&0.174&&0.213&&0.238&\\


==> results/topenr_female_any.tex <==
Female&&0.458&&0.541&&0.484&&0.527&\\


==> results/topenr_ind1.tex <==
Public administration&&0.351&&0.386&&0.270&&0.318&\\


==> results/topenr_ind10.tex <==
Extractive industries&&0.035&&0.020&&0.019&&0.012&\\


==> results/topenr_ind11.tex <==
Total in top 10 industries&&0.812&&0.822&&0.756&&0.790&\\


==> results/topenr_ind2.tex <==
Education&&0.082&&0.166&&0.098&&0.198&\\


==> results/topenr_ind3.tex <==
Services&&0.104&&0.079&&0.133&&0.104&\\


==> results/topenr_ind4.tex <==
Finance&&0.072&&0.058&&0.045&&0.042&\\


==> results/topenr_ind5.tex <==
Health and social services&&0.050&&0.015&&0.067&&0.017&\\


==> results/topenr_ind6.tex <==
Computer activities&&0.036&&0.023&&0.045&&0.026&\\


==> results/topenr_ind7.tex <==
Retail trade&&0.024&&0.030&&0.029&&0.035&\\


==> results/topenr_ind8.tex <==
Telecommunications&&0.034&&0.020&&0.019&&0.017&\\


==> results/topenr_ind9.tex <==
Professional associations&&0.023&&0.025&&0.031&&0.023&\\


==> results/topenr_ind_11.tex <==
Extractive industries&&0.032&&0.021&&0.022&&0.022&\\


==> results/topenr_ind_23.tex <==
Oil industry&&0.047&&0.021&&0.048&&0.026&\\


==> results/topenr_ind_51.tex <==
Wholesale&&0.020&&0.014&&0.015&&0.023&\\


==> results/topenr_ind_65.tex <==
Finance&&0.093&&0.058&&0.093&&0.074&\\


==> results/topenr_ind_72.tex <==
Computer activities&&0.021&&0.014&&0.027&&0.015&\\


==> results/topenr_ind_74.tex <==
Services provided to companies&&0.057&&0.033&&0.058&&0.079&\\


==> results/topenr_ind_75.tex <==
Public administration and defense&&0.405&&0.473&&0.358&&0.351&\\


==> results/topenr_ind_80.tex <==
Education&&0.121&&0.180&&0.132&&0.211&\\


==> results/topenr_ind_85.tex <==
Health and social services&&0.035&&0.013&&0.050&&0.016&\\


==> results/topenr_ind_92.tex <==
Recreational and cultural activities&&0.026&&0.015&&0.032&&0.017&\\


==> results/topenr_ind_t10.tex <==
Share hired by top 10 industries&&0.857&&0.844&&0.835&&0.835&\\


==> results/topenr_lwage_03.tex <==
Mean log hourly wage (2003--2008)&&2.795&&2.676&&0.119&\sym{***}\\
&&&&&&(0.001&)\\


==> results/topenr_lwage_13.tex <==
Mean log hourly wage (2008--2013)&&3.123&&3.028&&0.095&\sym{***}\\
&&&&&&(0.001&)\\


==> results/topenr_lwage_17.tex <==
Mean log hourly wage (2013--2018)&&3.417&&3.353&&0.063&\sym{***}\\
&&&&&&(0.001&)\\


==> results/topenr_n.tex <==
\(N\)&&7,915&&8,513&&9,464&&9,930&\\


==> results/topenr_n_ind.tex <==
\(N\)&&5,665&&6,414&&6,660&&7,762&\\


==> results/topenr_score.tex <==
Admission score&&0.861&&$-$0.279&&1.026&&0.094&\\


==> results/topenr_wage_grw_03.tex <==
Mean wage growth (2003--2008)&&0.085&&0.085&&0.000&\\
&&&&&&(0.000&)\\


==> results/topenr_wage_grw_13.tex <==
Mean wage growth (2008--2013)&&0.082&&0.081&&0.001&\sym{***}\\
&&&&&&(0.000&)\\


==> results/topenr_wage_grw_17.tex <==
Mean wage growth (2013--2018)&&0.045&&0.045&&$-$0.000&\\
&&&&&&(0.000&)\\


==> results/topenr_white_rais.tex <==
White&&0.832&&0.790&&0.709&&0.658&\\


==> results/wage_grw.tex <==
Gov't Firm&&0.345&\sym{***}&0.340&\sym{***}&0.249&\sym{***}&$-$0.020&\sym{***}&$-$0.019&\sym{***}&$-$0.026&\sym{***}\\
&&(0.005&)&(0.005&)&(0.010&)&(0.003&)&(0.003&)&(0.008&)\\
Constant&&2.975&\sym{***}&2.640&\sym{***}&2.700&\sym{***}&0.096&\sym{***}&0.132&\sym{***}&0.127&\sym{***}\\
&&(0.003&)&(0.009&)&(0.008&)&(0.002&)&(0.005&)&(0.006&)\\
\(N\)&&147858&&147351&&144445&&44377&&44185&&43234&\\

